Lateral turbulent jet in rarefied environment

Lateral jets play a crucial role in controlling the trajectory and aerodynamic heating of hypersonic vehicles. However, the complex interaction between turbulent and rarefaction effects has rarely been examined. This study fills this knowledge gap by employing the newly developed GSIS-SST method [J. Fluid Mech. 1002 (2025) A10], which combines the shear stress transport (SST) model for turbulent flow and the general synthetic iterative scheme (GSIS) for rarefied gas flow. It is found that, at altitudes from 50 km to 80 km, the maximum relative difference in the pitch moment between the GSIS-SST and pure GSIS (SST) reaches 28% (20%). While the jet is supposed to reduce the surface heat flux, its turbulence significantly diminishes this reduction, e.g., the GSIS-SST predicts a heat flux about one order of magnitude higher than the GSIS when the jet pressure ratio is 1.5. Increasing the angle of attack intensifies local turbulence, resulting in expanded discrepancies in shear stress and heat flux between GSIS-SST and GSIS. These insights enhance our comprehension of lateral jet flows and highlight the importance of accounting for both turbulent and rarefaction effects in medium-altitude hypersonic flight.

==> Methodology.tex <==
\section{Multiscale GSIS-SST method}\label{sec:NumMethod}

The GSIS-SST method \citep{Tian2024multiscale} is based on the GSIS that solves the Boltzmann model equation for rarefied gas flows \citep{Zeng2023General,Liu2024Further,Zhang2024Efficient} and the SST model for turbulent flows. Here we briefly introduce its basic features.

\subsection{GSIS for rarefied gas flows}

The original GSIS method for polyatomic gases is consisted of a mesoscopic solver and a macroscopic solver. The mesoscopic solver is grounded on the modified Rykov model \citep{Li2021Uncertainty,Wu2015kinetic}. Two velocity distribution functions (VDFs) ${f}_{1}$ and ${f}_{2}$ are used to describe the translational and internal states of molecules, and they are governed by the following kinetic equations:
\begin{equation}\label{eq:Rykov}
\frac{{\partial f}_{l}}{{\partial t}} + \boldsymbol{\xi} \cdot \nabla {f}_{l} = \frac{{g}_{l,t}-{f}_{l}}{\tau} + \frac{{g}_{l,i}-{g}_{l,t}}{{Z}_{i}\tau},\quad l=0, 1,
\end{equation}
where $t$ is the time, $\boldsymbol{\xi}$ is the molecular velocity; $\tau$ and ${Z}_{i}\tau$ are the elastic and inelastic collision time respectively, with ${Z}_{i}$ being the internal collision number. The reference VDFs ${g}_{l,t}$ and ${g}_{l,i}$ represent the state to which the gas system will relax.

When applied in two dimensional space, the dimension of velocity space is also reduced by integrating through the $z$ direction. The reduction of dimension introduces three VDFs:
\begin{equation}
(\tilde{{f}_{0}}, \tilde{{f}_{1}}, \tilde{{f}_{2}}) = \int({f}_{0}, {f}_{1}, {\xi}^2_{z}{f}_{0})d{\xi}_{z},
\end{equation}
Consequently, the index $l$ in ~\eqref{eq:Rykov} is extended to 2, and there are also six reference VDFs:
\begin{equation}\label{reference_VDF}
    \begin{aligned}
        g_{0t}&= \rho\left(\frac{1}{2\pi T_t}\right)\exp\left(-\frac{c^2}{2T_t}\right)\left[1+\frac{2\bm{q}_{t}\cdot\bm{c}}{15T_tp_t}\left(\frac{c^2}{2T_t}-2\right)\right],\\
        g_{0i}&= \rho\left(\frac{1}{2\pi T}\right)\exp\left(-\frac{c^2}{2T}\right)\left[1+\frac{2\bm{q}_{0}\cdot\bm{c}}{15Tp}\left(\frac{c^2}{2T}-2\right)\right],\\
        g_{1t}&=\frac{d_i}{2}T_rg_{0t} + \left(\frac{1}{2\pi T_t}\right)\frac{\bm{q}_{i}\cdot\bm{c}}{T_t}\exp\left(-\frac{c^2}{2T_t}\right), \\
        g_{1i}&=\frac{d_i}{2}Tg_{0i} + \left(\frac{1}{2\pi T}\right)\frac{\bm{q}_{1}\cdot\bm{c}}{T}\exp\left(-\frac{c^2}{2T}\right),\\
        g_{2t}&= \rho\left(\frac{1}{2\pi}\right)\exp\left(-\frac{c^2}{2T_t}\right)\left[1+\frac{2\bm{q}_{t}\cdot\bm{c}}{15T_tp_t}\left(\frac{c^2}{2T_t}-1\right)\right],\\
        g_{2i}&= \rho\left(\frac{1}{2\pi}\right)\exp\left(-\frac{c^2}{2T}\right)\left[1+\frac{2\bm{q}_{0}\cdot\bm{c}}{15Tp}\left(\frac{c^2}{2T}-1\right)\right],
    \end{aligned}
\end{equation}
where the macroscopic quantities (density, velocity, stress, temperature, heat flux) are related to the reduced VDFs as:
\begin{equation}
\begin{aligned}
(\rho, \rho\boldsymbol{u}) &= \int(\tilde{{f}_{0}}, \boldsymbol{\xi}\tilde{{f}_{0}})d{\boldsymbol{\xi}},\quad
\boldsymbol{\sigma}= \int\boldsymbol{cc}\tilde{{f}_{0}}-\frac{1}{3}(c^2\tilde{{f}_{0}}+\tilde{{f}_{2}})\textbf{I}d{\boldsymbol{\xi}},\\
\left(\frac{3}{2}\rho{T}_{t}, \frac{{d}_{i}}{2}\rho{T}_{i}\right) &= \int(\frac{1}{2}(c^2\tilde{{f}_{0}}+\tilde{{f}_{2}}),\tilde{{f}_{1}})d{\boldsymbol{\xi}},\quad
({\boldsymbol{q}}_{t}, {\boldsymbol{q}}_{i}) = \int\left(\frac{1}{2}(c^2\tilde{{f}_{0}}+\tilde{{f}_{2}}),\tilde{{f}_{1}}\right)\boldsymbol{c}d{\boldsymbol{\xi}},
\end{aligned}
\end{equation}
with $\textbf{I}$ being the identity matrix. 
The total temperature is $T=(3T_t+d_iT_i)/(3+d_i)$, the total pressure is $p=\rho {}T$, and the pressure related to the translational motion is $p_t=\rho {}T_t$; $\bm{q}_{0}$ and $\bm{q}_{1}$ are linear combinations of translational and internal heat fluxes \citep{Li2021Uncertainty}:
\begin{equation}
    \begin{bmatrix} 
        \bm{q}_{0} \\ \bm{q}_{1} 
    \end{bmatrix}
    =
    \begin{bmatrix}		
        (2-3A_{tt})Z_i+1 & -3A_{ti}Z_i  \\		
        -A_{it}Z_i & -A_{ii}Z_i+1 \\ 
    \end{bmatrix}
    \begin{bmatrix} 
    \bm{q}_{t} \\ \bm{q}_{i} 
    \end{bmatrix}.
\end{equation}
For nitrogen, we choose the internal degrees of freedom  $d_i=2$, $Z_i=3.5$, and $\bm{A}=[A_{tt},A_{ti},A_{it},A_{ii}]=[0.786,-0.201,-0.059,0.842]$.


The kinetic equation \eqref{eq:Rykov} can be solved by the implicit iterative discrete velocity method, which is rather slow when the Knudsen number is small, and is subject to large numerical dissipation when coarse spatial grids are used. The GSIS is developed to tackle the two problems\citep{Su2020Can,Su2020Fast,Zeng2023General,Liu2024Further,Zhang2024Efficient}, where the key innovation behind the GSIS is that, in addition to solve the mesoscopic kinetic equation, the macroscopic synthetic equations are also solved. 

The synthetic equations are exactly derived by taking the velocity moments of the kinetic equation \eqref{eq:Rykov}: 
\begin{equation}\label{eq:macroscopic_equation_2}
\begin{aligned}
\frac{\partial \rho}{\partial t} + \nabla \cdot (\rho \boldsymbol{u}) &= 0,\\
\frac{\partial \rho \boldsymbol{u}}{\partial t} + \nabla \cdot (\rho \boldsymbol{u} \boldsymbol{u}) &= -\nabla \cdot (\rho T_t \textbf{I} + \boldsymbol{\sigma}),\\    
\frac{\partial \rho e}{\partial t} + \nabla \cdot (\rho e \boldsymbol{u}) &= -\nabla \cdot (\rho T_t \boldsymbol{u} + \boldsymbol{\sigma} \cdot \boldsymbol{u} + {\boldsymbol{q}}_{t} + {\boldsymbol{q}}_{i}),\\
\frac{\partial \rho e_i}{\partial t} + \nabla \cdot (\rho e_r \boldsymbol{u}) &= -\nabla \cdot {\boldsymbol{q}}_{i} + \frac{d_i \rho}{2}\frac{T-T_i}{{Z}_{i}\tau},
\end{aligned}
\end{equation}
where $e=(3+d_i)T/2+u^2/2$, $e_i=d_iT_i/2$.

The above equation is not closed because the stress and heat flux are not known. In GSIS, the constitutive relations are constructed as follows,
\begin{equation}\label{eq:full_constitutive}
    \begin{aligned}
        \bm{\sigma} &= \underbrace{-\mu \left(\nabla\bm{u}+\nabla\bm{u}^{\mathrm{T}}-\frac{2}{3}\nabla\cdot\bm{u}\mathrm{I}\right)}_{\bm{\sigma}^{\text{NS}}} + \text{HoT}_{\bm{\sigma}},\\
        \bm{q}_{t} &=\underbrace{-\kappa_t\nabla T_t}_{\bm{q}_{t}^{\text{NS}}} + \text{HoT}_{\bm{q}_{t}},\quad
        \bm{q}_{i} =\underbrace{-\kappa_r\nabla T_i}_{\bm{q}_{i}^{\text{NS}}} + \text{HoT}_{\bm{q}_{i}},
    \end{aligned}
\end{equation}
which not only contain those used in the NS equation ($\mu$ is the physical viscosity; $\kappa_{t}$ and $\kappa_{i}$ are the translational and internal heat conductivities, respectively), but also contains the high-order terms (HoTs) that describe the rarefaction effects:
\begin{equation}\label{eq:getHoTs}
    \begin{aligned}
        \text{HoT}_{\bm{\sigma}} &= \int \left(\boldsymbol{cc}\tilde{{f}_{0}}-\frac{1}{3}(c^2\tilde{{f}_{0}}+\tilde{{f}_{2}})\textbf{I}\right)d{\boldsymbol{\xi}} - \bm{\sigma}^{\text{NS}},\\
      \text{HoT}_{\bm{q}_{t}} &= \int \frac{1}{2}\boldsymbol{c}(c^2\tilde{{f}_{0}}+\tilde{{f}_{2}}) \mathrm{d}\bm{\xi} - \bm{q}_{t}^{\text{NS}},\quad
        \text{HoT}_{\bm{q}_{i}} = \int \bm{c}\tilde{{f}_{1}} \mathrm{d}\bm{\xi} - \bm{q}_{i}^{\text{NS}}.
    \end{aligned}
\end{equation}


%viscosity $\mu_\text{ref}=\rho_\text{ref}v_\text{ref}L$, turbulent kinetic energy $k_\text{ref}=v^2_\text{ref}$, turbulent dissipation frequency $\omega_\text{ref}=\rho_\text{ref}v^2_\text{ref}/\mu_\text{ref}$.

Note that the above quantities are normalized by the corresponding reference quantities (denoted by subscript 0) \citep{Zhang2024Efficient}: density $\rho_\text{ref}=\rho_0$, temperature $T_\text{ref}=T_0$, length $L_0$, velocity $v_\text{ref}=\sqrt{RT_0}$, time $t_\text{ref}=L_0/v_\text{ref}$, pressure $p_\text{ref}=\rho_0 R T_0$, heat flux $q_\text{ref}=p_\text{ref}v_\text{ref}$. 
The relaxation time in ~\eqref{eq:Rykov} is determined as 
\begin{equation}
    \tau=\sqrt{\frac{\pi}{2}}\text{Kn}\frac{T^\omega}{p_t},
\end{equation}
where Kn is the Knudsen number, and $\omega=0.74$ is the viscosity index of nitrogen. 

Finally, it should be noted that, in GSIS, the NS constitutive relations in \eqref{eq:full_constitutive} and \eqref{eq:getHoTs} are evaluated at distinct iterative steps, and they don't cancel each other out until the convergence is achieved. It is in fact this unique arrangement that leads to the fast convergence and asymptotic-preserving of GSIS \citep{Su2020Fast}.



\subsection{SST turbulence model in continuum flows}

The NS equations (i.e., \eqref{eq:macroscopic_equation_2} and \eqref{eq:full_constitutive} with HoTs being zero) are adequate to describe gas dynamics in the continuum flow regime. However, the presence of turbulence requires highly refined spatial grid. Therefore, turbulence models, which permits the use of coarse grids, are widely used in engineering problems. Here the popular $k$-$\omega$ SST model \citep{Menter1994Two} is adopted, and the viscosity and thermal conductivities in the NS constitutive relations are changed to  
\begin{equation}\label{eq:Turb_full_constitutive}
    \begin{aligned}
        \mu\rightarrow & \mu_{lam}+\mu_{turb},\\
        \kappa_{t}\rightarrow & \kappa_{t,lam}+\kappa_{t,turb},\\
        \kappa_{i} \rightarrow& \kappa_{r,lam}+\kappa_{r,turb},
    \end{aligned}
\end{equation}
where the subscript $lam$ indicates the original physical parts, and the subscript $turb$ denotes the turbulent parts. 
The dimensionless turbulent viscosity is given by
\begin{equation}\label{eq:mu_t}
\mu_{turb} ={a_R \rho k}/{\max\left(a_R \omega, \frac{\Vert\Omega\Vert F_{\mu}}{\text{Re}_\text{ref}}\right)},
\end{equation}
where $k$ represents the turbulent kinetic energy, $\omega=\rho k/\mu_t$ is the turbulent dissipation frequency, with $\Vert\Omega\Vert$ being the vorticity magnitude. Here, $a_R$ is a constant from the Bradshaw assumption, $F_\mu$ is a blending function that takes the value of one for boundary layer flows and zero for free shear flows. The turbulent heat conductivity (irrespective of translational or internal) is obtained as follows: 
\begin{equation}\label{eq:mutCoupling}
    \kappa_{turb} =\frac{\mu_{turb}\text{Pr}_{lam}}{\text{Pr}_{turb}} \frac{c_p}{\text{Pr}_{lam}},
\end{equation}
where the laminar to turbulent Prandtl number ratio is set to 0.8, with the value of $c_p/\text{Pr}_{lam}$ for $\kappa_t$ and $\kappa_r$ obtained using the coefficients for nitrogen from \cite{Li2021Uncertainty} accordingly:
\begin{equation}\label{eq:kappaAnumber}
	\left[ 
      \begin{array}{ccc} 
        \kappa_t \\ \kappa_r 
      \end{array}
    \right]
	= \mu
        \left[
        \begin{array}{ccc} 
        3.546 \\ 1.435
        \end{array}
        \right].
\end{equation}

The SST model combines the advantages of both low- and high-Reynolds number turbulence models, blending the $k$-$\omega$ model near the wall with the $k$-$\epsilon$ model in the free stream. This combination allows it to accurately predict boundary layer separation and flow behavior under adverse pressure gradients, making it well-suited for complex aerodynamic flows. Furthermore, it embeds Bradshaw's assumption for boundary layers, which assumes that the turbulent shear stress is proportional to turbulent kinetic energy, providing a more reliable prediction of turbulent boundary layers \citep{Menter1994Two}.
The SST model is originally developed for incompressible flows. To simulate hypersonic flows, here the pressure-dilatation and dilatation dissipation terms are incorporated following the approach by \cite{Sarkar1992pressure}, while the pressure work term is omitted due to the absence of a satisfactory correction model and the lack of evidence supporting the coupling of separately developed correction models for these terms.

The final form of the SST model reads:
\begin{equation}\label{eq:k}
\begin{aligned}
\frac{\partial{\rho k}}{\partial{t}}+\frac{\partial{\rho u_j k}}{x_j}=&\frac{1}{\text{Re}_\text{ref}} \frac{\partial}{\partial{x_j}}
\left[
(\mu_{lam}+\sigma_k \mu_{turb})\frac{\partial{k}}{\partial{x_j}}
\right]
+\underbrace{\tau_{turb,ij}\frac{\partial{u_i}}{\partial{x_j}}}_{Prod_k}-\underbrace{\text{Re}_\text{ref}\beta^* \rho \omega k}_{Diss_k}\\
&-\underbrace{\text{Re}_\text{ref}\beta^*  \xi^* M^2_t \rho \omega k}_{\text{Dilatation dissipation}}
+\underbrace{\alpha_2 \tau_{turb,ij}\frac{\partial{u_i}}{\partial{x_j}} M_t + \text{Re}_\text{ref} \alpha_3 \beta^* \rho \omega k M^2_t}_{\text{pressure dilatation}},
\end{aligned}
\end{equation}
\begin{equation}\label{eq:omega}
\begin{aligned}
\frac{\partial{\rho \omega}}{\partial{t}}+\frac{\partial{\rho u_j \omega}}{x_j}=&\frac{1}{\text{Re}_\text{ref}} \frac{\partial}{\partial{x_j}}
\left[
(\mu_{lam}+\sigma_\omega \mu_{turb})\frac{\partial{\omega}}{\partial{x_j}}
\right]
+\gamma \frac{\rho}{\mu_{turb}} \tau_{turb,ij}\frac{\partial{u_i}}{\partial{x_j}}
\\
&-\text{Re}_\text{ref}\beta \rho \omega^2+\frac{2 (1-F_\phi)}{\text{Re}_\text{ref}} \frac{\rho \sigma_{\omega 2}}{\omega} \frac{\partial{k}}{\partial{x_j}}\frac{\partial{\omega}}{\partial{x_j}}
+\underbrace{\text{Re}_\text{ref}\beta^* \xi^* M^2_t \rho \omega^2}_{\text{Dilatation dissipation}}.
\end{aligned}
\end{equation}


%here, $F_\phi$ is the blending function which transform the model and its coefficients from $k$-$\omega$ model in near wall region ($F_\phi=1$) to $k$-$\epsilon$ model in the main flow area ($F_\phi=0$), the model coefficient $\phi=(\sigma_k, \sigma_{\omega}, \beta, \beta^*, \kappa_{\phi}, \gamma)$ is blended as $\phi=F_\phi \phi_1 + (1-F_\phi) \phi_2$. These model functions and coefficients are also given in \cite{Menter1994Two}. The $M_t=\sqrt{2k}/\sqrt{\gamma R T}$ is the turbulent Mach number. Compressibility correction related model coefficients ($\alpha_2, \alpha_3, \xi^*$) are summarized in reference\cite{Wilcox2006turbulence}. With these correction terms, the modified SST model works fine for jets and free shear flow at low Reynolds number.

Note that the Favre-averaged Reynolds-stress computed under the Boussinesq eddy-viscosity hypothesis is 
\begin{equation}
    \boldsymbol{\tau}_{turb} = \mu_{turb} \left(\nabla{\boldsymbol{u}}+\nabla{\boldsymbol{u^\text{T}}}-\frac{2}{3}\nabla\cdot\boldsymbol{u}\textbf{I}\right) - \frac{2}{3} \rho k \textbf{I}.
\end{equation}
And to eliminate certain erroneous spikes of $\mu_{turb}$ rooted in two-equation turbulence models~\citep{Menter1993Zonal}, the production term in ~\eqref{eq:k} is modified as
\begin{equation}
   {Prod'}_{k}= \min \left({Prod_k}, 20 Diss_k\right). 
\end{equation}

At solid surface, $k=0$ and $\omega =({60\mu_{lam}})/({\text{Re}_\text{ref}{\beta}_{1}\rho D_{1}^{2}})$ are specified, with $D_{1}$ being the distance of the first cell center to the wall. For other parameters we refer to \cite{Wilcox2006turbulence,Tian2024multiscale}.

%Notice, to be consistent with the normalization in GSIS~\citep{Zhang2024Efficient}, reference quantities are defined based on free flow properties (denoted by subscript 0): density $\rho_\text{ref}=\rho_0$, temperature $T_\text{ref}=T_0$, velocity $v_\text{ref}=\sqrt{RT_0}$, pressure $p_\text{ref}=\rho_0 R T_0$, heat flux $q_\text{ref}=p_\text{ref}v_\text{ref}$, viscosity $\mu_\text{ref}=\rho_\text{ref}v_\text{ref}L$, turbulent kinetic energy $k_\text{ref}=v^2_\text{ref}$, turbulent dissipation frequency $\omega_\text{ref}=\rho_\text{ref}v^2_\text{ref}/\mu_\text{ref}$.



\subsection{GSIS-SST for rarefied and turbulent flows}

As stated in the introduction, the direct simulation of turbulence based on kinetic theory is resource intensive. The cost-efficient path of considering turbulence with current multiscale methods still goes to the Reynolds-averaged Navier–Stokes (RANS) models. Thanks to the explicit inclusion of the synthetic NS solver, the eddy-viscosity hypothesis based RANS models can be seamlessly integrated into the GSIS framework through ~\eqref{eq:full_constitutive}. That is, in the GSIS-SST\citep{Tian2024multiscale}, the mesoscopic kinetic equation~\eqref{eq:Rykov} is solved, together with the macroscopic synthetic equation \eqref{eq:macroscopic_equation_2} equipped with the following constitutive relations 
\begin{equation}\label{eq:Turb_full_constitutive}
    \begin{aligned}
        \bm{\sigma} &= -(\mu_{lam}+\mu_{turb})\left(\nabla\bm{u}+\nabla\bm{u}^{\mathrm{T}}-\frac{2}{3}\nabla\cdot\bm{u}\mathrm{I}\right) + \text{HoT}_{\bm{\sigma}},\\
        \bm{q}_{t} &= -(\kappa_{t,lam}+\kappa_{t,turb})\nabla T_t + \text{HoT}_{\bm{q}_{t}},\\
        \bm{q}_{i} &= -(\kappa_{r,lam}+\kappa_{r,turb})\nabla T_r + \text{HoT}_{\bm{q}_{i}},
    \end{aligned}
\end{equation}
where the turbulence viscosity is obtained from the SST model. 

The GSIS-SST has nice asymptotic preserving behaviors. When the Knudsen number is low (Reynolds number is high), the HoT terms, obtained from the multiscale Chapman-Enskog expansion of the kinetic model~\citep{Su2020Fast}, are proportional to $\text{Kn}^2$. Therefore, in the continuum limit, the above constitutive relations reduce to the linear NS relations for turbulent flows. That is, the GSIS-SST method is effectively the SST turbulence model. When the Knudsen number is high (Reynolds number is low), the gas density decreases and molecular mean free path increases. The density and shear motion related turbulent viscosity $\mu_{turb}$ becomes negligible compared to the physical viscosity $\mu_{lam}$. As a result, the turbulence production is so weak that the flow dynamics are dominated by rarefaction effects. The GSIS-SST method is effectively the GSIS method that solves the Boltzmann kinetic equation for rarefied gas dynamics. In our previous work\citep{Tian2024multiscale}, it is reported that in the hypersonic flow of Mach number 25 passing over a blunt leading edge, the turbulent effects in GSIS-SST start to dominant only when $\text{Kn}\lessapprox0.001$. 


% The numerical procedure and validations can be found in our recent works\cite{Zhang2024Efficient,Tian2024multiscale}.

%The solution process starts with the physical domain decomposition process, in which the physical space is partitioned into connected pieces using the METIS tool. Then the macroscopic solver provides a roughly solved initial field. The mesoscopic solver calculates the VDFs in parallel using message passing interface (MPI) with these macroscopic variables and iterates to obtain the updated VDFs. Taking moments of these new VDFs, macroscopic variables are also updated and higher-order correction terms for the stress and heat flux are offered. The higher-order correction terms are the difference between the VDF-integrated values and the classical linear constitutive relations. The macroscopic solver iterates with these DVM provided variables and corrections for a certain amount of steps. After that, the VDFs are calculated from the new macroscopic variables and the above process are repeated until the mesoscopic solver converges.

%Theoretically, turbulence can be investigated by the DNS of \eqref{eq:macroscopic_equation_2} with the NS constitutive relations. However, its prohibitive numerical cost prompts the use of turbulence models.  Though the RANS models are derived on coarse grids under multiple assumptions, they are widely accepted in engineering due to its low computational cost and good accuracy on capturing the flow pattern. Here, the popular $k$-$\omega$ shear stress transport (SST) model, which combines the advantages of both the low- and high-Reynolds numbers turbulence models and embeds the Bradshaw's assumption for boundary layer, is considered~\citep{Menter1994Two}. It is good at predicting of flow with adverse pressure gradients and separation.

==> Section_C.tex <==


\begin{figure*}
    \centering
    {\includegraphics[width=0.49\linewidth,trim={20 20 30 90}, clip]{Artworks/H90dRhoCP.png}}
    {\includegraphics[width=0.49\linewidth,trim={20 20 30 90}, clip]{Artworks/H100dRhoCP.png}}\\
    % {\includegraphics[width=0.33\linewidth]{Artworks/H90Sigma.png}}
    % {\includegraphics[width=0.33\linewidth]{Artworks/H100Sigma.png}}
    \caption{(Top) Contour of density gradient magnitude.
    (Bottom) Profile of three shear stress components at $x_1=0.35~\text{m}$. The altitudes are 90~km and 100~km in the left and right columns, respectively. 
    }
    \label{fig:H90H100dRho}
\end{figure*}
%,trim={30 60 50 90}, clip


\section{The influence of flight altitude}\label{sec:altitude}
\subsection{Flow Structure}
We now examine the change of flow characteristics across large range of altitude. The jet pressure ratio is maintained at $\text{PR}=2.5$, and the angle of attack is 15°. 

At lower altitude of 65~km, all the flow features similar as that at 70~km in previous section, while
%We now examine results at altitudes above 80~km, where rarefaction effects dominate the flow dynamics. The jet pressure ratio is maintained at $\text{PR}=2.5$, and the angle of attack is 15°.
at higher altitudes, rarefaction causes significant diffusion of the flow structures. The outer shock becomes dispersed, and shear layer thickening is evident due to increased molecular mean free path. Contours of density gradient magnitude and streamlines at 90km (Kn = 0.2) and 100km (Kn = 1.2) are shown in Fig.~\ref{fig:H90H100dRho}.

At 90~km, barrel shock remnants are faint but discernible, while the Mach disk is nearly absent. The expanded jet flow experiences no much compression and continues far downstream due to the rarefied environment, resembles the case AoA=0° at 80~km. The shear layer between the jet flow and free stream is wide further from the wall, driven by enhanced diffusion. The upstream vortex near the jet exit reduces to a compact structure, and the downstream vortex shrinks. Both GSIS-SST and GSIS solutions exhibit minor differences here, since TKE comes from areas with large gradients, which are now sharply weakened.

At 100~km, the flow simplifies further. Rarefaction leads to significant jet expansion, erasing characteristic features such as barrel shocks and vortices. The flow resembles a jet expanding into a vacuum, with streamlines deflected upstream and in the shear layer by the free flow. Both GSIS-SST and GSIS solutions converge entirely in this regime.

%Shear stress profiles at 90km (Fig.\ref{fig:H90H100dRho}) show that $\sigma_{12,lam}$ rises near $|x_2|\approx0.3~\text{m}$ at the outer shock and peaks at $|x_2|\approx0.2~\text{m}$, with a secondary and global maximum at $|x_2|\approx0.085~\text{m}$ near the shear layer. The existence of this peak is bi-fold, decreasing temperature from post-shock flow to cold jet flow, and increasing velocity gradients when approaching shear layer. Near the wall, $\sigma_{12,lam}$ decreases within the jet layer before rising again due to the increasing near-wall velocity gradients.
%The rarefaction contribution $\sigma_{12,HoT}$ rises earlier than $\sigma_{12,lam}$ in the far field and exhibits a significant negative peak just below the shear layer, within the area of expanded jet. With $|x_2|$ approaching the wall-compressed jet layer, $\sigma_{12,HoT}$ transitions to near-zero values, and runs to a negative value at wall.
%At 100km, $\sigma_{12,lam}$ shows a shifted global maximum at $|x_2|\approx0.018\text{m}$ and a monotonic decline to the wall, lacking the fluctuations observed at 90~km. The profile of $\sigma_{12,HoT}$ mirrors its 90~km counterpart above the shear layer (the 90~km one). It also infiltrates into the jet area near the wall. Following a negative peak at $|x_2| \approx 0.019~\text{m}$, it rises to a positive value at the wall, indicating an increased degree of thermal non-equilibrium at this highly rarefied altitude, where the temperature slip is more pronounced due to reduced molecular interactions. In contrast, the negative HoT contribution at lower altitudes primarily compensates for velocity slip.

In summary, the 90~km results highlight transitional flow behavior, with rarefaction moderating flow structures like vortices and shear layers. By 100km, rarefaction suppresses these features entirely, reducing the flow to a simple jet expansion. These findings demonstrate how rarefaction progressively simplifies the flow field, with GSIS-SST converging to GSIS solutions in highly rarefied regimes.

%Since the results at altitude 70~km and 80~km have been discussed, here we focus on results at altitudes above 80~km.  When the flight altitude goes up, rarefaction effect gets stronger, causing the outer shock to take on a dispersed shape rather than maintaining a strong discontinuity, as seen at lower altitudes in the continuum regime. The jet pressure ratio is still kept at $\text{PR}=2.5$, and the angle of attack is 15°.

%The contours of density gradient magnitude and streamlines at altitude 90~km (Kn=0.2) and 100~km (Kn=1.2) are given in Fig.~\ref{fig:H90H100dRho}. At 90~km, the structures of barrel shock can still be roughly identified, the Mach disk is nearly invisible. The shear layer between the jet flow and the free stream has significantly thickened due to diffusion induced by the large mean free path of the gas molecules. Additionally, the vortices in front of the jet flow are reduced to a single, relatively small vortex compared to those at lower altitudes. The downstream vortex is also smaller in size, and only minor differences are observed between the GSIS-SST and GSIS solutions regarding this vortex.

%At 100~km, the flow dynamics changes dramatically. The highly rarefied environment enables the jet flow to expand more significantly, occupying a larger area near the wall. Consequently, nearly all characteristic structures of the jet flow field vanish, resulting in a flow field resembling a simple jet expanding into a vacuum, with the primary distinction being the deflected streamlines in the shear layer. No vortices or shocks are identifiable, and the differences between the GSIS-SST and GSIS models become negligible.

% Figure~\ref{fig:H90H100Tt} gives the translational temperature contour at altitude 90~km and 100~km. It is clear from the figure that the high altitude associated rarefaction changes the flow field significantly. All the shock structures are thickened and diffusive. At 90~km, the hot area after the outer bow shock still locates under the model surface near the jet exit (i.e., $x_1\approx0.09~\text{m}$ and $x_2\approx-0.06~\text{m}$), while at 100~km such temperature peak moves forward to the tip of the sharp leading edge. 
% \begin{figure*}
%     \centering
%     {\includegraphics[width=0.49\linewidth]{Artworks/H90Tt.png}}
%     {\includegraphics[width=0.49\linewidth]{Artworks/H100Tt.png}}
%     \caption{Contour of translational temperature $T_t$ at altitude 90~km and 100~km.}
%     %\caption{Contour of translational temperature at altitude 90~km and 100~km.}
%     \label{fig:H90H100Tt}
% \end{figure*}
%\leib{As for the distribution of turbulent kinetic energy, sensible concentration could only be found near the jet exit from initial condition at 90~km, and also the Mach disk (which could only be noticed from large TKE), forming a strip of high TKE. At 100~km, the TKE and $\mu_{r}$ are much more ignorable except the jet exit. Thus, the solutions from GSIS-SST and GSIS overlaps well.}

%\subsection{Profiles of field quantities}

%Figure~\ref{fig:H90H100dRho} provides insight into the physical processes that shape the flow field. It is clear that at altitudes 90~km and 100~km, the turbulent stress $\sigma_{12,turb}$ is close to zero throughout the profile, and only the NS laminar and HoT parts are present. Thus, there is no sensible influence from turbulence on surface quantities, and the GSIS-SST has reduced to the GSIS. 

% \begin{figure*}
%     \centering
%     {\includegraphics[width=0.49\linewidth]{Artworks/H90Sigma.png}}
%     {\includegraphics[width=0.49\linewidth]{Artworks/H100Sigma.png}}
%     \caption{Profile of shear stress at $x_1=0.35~\text{m}$ from different physical process at altitude 90~km and 100~km.}
%     \label{fig:H90H100sigma}
% \end{figure*}

%At 90~km, $\sigma_{12,lam}$ starts to emerge at $|x_2|\approx0.3~\text{m}$ when approaching the outer shock. It reaches a local maximum at around $|x_2|\approx0.2~\text{m}$ and then a local minimum at $|x_2|\approx0.16~\text{m}$, at which the core layer of free flow post shock stands. Continue to the wall, $\sigma_{12,lam}$ becomes maximum at $|x_2|=0.085~\text{m}$, corresponding to the shear layer between the jet and free flow, where the large velocity gradients produces such maximum shear stress. Then, within the jet layer near the wall, $\sigma_{12,lam}$ drops due to small velocity change within jet layer, low jet flow temperature and the resulting low $\mu_{lam}$ near wall. The NS laminar stress increases again due to near wall velocity gradients. The rarefaction part of the shear stress $\sigma_{12,HoT}$ has similar rise and drop pattern in the free flow dominated region. It rises at further location from the wall than $\sigma_{12,lam}$ since it captures the rarefaction effect in the rarefied far field. $\sigma_{12,HoT}$ runs oppositely to $\sigma_{12,lam}$ within $|x_2|<0.16~\text{m}$. From this position, $\sigma_{12,HoT}$ drops substantially to a negative local minimum at around the shear layer ($|x_2|\approx0.085~\text{m}$), and returns to around zero where the continuous jet flow layer dominates. Finally in the Knudsen layer, $\sigma_{12,HoT}$ poses some influence to support the slip condition on the wall.

%At the altitude of 100~km, profiles of $\sigma_{12,lam}$ and $\sigma_{12,HoT}$ are similar to that at 90~km in free flow region above the shear layer. Differences rest mostly within the shear layer and jet flow dominated area. Since the flight environment is further rarefied, the jet flow determined using the constant $\text{PR}$ value has also much lower density and has entered into the transition regime. Therefore, the gas rarefaction effect gets stronger and infiltrates also into the jet flow area. Therefore, the maximum of $\sigma_{12,lam}$ mentioned at $|x_2|=0.085~\text{m}$ from 90~km is now shifted to $|x_2|=0.018~\text{m}$. After this maximum, the curve of $\sigma_{12,lam}$ drops constantly to the wall without any fluctuation as at altitude 90~km. In the region below $|x_2|=0.4~\text{m}$, $\sigma_{12,HoT}$ looks like the mirrored version (mirror plane at $\sigma_{12}=42$) of that from 90~km. 

%If the velocity and viscosity profiles are plotted, the physical ground that shapes the $\sigma_{12}$ curves could be revealed. Figure~\ref{fig:H90H100Viscosity} provides such information. The velocity profile at altitude 90~km looks smooth as a typical laminar boundary layer, it is just the boundary layer is so thick that all the near wall layers from different source are included and indistinguishable. The $\mu_{turb}$ from GSIS-SST equals nearly 0 after the initial disturbance around the outer shock, and thus has no influence to the flow field and physical quantities.

%\begin{figure*}
%    \centering
%    {\includegraphics[width=0.49\linewidth]{Artworks/H90Vis.png}}
%    {\includegraphics[width=0.49\linewidth]{Artworks/H100Vis.png}}
%    \caption{Profile of shear stress at $x_1=0.35~\text{m}$ from different physical process at altitude 90~km and 100~km.}
%    \label{fig:H90H100Viscosity}
%\end{figure*}

%As for the case of altitude 100~km, the velocity profile is now extremely extensive in $|x_2|$ direction, smooth and no any sign of different flow layers. The maximum point of $\mu_{lam}$ rests at $|x_2|=0.28~\text{m}$ near the core of free flow layer post shock. Only from the plot of pressure, could the layered structure be inferred. It can be seen that the free flow pressure starts to rise at $|x_2|\approx1~\text{m}$ and continues the trend to around 0.1~m, where the jet flow area starts (refer to streamlines in figure~\ref{fig:H90H100Tt}). Pressure in the jet flow layer keeps a relative stable value and decreases sharply when approaching the wall due to large near wall temperature gradient.

% \subsection{Non-Equilibrium Effect}
% Lastly, the non-equilibrium effect is visited. Figure~\ref{fig:H90TtTr} depicts the ratio between $T_t$ and $Tr$ at altitude 90~km. The majority of the area exhibits non-equilibrium governed by $T_t$. Lower ratio of $Tt/Tr$ only appears in jet expansion fan and downstream the jet Mach disk. As the mean free path of molecules increases at higher altitudes, collision frequency is largely reduced. Therefore, the more collision-dependent rotational temperature lags behind the translational temperature in the transformation of internal energy from kinetic energy.

% \begin{figure}
%     \centering
%     {\includegraphics[width=1\linewidth]{Artworks/H90TtTr.png}}
%     \caption{Contour of ratio between translational and rotational temperature with various pressure ratio.}
%     \label{fig:H90TtTr}
% \end{figure}

% The solution of $Tt/Tr$ for altitude 100~km is omitted, as nearly the entire flow field is dominated by the $T_t$-governed non-equilibrium effect, with the exception of only a negligible region at the jet exit.
%\section{Overall Implication on Lateral Jet Application}
Influence of turbulence on the integrated force and moment on the model lower surface displays itself basically under the altitude of 80~km. The results are listed in Table~\ref{tab:ForceMoment}.

%\leib{In this part, the overall integrated force and moment on the model lower surface are investigated. Also, due to the minimal influence from turbulence, the results from 90~km and 100~km are discarded here, and results at 65~km and 75~km are added. For these two additional cases, AoA is also kept at 15° and $\text{PR}=0,2.5$. The results are listed in Table~\ref{tab:ForceMoment}.}

% \begin{table}
%     \centering
%     \begin{tabular}{cllcllcllll}\hline
%          Altitude& AoA&PR&  SST& $Fx_1$&$Fx_2$&  $Mx_3$ &$Mjx_3$ &$K_{Fx2}$ & $K_{Mx3}$&$Cim$\\ \hline
%          65 km & 15°&2.5&   0& 2.33&98.39&   32.33&22.29&4.64 & 10.68 &0.374\\
%  & & & 1& 3.05& 111.08& 36.95 &25.62&5.93 & 15.26 &0.579\\
%  & & &RelDiff & 31.1\%& 12.9\% &14.3\% &14.9\% &27.7\% & 42.9\%&54.6\%\\

%  70 km& 15°& 2.5& 0& 3.49& 102.50 & 33.96 &23.50 &4.56 & 10.72 &0.358\\
%  & & & 1& 4.23& 109.74 & 36.99 &25.79 &5.29 & 13.72 & 0.490\\
%  & & &RelDiff & 21.2\%& 7.1\% &8.9\% &9.7\% &16.1\% & 28.1\%&36.9\%\\ \hline

%  75 km& 15°& 2.5& 0 & 5.34& 110.07 & 36.98 &25.75 &4.65 &11.42 &0.360\\ \hline
% & & & 1& 5.93& 112.60 & 37.93 &26.44 &4.90 & 12.36 &0.396\\
%  & & &RelDiff & 11.1\%& 2.3\% &2.6\% &2.7\% &5.5\% & 8.2\% &10.0\%\\

%  80 km& 15°& 2.5& 0 & 8.02 & 123.67 &42.26 &29.65 &5.20 & 13.64 &0.401\\ \hline
% & & & 1 & 8.26 &124.11 &42.33 &29.67 &5.24 &13.70 &0.402\\
%  & & &RelDiff & 3.0\% &0.4\% &0.2\% &0.1\% &0.8\% & 0.4\% &0.2\%\\
%     \end{tabular}
%     \caption{Axial force $Fx_1$, normal force $Fx_2$, pitch moment $Mx_3$ (relative to nose-tip), $Mjx_3$ (relative to jet center) and corresponding augmentation factors $K$ over 65~km to 80~km. Condition flags same as previous that in previous rows are omitted. Rows with SST flag equals 0 list GSIS results, while with flag 1 list GSIS-SST results. The rows start with RelDiff provides the relative difference of quantity of interest (QoI) from GSIS-SST (1 row above) relative to GSIS (2 rows above), i.e., $QoI_{GSIS-SST}/QoI_{GSIS}-1$.}
%     \label{tab:ForceMoment}
% \end{table}

% \begin{figure}
%     \centering
%     \subfloat[]{\includegraphics[width=0.32\linewidth]{Artworks/M20Mx3.png}}
%     \subfloat[]{\includegraphics[width=0.32\linewidth]{Artworks/M25Mx3.png}}
%     \subfloat[]{\includegraphics[width=0.32\linewidth]{Artworks/RelErrMx3.png}}
%     % {\includegraphics[width=0.32\linewidth]{Artworks/JetFM70.png}}
%     % {\includegraphics[width=0.32\linewidth]{Artworks/JetKM70.png}}
%     % {\includegraphics[width=0.32\linewidth]{Artworks/JetLD70.png}}
%     %{\includegraphics[width=0.32\linewidth]{Artworks/JetFM80.png}}
%     %{\includegraphics[width=0.32\linewidth]{Artworks/JetFM70_104.png}}
%     %{\includegraphics[width=0.32\linewidth]{Artworks/JetFM80_104.png}}
%     %{\includegraphics[width=0.32\linewidth]{Artworks/JetFMAll_10465.png}}
%     %{\includegraphics[width=0.32\linewidth]{Artworks/JetKM70.png}}
%     %{\includegraphics[width=0.32\linewidth]{Artworks/JetKM80.png}}
%     %{\includegraphics[width=0.32\linewidth]{Artworks/JetLD70.png}}
%     %{\includegraphics[width=0.32\linewidth]{Artworks/JetLD80.png}}
%     \caption{Figures above give the integrated forces, moments and their corresponding augmentation factors over the lower surface from 65~km to 80~km, thicker lines and larger symbols represent cases with jet, thinner lines and smaller symbols are for no jet cases. The first row are results at 70~km with variation in pressure ratio $\text{PR}$, the last row are results at nominal condition (AoA=0°, jet $\text{PR}=2.5$ and no jet cases) from 65~km to 80~km. The first column presents forces and moments (relative to nose-tip, i.e., origin) integrated over full range of the model lower surface, with jet boundary skipped if jet is on. The second column gives the force and moment augmentation factors for normal force $K_{Fx2}$, moment relative to origin $K_{Mx3}$ and to jet exit center $K_{Mx3_j}$. The last column offers plots of lift, drag and lift-to-drag ratio.
%     %the middle column are at 80~km with variation in angle of attack }
%     }
%     \label{fig:Mx3}
% \end{figure}

% \subsection{Integrated Forces and Moment}


% The integrated forces and moments on the model's lower surface were analyzed for altitudes of 65~km and 75~km, where the angle of attack was fixed at 15° and the pressure ratio $\text{PR}$ was set to 0 and 2.5. Results from these altitudes are shown in Table~\ref{tab:ForceMoment}. Due to the negligible influence of turbulence at 90~km and 100~km, data from these higher altitudes were excluded.

% Across altitudes ranging from 65~km to 80~km, a consistent trend emerges in the non-dimensional axial force $Fx_1$, normal force $Fx_2$, and pitching moment $Mx_3$. When the jet is off ($\text{PR}=0$), both $Fx_1$ and $Mx_3$ increase rapidly with altitude, whereas $Fx_2$ shows a nearly linear increase. The results from GSIS-SST closely converge with those from GSIS at higher altitudes, reflecting the reduced influence of turbulence as rarefaction effects dominate.

% When the jet is activated ($\text{PR}=2.5$), the aerodynamic behavior changes substantially. The axial force $Fx_1$ decreases significantly, while $Fx_2$ and $Mx_3$ increase sharply. The axial force now scales linearly with altitude, while the normal force increases at a faster rate. The trend of $Mx_3$ closely follows that of $Fx_2$, suggesting a less varied arm of $Fx_2$, implying the stable control effect of lateral jet designed with our $\text{PR}$. Differences between GSIS-SST and GSIS are most pronounced at lower altitudes, particularly for $Fx_1$, where a maximum relative difference of 31\% is observed at 65~km. At 80~km, this difference reduces to approximately 3\%, highlighting the turbulence adaptation capabilities of GSIS-SST.

% \leib{Asymptotic behavior Still Running}
% It has been seen that the GSIS-SST and GSIS converges above altitude 65~km, when there is no jet, while the turbulence jet expands the discrepancies between the two solvers, and exhibits an increasing discrepancy when flight altitude drops. Thus, flight altitudes in the range of 50~km to 70~km are investigated with the synthetic NS equations set, i.e, conventional two temperature NS solver, to examine the asymptotic behavior between GSIS-SST and NS-SST (NS solver with $k=\omega$ SST turbulence model).
% Since it is not realistic for a Mach 25 condition at 50~km, the Mach number for these NS related cases are reduced to 20. The jet pressure ratio and flight angle of attack are kept the same as previous section~\ref{sec:altitude}.

% The results of integrated normal force is \leib{plotted}, it is clear that the solution from GSIS-SST runs with a converging trend toward the NS-SST ones. 

% \leib{Figure} further illustrates the relative differences (GSIS-SST relative to NS-SST, GSIS-SST relative to GSIS). It can be read that from 50~km to 80~km, the GSIS-SST deviates from NS-SST, and converges with GSIS. The convergence of GSIS-SST and GSIS has been validated previously. The asymptotic behavior of GSIS-SST toward NS-SST is confirmed here through the trend of the curves, due to the existence of localized rarefaction effect and continuum breakdown, which is shock related and plentiful in the lateral jet flow field. Therefore, the normal forces from both solvers still stand a short distance from each other at low altitude of 50~km. Fortunately, the exact asymptotic behavior has been verified in our recent publication \leib{JFM accepted}.

% It could be concluded that the turbulence of jet at current pressure ratio and angle of attack poses most impact around 50~km to 75~km, at which conventional NS loses its validity due to rarefaction and traditional gas kinetic scheme becomes insufficient due to the absence of turbulence consideration. 

%As the jet is activated, axial force is largely reduced and normal force as well as moment is greatly increased. Their relationship with flight altitude have changed. The $Fx_1$ goes now near linearly, while $Fx_2$ takes a faster increasing pace as flies higher. The flow of $Mx_3$ curve resembles that of the normal force. The GSIS-SST results run similarly as the GSIS ones, with larger absolute difference occurring at lower altitudes. Though the difference between GSIS-SST and GSIS seems large for $Fx_2$ and $Mx_3$ (also $Mjx_3$), the largest relative difference comes from $Fx_1$, being 31\% at 65~km. GSIS-SST and GSIS results gradually converge as altitude increases, with the largest relative difference only around 3\% ($Fx_1$) at 80~km, reflecting the automatic adaption of GSIS-SST in activating the turbulence model.
%Deviation between the two solvers exists primarily at lower altitude of 65~km, though not as obvious as the normal force or moment in absolute scale, the relative error is largest for the axial force reaching 31\% (65~km), while at higher ones such difference decreases
% The relationship between forces, moments, and the pressure ratio $\text{PR}$ is illustrated in Figure~\ref{fig:FM} for the 70~km case. With increasing $\text{PR}$, the normal force $Fx_{2}$ and pitching moment $Mx_{3}$ both exhibit monotonic increases, while the axial force $Fx_{1}$ decreases slightly. The axial force with the jet on is notably lower than in the no-jet condition, confirming the effectiveness of the lateral jet in reducing frictional stress. The forces and moments relative to the nose tip scale nearly linearly with $\text{PR}$ across the range investigated. However, GSIS-SST consistently predicts higher values than GSIS, with discrepancies growing as $\text{PR}$ increases.

% Quantitatively, the relative difference in $Fx_{1}$ between GSIS-SST and GSIS grows from less than 0.1\% at $\text{PR}=0$ to 24\% at $\text{PR}=1.5$, stabilizing around 20\% for $\text{PR}=3.5$. For the normal force $Fx_{2}$, GSIS-SST and GSIS results converge at $\text{PR}=0$, but the discrepancy rises with increasing $\text{PR}$, reaching approximately 7.1\%. A clearer pattern is observed for $Mx_{3}$, where the relative difference increases with $\text{PR}$, peaking at 10.4\% at $\text{PR}=3.5$. These findings suggest that the modeled turbulence influence is non-uniform and plays a role in shifting the aerodynamic center.

%Lastly, for varying AoA, the largest discrepancy between GSIS-SST and GSIS occurs at AoA=0°, where a 4\% difference in $Fx_{1}$ is observed. This highlights the sensitivity of axial force predictions to turbulence effects at small angles of attack.
%As for the pattern of change for force $Fx_{1}$, $Fx_{2}$ and $Mx_{3}$ with pressure ratio $\text{PR}$, results at 70~km are plotted in the second row of figure~\ref{fig:FM}. It is clear that with the jet on, $Fx_{2}$ and $Mx_{3}$ increase as $\text{PR}$ goes up, while horizontal force $Fx_{1}$ reduces slightly with increased $\text{PR}$. Also the axial force $Fx_{1}$ with jet on is much lower than the no jet condition, affirming the effective friction reduction by the jet. Apart from the forces with jet off, the forces and moment relative to the nose-tip all scale near linearly with $\text{PR}$ investigated here. The deviation of GSIS-SST solution (represented only by symbols) from GSIS also enlarges with $\text{PR}$, with GSIS-SST always provides higher values. As for the quantified discrepancy, the relative difference of GSIS-SST $Fx_{1}$ with respect to GSIS is less than 0.1\% at no jet condition, 24\% to 20\% for $\text{PR}$ from 1.5 to 3.5, respectively. For the normal force $Fx_2$, GSIS-SST and GSIS converge again (relative difference $<0.01\%$), while with jet, the discrepancy rises as $\text{PR}$ increases and stagnates around 7.1\%. Larger and clear pattern between relative difference of moment $Mx_3$ is observed, reaching 10.4\% at $\text{PR}=3.5$. This suggests that the modeled turbulence influence is also not uniformly distributed and is effective also in shifting the aerodynamic center.

%As for the influence of turbulence with varying angle of attack, largest discrepancy of 4\% between GSIS-SST and GSIS is observed at AoA=0° for axial force.

%Moving on to altitude 80~km, the influence from angle of attack could be examined. The figures for 80~km also plot the result of GSIS and GSIS-SST for no jet cases at each AoA, which are presented with thinner lines and smaller symbols. There is no doubt that for the no jet cases, GSIS-SST and GSIS predictions make no difference. All the forces and moments increase as AoA goes up. The $Fx_1$ follows a good linear relation with AoA, while the $Fx_2$ and $Mx_3$ show an accelerating positive relation. With the jet on, it is shown that the shear stress $\sigma_{12}$ dominated $Fx_1$ heavily drops, and the pressure driven vertical force $Fx_2$ and its moment $Mx_3$ both increase. The discrepancy between GSIS-SST and GSIS is reduced to less sensible level of around 3.9\% (AoA=0°) to 3\% (15° and 30°) in $Fx_1$, a similar saturation in relative difference is also observed here. For $Fx_2$, the differences are 0.1\%, 0.4\% and -0.1\% for the three angles of attack, while for $Mx_3$ they are 0.5\%, 0.2\% and -0.4\%, arbitrary but negligible.



%\subsection{Forces and Moment over Lower Surface}
%Looking at the integrated force from $x_1=0.104~\text{m}$, the plots resemble the full forces but at slightly lower values, which means that the high pressure upstream of the jet does not have dominated influence on the whole model lower surface. The relative difference caused by the incorporation of turbulence model expands to 122.2\%, 112.9\%, 100.4\% for $F104x_1$, and 4.8\%, 9.2\%, 10.5\% for $F104x_2$, with $\text{PR}=1.5, 2.5, 3.5$. But for no jet case, relative difference for $F104x_1$ increased to 0.1\%, and for $F104x_2$ reduced further to 0.001\%. This is obviously due to that the viscous friction increases as turbulence generates along the surface, while the turbulence influence on vertical force is biased around the nose-tip after the leading shock. 

%The moment of $Fx_2$ with respect to the center of jet exit $Mjx_3$ is also calculated, since in many engineering scenarios, the lateral jet is placed with its axis aligned with the vehicle center of mass. And the jet induced extra force and moment act as unwanted disturbance. The results of such moment $Mjx_3$ is naturally lower than the $Mx_3$, while the distribution still follows the pattern of $Mx_3$. The relative difference for such moment is then 3.7\%, 9.7\%, 12.0\% for the three jet pressure ratios (discrepancy for no jet case is still very much ignorable). It is obvious that the gap of $Mjx_3$ between the two solvers is getting more significant than $Mx_3$ at corresponding $\text{PR}$.

%When the independent variable changes from $\text{PR}$ into angle of attack, it is observed that the distribution of $F104x_1$, $F104x_2$ and $Mjx_3$ closely follow the pattern of the full forces and moment as shown in middle figure of the first row. The differences between the GSIS-SST and GSIS for $F104x_1$ are 11.0\% (0°), 14.2\% (15°) and 7.5\% (30°). It is again larger than that for $Fx_1$, but the extent of increment is much smaller compared to that at 70~km (21.2\% to 112.9\%). For $F104x_2$, the difference are 0.8\%, 0.5\% and -0.1\%, such simple decreasing trend is different from that of the full $Fx_2$. And the difference in $Mjx_3$ takes a similar trend as $Mx_3$, from 0.8\% to 0.1\% and -0.5\%, a linear relation.

%For higher altitude of 90~km and 100~km, things are similar as that with full forces and moment.

% \subsection{Force and Moment Augmentation Factors}
% Another key aspect which the aerospace engineers interest of is the force and moment augmentation factor $K$. It is defined as follows:
% \begin{equation}
% K=\frac{FM_{Wall,jet on}+FM_{jet}-FM_{Wall, jet off}}{FM_{jet}},
% \end{equation}
% here, quantity $FM$ could either be force or moment. %In this study, the force and moment here are only about the vertical force $Fx_2$, since the jet is placed also vertically and the lower surface is horizontal. The moments analyzed are in $x_3$ direction with two distinct centers of moment. The first one is a pitch moment (relative to nose-tip) serving for attitude adjustment (installment of the jet not aligning with vehicle center of mass), the second one is calculated to display the jet induced disturbance on attitude stabilization during orbital maneuver (jet exhausting axis crossing the center of mass). An interaction moment coefficient $Cim$ is defined as below to quantify the deviation of pitch moment from trimming condition caused by the jet. The results are plotted in the second column of figure~\ref{fig:FM}.
% In this study, we focus on the forces and moments generated by the lateral jet, primarily the vertical force $Fx_2$ and the moment $Mx_3$, which are critical for attitude control and stabilization. The pitch moment is evaluated relative to two reference points: the nose-tip, representing attitude adjustment, and the center of mass, reflecting disturbances during orbital maneuvers. To quantify deviations from trimming conditions caused by the jet, we define the interaction moment coefficient $Cim$ as follows:
% \begin{equation}
% Cim=\frac{M_{Wall,jet on}-M_{Wall, jet off}}{M_{Wall, jet off}},
% \end{equation}
% The results for $K_{Fx2}$, $K_{Mx3}$, and $Cim$ are summarized in Table~\ref{tab:ForceMoment} and plotted in Figure~\ref{fig:FM}.

% %From the aspect of variation in flight altitude, the force augmentation factor $K_{Fx2}$ from GSIS slightly increases from 4.64 (65~km) and 4.56 (70~km) to 4.65 (75~km) and 5.20 (80~km), while GSIS-SST predicts a convex curve over the GSIS one with the minimum reaching 4.90 at 75~km, and 6\% to 28\% higher than the GSIS ones. 

% %The $K_{Mx3}$ from GSIS is also non-linear, and favor the altitude of 80~km, while the GSIS-SST instead predicts basically a decreasing and toward GSIS converging trend, therefore the plot is again convex. The discrepancy between the two solutions on $K_{Mx3}$ comes larger than the $K_{Fx2}$, arriving 43\% at 65~km and remaining 8.2\% at 75~km. 
% The augmentation factor for the vertical force, $K_{Fx2}$, shows a generally increasing trend with altitude. For GSIS, $K_{Fx2}$ rises from 4.56 at 65km to 5.20 at 80km, while GSIS-SST predicts a convex trend, peaking at 75km with a value 28\% higher than GSIS at this altitude. The moment augmentation factor $K_{Mx3}$, however, exhibits non-linear behavior. GSIS results favor higher altitudes, while GSIS-SST trends towards GSIS as altitude increases, with discrepancies reaching 43\% at 65km and narrowing to 8.2\% at 75~km.

% %The coefficient $Cim$ from GSIS stays around 0.35 at all altitudes, while a decreasing pattern is observed for GSIS-SST. The GSIS-SST $Cim$ is 55\% higher at 65~km and only 0.2\% higher at 80~km. Thus, the turbulence impacts the attitude stabilization more than maneuver, especially at lower altitudes, posing greater challenge to flight control systems.
% The interaction moment coefficient $Cim$ remains around 0.35 across altitudes for GSIS, while GSIS-SST shows a decreasing trend, with differences as high as 55\% at 65km and diminishing to 0.2\% at 80km. These results suggest that turbulence effects, captured by GSIS-SST, exert stronger influence at lower altitudes, posing greater challenges for flight control systems due to increased destabilizing moments.
%as the rarefied environment reduces the intensity of jet and free flow interaction. 
%from both GSIS-SST and GSIS resemble the $K_{Mx3}$, with the exception of 65 to 70~km from GSIS, in which the minimum of the curve falls around 70~km (for $K_{Mx3}$ it is 65~km). The differences between GSIS-SST and GSIS regarding $Cim$ are enhanced.
%The difference between the two solvers roots completely at 70~km. Also a interesting point to be noticed is that, $K_{Fx2}$ from 70~km and 80~km takes very similar value, and $K_{Mx3}$ are exactly the same at these two altitudes. 

%Observing the change of augmentation factors with varying pressure ratio, it is seen that the augmentation factor falls with increasing $\text{PR}$, while the relative difference between the two solvers reaches the maximum at $\text{PR}=2.5$ of 16.1\% (13.5\% at 3.5), while only 11\% at lowest pressure ratio. The moment augmentation factor $K_{Mx3}$ agrees with the pattern of $K_{Fx2}$, with a maximum value of 14.7 (GSIS-SST) and 12.8 (GSIS) at $\text{PR}=1.5$ and a maximum overshoot from GSIS-SST of 28.1\% at $\text{PR}=2.5$. It is noticed also that the $K_{Mx3}$ difference reaches to 27.9\% closely to maximum at $\text{PR}=3.5$, it seems that the difference in augmentation factor saturates as pressure ratio increases. The possible reason could be that with too high a pressure ratio, the length of the model is not long enough to capture the whole influence of the jet. The $Cim$ behaves in contrast near linearly with increasing pressure ratio, while the relative difference between GSIS-SST and GSIS shows an decelerated increasing trend. This is due to the fact that the aerodynamic center in GSIS is closer to the jet exit with larger $\text{PR}$, while the GSIS-SST shifts the aerodynamic center away from the jet exit, enlarging the arm of force. Such complex interplay shapes thus the obscured turbulence influence on $Cim$.

% Both $K_{Fx2}$ and $K_{Mx3}$ decrease with increasing pressure ratio $\text{PR}$, reflecting a weakening influence of the lateral jet as $\text{PR}$ rises. For $K_{Fx2}$, the relative difference between GSIS-SST and GSIS reaches a peak of 16.1\% at $\text{PR}=2.5$, while for $K_{Mx3}$, the maximum overshoot is 28.1\% at the same pressure ratio. Notably, discrepancies in $K_{Mx3}$ remain significant at higher pressure ratios, reaching 27.9\% at $\text{PR}=3.5$. This saturation in augmentation factor differences may be attributed to insufficient model length to fully capture jet-induced effects at high $\text{PR}$.

% The interaction moment coefficient $Cim$ increases almost linearly with $\text{PR}$, with the relative difference between GSIS-SST and GSIS decelerating as $\text{PR}$ grows. This behavior is linked to a shift in the aerodynamic center: GSIS places it closer to the jet exit at higher $\text{PR}$, while GSIS-SST predicts a shift away from the jet exit, amplifying the lever arm and consequently the moment.

%The influence of angle of attack (AoA) is interwoven with $\text{PR}$ effects. For example, at 80~km, augmentation factors display non-linear behavior with AoA, but the percentage differences between GSIS-SST and GSIS remain minor, typically under 4\%. This suggests an indirect relationship between turbulence and AoA in shaping the augmentation factors, primarily mediated by changes in flow alignment and jet penetration. Given the limited impact, these results are included here for completeness.

%Augmentation factors for 80~km with variation in AoA is non-linear, but due to the small percentage difference, the relations between turbulence influence and angle of attack on augmentation factors remain indirect, thus we only illustrate the results here for completeness.
%The interplay between altitude, pressure ratio, and angle of attack reveals distinct turbulence effects captured by GSIS-SST, with significant implications for both attitude control and stabilization. At lower altitudes and moderate $\text{PR}$, turbulence exacerbates destabilizing moments, demanding advanced control strategies. At higher altitudes or extreme $\text{PR}$, differences between the solvers diminish, reflecting the adaptive nature of GSIS-SST in resolving turbulence. These findings underline the necessity of incorporating turbulence effects into aerodynamic design and control systems, particularly in hypersonic flight regimes.
%Finally, the $K_{Mjx3}$ has much lower values and an opposite trend with increasing $\text{PR}$. Its maximum value and relative difference both appear at $\text{PR}=3.5$ of 0.61 (GSIS-SST), 39.1\% higher than GSIS prediction. For pressure ratio of 2.5 and 1.5, $K_{Mjx3}$ is 0.49 (GSIS-SST) and 36.9\% higher, 3.03 (GSIS-SST) and 18.1\% larger than the GSIS one. The positive relation between the turbulence influence and pressure ratio is more apparent here.

%Augmentation factors for 80~km with variation in AoA is clearly non-linear. The $K_{Fx2}$ climbs from 4.35 (GSIS-SST) to around 5.2, with the maximum appears at AoA=15° of 5.24 (GSIS-SST). The differences between GSIS-SST and GSIS are insignificant, but seems random, i.e., 0.1\% 0.8\% and -0.8\% with increasing AoA. The moment augmentation factor $K_{Mx3}$ falls between 10 and 14, with the maximum also lies on AoA=15° of 13.7 (GSIS-SST). The discrepancy between the two solvers stands out as -3.7\% at AoA=30°, whilev it is less than 1\% (Absolute value) at the other AoA. For $K_{Mjx3}$, it is rather small and is decreasing substantially with increasing angle of attack. It is 1.76, 0.40 and 0.082 from GSIS-SST, and 1.1\%, 0.2\%, -6.4\% larger than from GSIS. 


%\subsection{Lift and Drag}
%\leib{If transform the forces (apart from the jet thrust) further into lift and drag, the influence from turbulence is weakened, as these forces are the angle of attack dependent combination of the smaller but turbulence more relevant axial force $Fx_1$ and the larger but turbulence less influenced normal force $Fx_2$. 

%It could be noticed that the lift and drag curves look the same as $Fx_{1}$ and $Fx_{2}$, but the relative differences between the GSIS-SST and GSIS for lift and drag are averaged, for instance 13\% for lift and 14\% for drag at 65~km. Such differences decrease as flight altitude increases. For the L/D ratio, a decreasing aerodynamic performance is observed. The application of lateral jet increases the L/D by at least 71\% (GSIS-SST at 65~km). The L/D around 3.4 (GSIS) at 65~km falls all the way down to 2.95 (GSIS) at 80~km. It is apparent that the GSIS-SST constantly produces a less L/D within acceptable deviation of around 2\%. This observation suggests that the turbulence influence affects more the force and moments, i.e., propulsion and flight control system, while may not become problems for the design of ballistic and overall aerodynamic configuration.

%When the forces (excluding jet thrust) are transformed into lift and drag, the turbulence influence diminishes. This reduction occurs because lift and drag represent angle-of-attack-dependent combinations of the turbulence-sensitive axial force ($Fx_1$) and the less turbulence-influenced normal force ($Fx_{2}$). Consequently, lift and drag exhibit similar trends to $Fx_{1}$ and $Fx_{2}$, but the relative differences between GSIS-SST and GSIS are averaged. For example, at 65~km, these differences are approximately 13\% for lift and 14\% for drag, with a decreasing trend at higher altitudes.

% The lift-to-drag ratio (L/D) reveals a declining aerodynamic performance with increasing altitude. The application of the lateral jet enhances the L/D by at least 71\% (GSIS-SST at 65km), increasing from 3.4 (GSIS at 65km) to 2.95 (GSIS at 80~km). Across all conditions, GSIS-SST consistently predicts a slightly lower L/D, with deviations from GSIS around 2\%, indicating that turbulence influences are more critical for force and moment predictions (propulsion and flight control) than for the overall aerodynamic performance or vehicle configuration.

%The detailed values of lift and drag for various pressure ratios are not elaborated here. For the jet cases, differences of lift and drag from GSIS-SST relative to GSIS are 3.5\% and 6.6\% at $\text{PR}=1.5$, 7.0\% and 8.7\% at 2.5, 6.9\% and 8.2\% at 3.5, clearly peaks at $\text{PR}=2.5$, the reason behind this is probably about the length of the model again. Meanwhile, the Lift-Drag-Ratio (L/D) increases from 1.9 with no jet, to 3.09 ($\text{PR}=1.5$), 3.23 ($\text{PR}=2.5$) and 3.31 ($\text{PR}=3.5$) from GSIS-SST, exhibiting an expected positive trend. The differences in L/D relative to GSIS reveals itself more at lower $\text{PR}$ values, and follows a monotonic diminishing trend with variation in $\text{PR}$. It can be seen that the differences of force reach maximum at $\text{PR}=2.5$, while the difference for L/D follows. 

% With varying pressure ratios ($\text{PR}$), the differences in lift and drag between GSIS-SST and GSIS reach their peak at $\text{PR}=2.5$, with discrepancies of 3.5\% and 6.6\% at $\text{PR}=1.5$, increasing to 7.0\% and 8.7\% at $\text{PR}=2.5$, and slightly decreasing to 6.9\% and 8.2\% at $\text{PR}=3.5$. This peak discrepancy may result from the limited length of the model, affecting the jet-induced flow field. The L/D ratio exhibits a steady increase with $\text{PR}$, from 1.9 (no jet) to 3.09 ($\text{PR}=1.5$), 3.23 ($\text{PR}=2.5$), and 3.31 ($\text{PR}=3.5$), as predicted by GSIS-SST. Differences in L/D relative to GSIS are more pronounced at lower $\text{PR}$ and diminish monotonically as $\text{PR}$ increases, aligning with trends in force discrepancies.

%For the influence of angle of attack, though the results from both solvers at flight altitude 80~km do not deviate from each other significantly, the underlying mechanism could still be observed. Since only the lower surface is considered and a vertical jet exists, L/D naturally peaks at AoA=0°, whereas for real vehicle the maximum appears at a positive AoA. As analyzed previously, turbulence diffusion works best when there is space for it to progress. Difference from turbulence concentrates on the drag force at low AoAs, and subsequently impacts the L/D ratio. In contrast, lift experiences no sensible changes with different solvers.
%When the flight altitude reaches 80~km, lift force increases significantly from around 48 to 117 and 238, while the drag also increases from around 3 to 40 and 152. The relative difference for lift is trivial, yet for drag 3.92\% exists between GSIS-SST over GSIS at AoA=0°, but the difference diminishes quickly with increasing angle of attack. The L/D also decreases significantly with AoA, since only the lower surface is considered, and thus AoA=0° enjoys the largest ratio of 16.2 from GSIS-SST and 16.82 from GSIS (a -3.68\% difference due to deviation in drag). The reason behind the observation is that as AoA increases, contribution from pressure on lift and drag dominates, thus the turbulence influence in the form of viscous shear stress is outweighed.

%For higher altitude, Lift and drag continue climb, but the L/D decreases. The difference between the two solvers also approaches values below 0.1\%.
% The influence of angle of attack (AoA) becomes apparent when considering flight at 80~km. Though GSIS and GSIS-SST results show minimal deviations, the underlying turbulence mechanisms are discernible. The L/D ratio naturally peaks at AoA´0° for the simplified lower surface with a vertical jet, whereas real vehicles exhibit maximum L/D at positive AoA. Turbulence effects primarily affect drag at low AoA, subtly reducing L/D. In contrast, lift remains nearly identical between the solvers, highlighting the limited impact of turbulence on lift under these conditions.

% Overall, large deviations between GSIS-SST and GSIS are most likely to appear in cases with small pressure ratios and angles of attack at lower altitudes.}

\section{Conclusions}\label{sec:conclusion}

We have analyzed the lateral turbulent jet interactions in rarefied flow regime using the multiscale GSIS-SST method. Key findings are summarized as follows:
\leib{
\begin{itemize}    
    \item \textbf{Complex relationship between pressure ratio and turbulent effects}: The relationship between the pressure ratio PR and the turbulence-induced variations in shear stress and heat flux is inherently intricate, shaped by alterations in flow structures, turbulence dynamics, boundary layer interactions, and shock effects. As PR escalates, the jet's momentum and its ability to penetrate the surrounding flow increase, resulting in the emergence of more complex flow structures, such as intensified shock waves and expanded separation regions. While the discrepancies between the GSIS-SST and GSIS models become more evident in the near-wall layers, the influence of turbulence on shear stress and heat flux does not adhere strictly to a uniform pattern as PR fluctuates. 
    Instead, there exists roughly positive relations for properties include point-to-point shear stress and the heat flux, vertical force and moments of vertical force, force and moment augmentation factors with an increasing PR, also roughly negative relations for properties such as integrate horizontal force, Lift-to-Drag ratio. It is the results at $\text{PR}=2.5$ that always makes theses patterns less distinct by giving a more or less similar influence as at higher PR of 3.5. Thus, a critical point might exit where the impact of turbulence on aerodynamic forces and heat transfer is most pronounced and significant. It is then imperative to acknowledge and account for the effects of turbulence in pertinent research endeavors to accurately forecast the aerodynamic performance and thermal management strategies of hypersonic vehicles.
    
    \item \textbf{Positive impact of AoA on turbulence in local structures}: The AoA substantially affects the lateral interactions of the jet flow. With an increasing AoA, the penetration of the jet diminishes, leading to a more constrained flow field and the emergence of more intense shock and separation structures. Turbulence generation is enhanced around most of the shock structures. The vortex is jet flow area experiences an increasingly stronger stretching and production of turbulent kinetic energy when AoA increases. Influence from turbulence on all the moment augmentation factors enjoys also a positive relation with AoA, pointing out the shift of aerodynamic center under turbulence. Yet, the turbulence influence on integrated force and L/D generally diminishes, as lower AoA provides favorable environment for turbulent related diffusion and mixing process, while at larger AoA convection related process dominates as interaction intensifies.
    %The divergence between the GSIS-SST and GSIS models becomes more pronounced at larger AoA, signifying a more substantial impact of turbulence on the flow field and surface parameters. 
    These observations underscore the critical necessity of accurately modeling turbulence to effectively capture these effects in hypersonic applications.    
    
    %\item \textbf{Diminished turbulent effect}: In rarefied environments, the influence of turbulence is attenuated due to the low-density conditions and the unique characteristics of the jet flow. At the altitude above 80 km, the role of turbulence becomes minimal. Simultaneously, rarefaction effects intensify with increasing flight altitude, resulting in more dispersed shock structures and potentially causing jet flow features to become altered or even vanish. The GSIS-SST model is effectively the GSIS model for rarefied gas dynamics. Additionally, on the integrated force, moments and their augmentation factors, the GSIS-SST provides usually a more consistent monotonic or smoother trend.

    \item \textbf{Necessity of turbulence consideration in jet application}: Turbulence influence on aerodynamic performance indicators such as lift, drag positively and their ratio negatively with variation in pressure ratio, angle of attack. Smaller PR reduces penetration height and impacts surface friction more intensively, smaller angle of attack provides room for turbulence influence to take effect on drag, and L/D is more sensitive to AoA rather than PR changes (at AoA=15°). For nominal $\text{PR}=2.5$ and AoA=15°, though the turbulence effect diminishes with increased flight altitude and gas rarefaction level, a turbulence auto adaption method should be considered to avoid potential overestimation of L/D by laminar methods.
    The interplay between altitude, pressure ratio, and angle of attack reveals distinct turbulence effects captured by GSIS-SST, with significant implications for both attitude control and stabilization. At lower altitudes and moderate $\text{PR}$, turbulence exacerbates destabilizing moments, demanding advanced control strategies. At higher altitudes or extreme $\text{PR}$, differences between the solvers diminish, reflecting the adaptive nature of GSIS-SST in resolving turbulence. These findings underline the necessity of incorporating turbulence effects into aerodynamic design and control systems, particularly in hypersonic flight regimes.
    
\end{itemize}
}
Our findings provide new insights into the complex flow dynamics of jets in high-altitude applications. The results underscore the importance of considering both turbulent and rarefied effects in the development of jet-based control systems for hypersonic vehicles. With these insights and the robust numerical framework of GSIS-SST, future design and optimization of jet-based active flow control systems can be effectively pursued in flow regimes where conventional methods are inadequate.

%\leib{Limitations do exist, since the parameter space is not covered in finer grain and the model studied could be improved into a full-scale typical hypersonic flight vehicle. As the model has a long and flat low surface, transition model might improve the accuracy of results, even though the jet has been defined as developed turbulent flow. Our solver is also under development of integrating more sophisticated turbulence modeling strategy, and continuously working on the interaction between turbulent and rarefied flows.}


\section*{Acknowledgments} 
This work is supported by the National Natural Science Foundation of China (12450002) and the Stable Support Plan (80000900019910072348). %The authors thank Yanbing Zhang for his help with the GSIS code, and Quanhua Sun for the discussions on the laminar, turbulent and rarefied parts of shear stress and heat flux.

\section*{Declaration of interests} 
The authors report no conflict of interest.

\section*{Data availability}
The data that support the findings of this study are available from the corresponding author upon reasonable request. 

==> bk.tex <==

The persistent drive for increased velocity and enhanced maneuverability in hypersonic vehicles is transforming the landscape of aerospace technology. To accomplish high-speed, high-altitude maneuvers, these vehicles must contend with extreme conditions (e.g., diminished dynamic pressure and extreme aerodynamic heating) that outstrip the capabilities of conventional flight control systems. Active flow controls, such as lateral jets, have become a critical technology to mitigate the detrimental impacts of these extreme conditions and sustain control in hypersonic flights~\citep{Mahesh2013Interaction}.

At low altitudes, the Navier-Stokes (NS) equations are widely used to model the continuum gas flow. Turbulence is expected due to the high Reynolds numbers (Re), and the numerical methods such as Reynolds-Averaged Navier-Stokes (RANS)~\citep{Sanaka2024Re} method and large eddy simulations~\citep{Boles2010Large,Miller2018Transient} are used to resolve turbulence in the flow and capture the dynamic interaction between the jet and the free stream.

At high altitudes, rarefaction effects gain prominence as the Knudsen number (Kn) increases\footnote{The Knudsen number is defined as the mean free path of gas molecular over the characteristic length $L$. If the same length $L$ is used in the definition of the Reynolds number, then $\text{Kn}\propto\text{Ma}/\text{Re}$.}, which not only lead to velocity slip and temperature jump at solid walls but also alter the constitutive relations. Consequently, the continuum fluid hypothesis underlying the Navier-Stokes (NS) equations is no longer valid, necessitating the use of the Boltzmann equation. The Boltzmann equation, which is defined in the six-dimensional phase space, is solved by the direct simulation Monte Carlo (DSMC) method \citep{Bird1994Molecular, Boyd1995Predicting, Gimelshein2002Modeling} and the discrete velocity methods~\citep{Xu2010unified,Liu2024Further,Zhang2024Efficient}.

Theoretically, the Boltzmann equation provides an accurate model for dilute gas flows, spanning from the continuum to the free-molecular flow regimes. The Navier-Stokes (NS) equations, which are effective in the continuum flow regime where the Knudsen number is small, can be derived from the Boltzmann equation through the Chapman-Enskog expansion~\citep{Chapman1990Mathematical}. 
However, directly solving the Boltzmann equation for continuum flows, particularly in the presence of turbulence, is computationally intensive. For instance, simulating turbulent flow in the Taylor-Green vortex required over half a million cores for 500 hours~\citep{Gallis2017Molecular}. Despite the computational cost, there are certain researches trying to find turbulence in rarefied flows or vice versa, with kinetic solvers. Some notable attempts include \cite{Stefanov1993Monte}, they have conducted DSMC simulation on Taylor-Couette flows with Kn around $10^{-2}$ to study the Taylor instability, and have witnessed the transition of a new instability into chaotic dynamics, which was thought as a sign to turbulence. \cite{Komatsu2014glimpse} confirmed that the energy spectrum of freely decaying turbulence still follows Kolmogorov scaling with molecular dynamics simulation, even though the Kolmogorov scale is already the size of a few molecular diameter. 
The recently developed multiscale numerical methods can be faster than DSMC in the near-continuum flow simulations~\citep{Liu2020Unified,Wei2023Adaptive,Su2020Can,Zhang2024Efficient}, however, there is no report proving their efficiency in simulating turbulence flow. Relevant studies include: \cite{Li2018Thermal} deterministically solved the Boltzmann equations for simulation of the decaying isotropic turbulence with small scale thermal-non-equilibrium (TNE) effect, and discovered that those small scale TNE is able to alter the energy decay exponent up to 10\%. A first attempt to study three-dimensional compressible isotropic turbulence with Boltzmann based mesoscopic solver has been reported by \cite{Chen2022Simulation}.
Despite these findings of interaction between the large scale turbulence and the small scale rarefaction induced non-equilibrium or proofs of turbulence simulating ability with Boltzmann equations, the published efforts in ideal scenarios do not provide significant macroscopic alternations that worth engineering attention. 

Due to the limitation of Boltzmann equation in continuum application and NS equations in continuum breakdown, existing study on lateral jets  
Despite the inclusion of NS equations in Boltzmann equation, the continuum and kinetic solvers remain independent and dominant in their own advantageous regimes. Problem setups in existing studies also bias toward the numerical methods applied, i.e. continuum flows with higher density jets~\citep{Viti2004Jet,Rowton2024ANumerical} or rarefied flows with lower density jets~\citep{Gimelshein2002Modeling,Zhuang2022Effectiveness,Karpuzcu2023Study}, whereas only a few of them has considered the emerging scenario involving both rarefied flows and higher density jets~\citep{Zhao2023Numerical}, not to say further consideration of potential turbulence associated with the jet. 

While existing methods—whether based on continuum solvers like RANS or kinetic solvers like DSMC—have provided valuable insights into different aspects of hypersonic flow, they each face significant limitations when both turbulence and rarefaction effects are present simultaneously. Continuum solvers struggle to account for rarefaction at high altitudes, and kinetic solvers face prohibitive computational costs when turbulence is involved. To overcome these challenges, we introduce a novel approach: the GSIS-SST solver~\citep{Tian2024Multiscale}. This multiscale solver integrates the General Synthetic Iterative Scheme (GSIS), a kinetic solver designed for rarefied flows, with the turbulence modeling capabilities of the $k$-$\omega$ SST model, enabling it to resolve both turbulence and rarefaction in a unified framework. The GSIS method provides fast convergence and asymptotic-preserving properties, allowing for efficient solutions on coarse grids, while the SST turbulence model captures turbulent effects and alleviates the stringent grid resolution requirements of traditional direct numerical simulation (DNS) methods. Together, these models enable accurate simulation of flows across a wide range of regimes, from free-molecular to turbulent continuum.

By leveraging the GSIS-SST solver, this study investigates the interaction between lateral turbulent jets and rarefied hypersonic flows. We focus on key flow structures, including jet penetration, shock formation, and vortex dynamics, as well as important surface quantities like shear stress and heat flux. The findings provide new insights into the combined effects of rarefaction, non-equilibrium dynamics, and jet-induced turbulence, offering valuable guidance for the design and optimization of jet-based active flow control systems for hypersonic vehicles.

%There is also general synthetic iteration scheme (GSIS) \cite{Su2020Can,Su2020Fast}, which differs from above methods by its inclusion of a macroscopic solver. These methods bring a more suitable description of flows in transition regime and usually have the asymptotic behavior of returning to the NS solution at extreme conditions. They have also relaxed the spatial and temporal discretization requirements for multiscale flow problems and achieved good results in many engineering applications. Recently are there studies on lateral jet in rarefied flow \cite{Zeng2023Computational,Zhao2023Numerical}.  Yet the computational demands still render it inefficient for high-density or turbulent problems.

%Yet, they still lack practical means to tackle engineering turbulence problems due to the absence of turbulence modelling method within the gas kinetic theory. Pioneering studies do exist, studies using UGKS or DUGKS for are attempting to create a new DNS path of solving turbulence problems with mesoscopic methodology based on gas kinetic theory (\cite{Cao2022High,Chen2022Simulation}). They are still a little bit far from application. 

%So there is a brand new problem which incorporates rarefaction effect, complex shock structure and also highly possibly turbulence effect, and there is no efficient and suitable tool to solve the problem properly. Taking the advantage of containing a macroscopic solver in GSIS, a method bridging widely-accepted RANS models with gas kinetic theory powered mesoscopic solver could be established. 

However, the interplay of turbulent and rarefaction effects, particularly in hypersonic conditions, still remain under-explored. In fact, there is no efficient tool to solve the problem properly, primarily due to the challenges posed by rarefaction effects which invalidate the continuum assumption used in the Navier-Stokes (NS) equations.  
Although recent research has shown the potential of DSMC to simulate turbulent flows \citep{Gallis2017Molecular,Gallis2019DSMC}, it demands huge and sometimes prohibitive computational resources to effectively tackle typical continuum jet problems.

%However, the interaction between lateral turbulent jets and rarefied environments has not yet been explored. This is due to the fact that the Boltzmann equation is defined in a six-dimensional phase space, necessitating fine spatial grids to capture turbulence and refined velocity grids to capture rarefaction effects. These requirements also present a substantial computational challenge that currently exceeds the capabilities of most computational resources, when both turbulent and rarefaction effects are taken into account.

%the flow regimes are then categorized based on the Kn, with Kn<0.001 being continuum regime, 0.001<Kn<0.1 the slip flow regime with emerging rarefaction effect, 0.1<Kn<10 the transition regime with significant rarefaction, and if Kn goes beyond 10, it is considered the free molecule flow. 
%Meanwhile, the Kn could be related to Re as: $\text{Re}\propto \text{Ma}/\text{Kn}$. It could be deduced then that for Kn>0.001, the Re will be too low to support persistent turbulence. Therefore, relevant researches targeting high altitude application does not need to consider turbulence, and set up the problems clearly without turbulence, probably due to the inefficiency of kinetic solvers in modeling continuum. 



% Due to the rarefied environment, turbulence is normally out of consideration, since high Knudsen number is always associated with a low Re.
% In the kinetic solver, Boltzmann,  ...
% The rarefaction effects are characterized by the Knudsen number, which is defined as the ratio between the molecular mean free path $\lambda$ and the flow length $L$: 
% % \begin{equation}
% %     \text{Kn}=\frac{\lambda_{\infty}}{L}=\frac{\mu_{\infty}}{\rho_{\infty}L}\sqrt{\frac{\pi}{2RT_{\infty}}},
% % \end{equation}
% with $\lambda$ being the molecular mean free path, $R$ stands for the gas constant.
% The flow regimes and Kn ....
}  




% As a result, literature on this subject is quite limited and typically relies on the stochastic direct simulation Monte Carlo (DSMC) method, either on its own or in combination with NS solvers~\citep{Tartabini1995Direct,Gilmore1995Axisymmetric,Gimelshein2002Modeling,Liang2014DSMC,Ding2019DSMC,Virgile2022Optimisation,Zhuang2022Effectiveness,Karpuzcu2023Study}.


% Although lateral jets have been widely studied in continuum and vacuum regimes by respectively the continuum and kinetic solvers~\citep{Brandeis1998Experimental,Graham2002Numerical,Chen2014Flow,Adeli2015Side,Cai2022Review}, 
%The interplay of a sonic lateral jet with the incoming rarefied gas flow near a sharp leading edge is considered. This setup simulates the cold jet-based attitude control system for hypersonic vehicles. The exit temperature of the jet is 250 K. The central axis of the jet nozzle is positioned 0.102 m from the nose-tip. The diameter of the jet nozzle is 0.004 m. 

%The jet is sourced from a pressurized nitrogen tank, which is characterized by the jet pressure ratio (PR). This ratio represents the ratio of the total pressure between the jet and the free flow after the normal shock has occurred, where the total pressure of free flow after normal shock is obtained with the normal shock relation \citep{Tian2024multiscale}.
% At an altitude of 70 km, a $\text{PR}$ of 2.5 signifies that the jet exit pressure is approximately 1,000 times greater than that of the ambient free stream pressure.

%The jet is assumed to have a have a higher turbulence intensity of $I_t = 3\%$, and a characteristic
%length-scale $l_t =\sqrt{\pi R^2_j}$ (non-dimensionalized with reference length) is assigned to the jet. The turbulence kinetic energy $k$ and specific dissipation rate $\omega$ are calculated as  $k=1.5(I_t \Vert \bm{u} \Vert)^2$ and $\omega=\sqrt{k}/l_t$.

%As can be seen in the previous subsection, the rarefied hypersonic flow field with turbulent lateral jet is plenty of shocks, shear, expansion and separation regions. The associated localized non-equilibrium and rarefaction, as well as turbulence, could impact the flow field and the derived aerodynamic performance parameters significantly. Conventional continuum or rarefied solvers are not able to take account of all these phenomena simultaneously, while the GSIS-SST is specifically tailored for such complex problems.
The rarefied hypersonic flow field with a turbulent lateral jet features an intricate interplay of shocks, shear layers, expansion zones, and separation regions. These phenomena, coupled with localized non-equilibrium effects, rarefaction, and turbulence, significantly influence the flow field and the resulting aerodynamic performance. Conventional continuum or rarefied solvers are unable to simultaneously account for all these complexities. The GSIS-SST method, specifically designed for such multiscale problems, addresses this gap effectively.

% To show the superiority of GSIS-SST, we take conventional Navier-Stokes solver (a two temperature NS model, denoted as NS solver), NS solver with the same turbulence model (NS-SST) and baseline GSIS as reference, and use the sensible and attitude control related aerodynamic parameter, the pitch moment, to analyze the asymptotic behavior among the solvers (note the contribution from jet thrust is excluded since it is the same for all solvers). The flight angle of attack and jet pressure ratio are still 15° and 2.5, and the free stream Mach number is 25.
To demonstrate the capabilities of GSIS-SST, its results are compared against those from a conventional two-temperature Navier-Stokes (NS) solver, an NS solver with the same turbulence model (NS-SST), and the baseline GSIS solver. Pitch moment, a parameter critical for attitude control, is used as the primary metric for this analysis, excluding contributions from jet thrust, as these remain consistent across all solvers. The comparisons are conducted under a flight angle of attack of 15°, a jet pressure ratio (PR) of 2.5, and a free-stream Mach number of 25.
%In this part, the asymptotic behavior of GSIS-SST is exhibited, to identify the most suitable range of GSIS-SST application, i.e., when to use a method with contributions from both higher order information and turbulence consideration. We use the sensible aerodynamic index, the pitch moment, to compare the different solvers, including NS-SST (two temperature NS solver with $k=\omega$ SST turbulence model) and GSIS. The flight altitude is further decreased down to 30~km, with Mach number slightly reduced to 20, out of the consideration of real flight needs. The flight angle of attack and jet pressure ratio are still 15° and 2.5.

%Peek at the trend across altitude 65~km to 80~km (figure~\ref{fig:FM}), the pattern of change between altitude and the forces and moments could be noticed, with AoA=15° and $\text{PR}=0, 2.5$ (also remember that the forces and moment are in non-dimensional form). Forces and moment increases as the model flies higher. When the jet is off,  $Fx_1$ and $Mx_{3}$ (as well as $Mjx_{3}$) increase in a faster pace than $Fx_{2}$, which scales linearly with altitude. GSIS-SST converges to GSIS at all altitudes when there is no jet. 
% Figure~\ref{fig:Mx3}(a) depicts results from 30~km to 80~km. There are four curves in the figure, each represents the result from conventional NS solver, NS-SST, GSIS and GSIS-SST.

% The NS curve tells that the moment increases as flight altitude gets higher. The NS-SST curve, in contrast, follows a slight increasing trend at altitude below 50~km, and gradually decreases until 75~km, finally rises again and converges with the NS curve.
% The GSIS curve seems similar as the NS one, yet always with a positive offset. Meanwhile, the GSIS-SST curve exhibits a similar shape as the NS-SST curve, but has a more apparent increasing trend below 60~km, then stagnates around 60~km to 65~km. After a slight decrease at 70~km, the GSIS-SST curve rises again and catches the GSIS one at 80~km.
Figure~\ref{fig:Mx3}(a) presents the pitch moment results from 30~km to 100~km for the conventional NS solver, NS-SST, GSIS, and GSIS-SST. The NS curve shows a steady increase in moment with altitude. In contrast, the NS-SST curve rises slightly below 60~km, then gradually decreases until 75~km, where it converges with the NS curve. The GSIS curve displays a similar trend to the NS curve but is consistently offset positively. The GSIS-SST curve closely follows the NS-SST pattern, with a more prominent increase below 60~km, a plateau from 60~km to 65~km, a slight decrease at 70~km, and eventual convergence with the GSIS curve at 80~km.

% Three clear converging points and an additional converging trend could be read. 
% On the direction of decreasing altitude, the GSIS-SST curve converges with the NS-SST one at 30~km, while the discrepancy increases steadily on the direction of increasing flight altitude. The GSIS-SST curve thus shares the same pattern as the NS-SST one. 
% The GSIS-SST one converges with the GSIS one at 80~km, signaling the diminish of jet turbulence at current pressure ratio when the altitude is too high. This also confirms again the adaptive nature of GSIS-SST on applying the turbulence model, i.e., automatically cancels the modeled turbulence viscosity at low density and smooth flow fields.
% Also the NS-SST converges with NS curve at high altitudes, they start to approach each other at as low as 60~km.
% And the GSIS curve seems on the way of reaching the NS curve at low altitudes. The exact asymptotic property has been validated in \cite{Su2020Fast} mathematically and in \cite{Tian2024multiscale} for hypersonic boundary layer. Yet, for the complex jet interaction flow field, they have failed to reach a stable solution.

% Among these curves, the NS-SST one best fits the design purpose of the jet with $\text{PR}$, as it produces a rather constant moment from 30~km to 60~km. This is also due to the fact the the $\text{PR}$ is discovered based on theoretical, numerical and experimental analysis in continuum environment, for stable active flow control purpose. The cutoff of NS and GSIS curves below 50~km is due to hard convergence of these solvers, since the free stream environment has increased Re value, which means the flow instability is easily triggered and the modeling of turbulence is getting essential.
Three distinct convergence behaviors are observed. First, the GSIS-SST curve aligns with the NS-SST curve at 30~km, but their divergence grows with altitude, emphasizing the influence of turbulence and rarefaction. Second, the GSIS-SST and GSIS curves converge at 80~km, reflecting the diminishing effect of jet turbulence in low-density conditions and demonstrating GSIS-SST's adaptive ability to suppress turbulence modeling under such environments. Third, the NS-SST and NS curves converge above 60~km, as rarefaction reduces turbulence effects. The GSIS curve also trends toward the NS curve at lower altitudes. Though this behavior in jet interaction flows is limited by solver convergence issues, mathematical proof and validation in simpler hypersonic flows \citep{Su2020Fast, Tian2024multiscale} have confirmed the asymptotic properties of these solvers.
%though obtaining reliable solutions in jet interaction flows remain challenging.

The NS-SST curve is the most aligned with the design objectives of $\text{PR}=2.5$, maintaining a nearly constant pitch moment from 30~km to 60~km, a critical feature for stable active flow control. The cutoff in NS and GSIS results below 50~km arises from solver instability at higher Reynolds numbers, where turbulence modeling becomes essential to address flow instability.
%A clear converging trend between GSIS-SST and NS-SST (red curves) could be noticed at first glance. Whereas the solvers without turbulence consideration also tend to converge at lower altitude, yet they face difficulty in convergence during iteration at 30~km, thus no result is shown.

%shows the results of Mach number 25 cases, which include flight altitude of 65~km, 70~km, 75~km and 80~km. As the flight altitude is getting higher, it is unnecessary to consider conventional NS/NS-SST solvers. What is clear is that the pitch moment $Mx_3$ from GSIS increases with altitude, while the GSIS-SST prediction stays around 44 from 65~km to 75~km, then increases to 47 at 80~km. The difference between GSIS-SST and GSIS decreases as flight altitude rises.
Figure~\ref{fig:Mx3}(b) highlights the relative differences in pitch moment among the solvers. The GSIS-SST and NS-SST discrepancies, shown by the solid orange line, increase from 0\% at 30~km to 20\% at 80~km, reflecting the growing impact of gas rarefaction. The dashed orange line compares GSIS and NS, showing larger discrepancies that also grow with altitude but are constrained by solver limitations. The solid blue line compares GSIS-SST and GSIS, displaying a decreasing trend that approaches zero since 80~km.
% Figure~\ref{fig:Mx3}(b) summarizes the relative difference of pitch moments among the solvers. The solid orange line compares the GSIS-SST results relative to NS-SST ones. It is apparent that the discrepancy between the solver rises with an accelerated pace as flight altitude increases, from 0\% at 30~km to 10\% at 70~km. The dashed orange line gives the relative difference between GSIS and NS, such difference is even larger than the SST pair, also increasing under higher altitudes. But this curve is limited in range since both solvers exhibit shortage in certain altitude range. The solid blue gives the comparison between GSIS-SST and GSIS. It shows a decreasing trend with the rise of altitude, and stays close to 0 above 80~km. 
% It could be deducted from the results that higher Mach number tends to increase the discrepancy between the two solvers, and the two solvers still converge to each other at higher altitude, i.e., 80~km with current jet condition.

The two SST curves also reveal more information on the interaction between turbulence and gas rarefaction. Turbulence offsets the prediction on pitch moment positively and constantly, but the effect diminishes as flight altitude increases. However, the pitch moment from laminar solver predicts always an increasing trend. Thus, when the turbulence offset of NS-SST starts to disappear after 60~km, and the altitude effect does not increase the NS moment high enough over the NS-SST prediction, the NS-SST curve falls then to approach the NS one, and follows the laminar trend of increasing over 75~km. When it comes to the GSIS-SST curve, the inclusion of rarefaction effect shifts the GSIS-SST prediction upward from the NS-SST one over 30~km, and a near constant shift from GSIS due to turbulence. 
Also the discrepancy between GSIS-SST and NS-SST at 50~km is smaller than the GSIS/NS pair, while such discrepancy quickly reaches the discrepancy between the GSIS/NS pair over 60~km, as rarefaction intensifies, which implies that turbulence in continuum regime biased flow suppresses gas rarefaction effect. %there is direct interwoven between turbulence and rarefaction.
Therefore, due to the asynchronous change in turbulence and gas rarefaction effect, the GSIS-SST curve exhibits a strange disruption within 60~km to 80~km. 

These findings imply that the rarefaction effect in current scenario functions in a mechanism similarly for both the NS and Boltzmann based solvers, also rather independently from turbulence effect. It is highly possible that the rarefaction affects the outer rarefied flow field, while the turbulence influence impacts the inner jet flow field, and both alter the macroscopic flow structures, thus producing a solution with superimposed influence from both rarefaction and turbulence. This recognition will be displayed later in this paper.

The analysis confirms GSIS-SST's superior performance and adaptive behavior in rarefied hypersonic flows, as well as its asymptotic convergence to NS-SST in turbulence-dominated conditions and to GSIS in highly rarefied flows. In the subsequent paper, systematical investigation of jet pressure ratio, angle of attack, and altitude effects on aerodynamic performance are performed. Any discrepancies between GSIS-SST and GSIS results can be attributed to turbulence modeling, providing deeper insight into turbulent effects under varying flow conditions.
% The asymptotic behavior of GSIS-SST toward NS-SST is confirmed here, and GSIS-SST presents the most capable solving ability.
% In the subsequent paper, the solutions derived from GSIS-SST and GSIS concerning high altitude scenarios will be compared. The influences of the jet PRs, AoAs, and flight altitudes on the aerodynamics are systematically investigated. Should there be any discrepancies between the two sets of results, they can be attributed to the influence of turbulent effects. 
%through the trend of the curves, due to the existence of localized rarefaction effect and continuum breakdown, which is shock related and plentiful in the lateral jet flow field. Fortunately, the exact asymptotic behavior has been verified in our recent publication \leib{JFM accepted}.

%In the subsequent paper, the solutions derived from GSIS-SST and GSIS will be compared.% at altitudes exceeding 65 kilometers. 
%Should there be any discrepancies between the two sets of results, they can be attributed to the influence of turbulent effects.%, under rarefied environments.

%where the role of turbulence will be pinpointed by comparing the  GSIS-SST and GSIS results.
%Figure~\ref{fig:Geom} depicts the \leib{surface shear stress $\sigma_{12}$ on the lower surface, which clearly show that the coarse grid exhibits a slightly higher deviation from the fine grid around the upstream interaction region ($x_1\approx0.075~\text{m}$), whereas the moderate grid shows excellent agreement with the fine grid.} Consequently, the moderate grid %in Fig.~\ref{fig:Geom} is chosen for further calculations.


% \begin{figure}
% 	\centering
% 	\subfloat{}{\includegraphics[width=0.49\linewidth,trim={50 50 20 220}, clip]{Artworks/GeomPlate.png}}
%  \subfloat{}{\includegraphics[width=0.45\textwidth, trim={20 20 20 150}, clip]{Artworks/GridIndeSig12.png}}
% 	\caption{(a) Geometry of the sharp leading edge and spatial grid. The free flow boundary is indicated in red, the outflow boundary is marked in blue, the wall is colored green, and the jet, situated approximately at $x_1=0.1~\text{m}$, is highlighted in orange. \leib{The jet exit is allocated 30 nodes, with 84 nodes positioned before the jet and 120 nodes} after it on the lower horizontal surface. The height of the first grid layer is one micron. (b) \leib{Surface shear stress $\sigma_{12}$ from GSIS-SST in the grid independence study with PR=3.5}.
% }
% 	\label{fig:Geom}
% \end{figure}


%\subsection{Solution without Jet}

% \begin{figure}
% 	\centering
% 	\includegraphics[width=0.49\linewidth, trim={20 20 20 150}, clip]{Artworks/NJForce.png}
% 	\caption{
% 		Integrated forces \leib{and moments} on the lower surface of the model at various flight altitudes, in the absence of a jet. \leib{Moments here are taken with respect to the nose-tip $(x_1,x_2)=(0,0)$, positive means counter-clockwise rotation.}
% 	}
% 	\label{fig:NJForce}
% \end{figure}

%In our previous work\cite{Tian2024multiscale}, we have validated our approach with turbulent boundary layer at Mach number 9.22, and also flow around blunt leading edge across large range of Knudsen number at Mach number 25. The results reported there has proved the correctness and ability of the method to capture turbulence effect. It also hints that sensitive deviation appears from GSIS-SST to original GSIS starting from Kn=0.001. Here, in this study, we further validate the approach with no jet condition on the sharp leading edge model from altitude $70\sim100~\text{km}$ at AoA=15°, to obtain the information of influence from the implemented turbulence model. 
%
%The results on integrated forces are shown below in figure~\ref{fig:NJForce}. The plots of non-dimensional drag force $Fx_1$ from both GSIS and GSIS-SST increase in a quadratic manner as altitude rises, while the lift force $Fx_2$ from both solutions increases almost linearly. It is also clear that $Fx_1$ and $x_2$ from GSIS and GSIS-SST converges completely with each other at every altitude. Additionally, the more sensitive surface heat flux experiences good agreement between GSIS and GSIS-SST each boundary cell, with an relative error of far below 0.1\% for all altitudes investigated.
%
%Thus, it could be concluded here that in the altitude above 70~km, the free flow is essentially free from turbulence. 

%In our previous work\cite{Tian2024multiscale}, we have validated the GSIS-SST with a turbulent boundary layer at a Mach number of 9.22, as well as the flow around a blunt leading edge across a broad range of Knudsen numbers at a Mach number of 25. The results demonstrated the accuracy and capability of GSIS-SST in capturing turbulence effects, where the laminar solution of GSIS deviates sensitively to GSIS-SST at $\text{Kn} \lessapprox 0.001$. 

%We validate the GSIS-SST under no jet conditions on a sharp leading edge model from altitudes ranging from 65 to 100 km at AoA=15°. The axial force $Fx_1$, normal force $Fx_2$ and pitch moment $Mx_3$ (pointing outward of the paper, relative to the nose-tip) from GSIS and GSIS-SST are in complete agreement at every altitude. The sensitive surface heat flux also shows excellent agreement between GSIS and GSIS-SST at each location, with a relative error well below 0.2\% for all altitudes studied. Thus, it can be concluded that above an altitude of 65 km, the free stream is essentially free from turbulence. And the coupled SST turbulence model and the assumed free flow turbulence will not influence the solution. 
%The force integrated along the model's lower surface are presented in Fig.~\ref{fig:NJForce}. 
%The horizontal force $Fx_1$ obtained from both GSIS and GSIS-SST
%increases quadratically with altitude, while the vertical force $Fx_2$ \leib{and moment around nose-tip} increase almost linearly. It is evident that \leib{$Fx_1$, $Fx_2$ and $Mx_3$ (pointing outward of the paper)} from GSIS and GSIS-SST are in complete agreement at every altitude. Furthermore, the surface heat flux, which is more sensitive, shows excellent agreement between GSIS and GSIS-SST for each boundary cell, with a relative error well below 0.2\% for all altitudes studied. Thus, it can be concluded that above an altitude of 70 km, the free stream is essentially free from turbulence. And the coupled SST turbulence model and the assumed free flow turbulence will not influence the solution. 


\begin{table}
    \centering
    \begin{tabular}{cllcllcllll}\hline
         Altitude& AoA&PR&  SST& $Fx_1$&$Fx_2$&  $Mx_3$ &$Mjx_3$ &$K_{Fx2}$ & $K_{Mx3}$&$K_{Mjx3}$\\ \hline
         65 km & 15°&2.5&   0& 2.33&98.39&   32.33&22.29&4.64 & 10.68 &0.272 \\
 & & & 1& 3.05& 111.08& 36.95 &25.62&5.93 & 15.26 &0.367\\
 & & &RelDiff & 31.1\%& 12.9\% &14.3\% &14.9\% &27.7\% & 42.9\%&34.6\%\\ \hline

 70 km& 15°& 1.5& 0& 4.02& 93.57 & 31.30 &21.75&5.42 & 12.79 &0.204\\
 & & & 1& 4.99& 97.09 & 32.46 &22.56 &6.01 & 14.71 &0.233\\
 & & &RelDiff & 24.2\%& 3.8\% &3.7\% &3.7\% &11.0\% & 15.1\%&13.9\%\\

 & & 2.5& 0& 3.49& 102.50 & 33.96 &23.50 &4.56 & 10.72 &0.264\\
 & & & 1& 4.23& 109.74 & 36.99 &25.79 &5.29 & 13.72 & 0.329\\
 & & &RelDiff & 21.2\%& 7.1\% &8.9\% &9.7\% &16.1\% & 28.1\%&24.8\%\\

 & & 3.5& 0 & 3.09& 111.12 & 36.27 &24.93 &4.16 & 9.58 &0.306\\
 & & & 1& 3.71& 118.86 & 40.04 &27.92 &4.72 &12.26 &0.380\\
 & & &RelDiff & 20.1\%& 7.0\% &10.4\% &12.0\% &13.5\% & 27.9\% &24.2\%\\ \hline

 75 km& 15°& 2.5& 0 & 5.34& 110.07 & 36.98 &25.75 &4.65 &11.42 &0.265\\ 
& & & 1& 5.93& 112.60 & 37.93 &26.44 &4.90 & 12.36 &0.284\\
 & & &RelDiff & 11.1\%& 2.3\% &2.6\% &2.7\% &5.5\% & 8.2\% &7.2\%\\ \hline

 80 km& 0°& 2.5& 0 & 2.86& 48.03 & 15.41 &10.51 &4.34 & 10.98 &0.636\\ 
& & & 1& 2.97& 48.08 &15.49 &10.59 &4.35 & 11.06 &0.638\\
 & & &RelDiff & 3.9\%& 0.1\% &0.5\% &0.8\% &0.1\% & 0.8\% &0.4\%\\

 & 15°& & 0 & 8.02 & 123.67 &42.26 &29.65 &5.20 & 13.64 &0.286\\
& & & 1 & 8.26 &124.11 &42.33 &29.67 &5.24 &13.70 &0.287\\
 & & &RelDiff & 3.0\% &0.4\% &0.2\% &0.1\% &0.8\% & 0.4\% &0.1\%\\

 & 30°& & 0 & 12.82 & 283.10 &100.78 &71.90 &5.24 &10.98 &0.080\\ 
& & & 1& 13.20& 282.78 &100.40 &71.55 &5.19 & 10.57 &0.076\\
 & & &RelDiff & 3.0\% &-0.1\% &-0.4\% &-0.5\% &-0.8\% &-3.7\% &-5.9\%\\ \hline
    \end{tabular}
    \caption{Axial force $Fx_1$, normal force $Fx_2$, pitch moment $Mx_3$ (relative to nose-tip), $Mjx_3$ (relative to jet center) and corresponding augmentation factors $K$ over 65~km to 80~km. Condition flags same as previous that in previous rows are omitted. Rows with SST flag equals 0 list GSIS results, while with flag 1 list GSIS-SST results. The rows start with RelDiff provides the relative difference of quantity of interest (QoI) from GSIS-SST (1 row above) relative to GSIS (2 rows above), i.e., $QoI_{GSIS-SST}/QoI_{GSIS}-1$.}
    \label{tab:ForceMoment}
\end{table}
Although the Boltzmann equation comprehensively captures gas dynamics across turbulent to rarefied flow regimes, the computational demands of direct numerical simulation (DNS) are prohibitively high. In high Reynolds number (Re) regions, the spatial grid must be extremely fine to resolve small-scale turbulent structures, while in regions of high Knudsen number (Kn), the discrete velocity grid demands dense sampling to capture the molecular interactions accurately. Given that DNS of the Navier-Stokes (NS) equations already requires significant computational resources to simulate turbulence, performing DNS for the Boltzmann equation in scenarios where both turbulence and rarefaction coexist far exceeds current computational capabilities.

To overcome this limitation, we propose a multiscale modeling approach that offers a practical and efficient alternative. Our strategy is to couple the Reynolds-Averaged Navier–Stokes (RANS) turbulence model with the Boltzmann equation, thereby alleviating the need for finely-resolved spatial grids in turbulent regimes. This coupling ensures that the model retains the asymptotic-preserving property: it naturally recovers the RANS model in high-Re flows and reverts to the Boltzmann equation in highly rarefied environments (large Kn).

From a numerical perspective, since RANS produces time-averaged steady-state solutions, the Boltzmann equation is efficiently solved using the General Synthetic Iteration Scheme (GSIS), specifically designed for steady-state simulations~\citep{Su2020Can,Zhang2024Efficient}.

In the following sections, we first introduce the Boltzmann kinetic model, which describes gas dynamics across the continuum and rarefied regimes. Next, we derive the two-temperature Navier-Stokes equations from the kinetic model in the small Knudsen number limit and present the RANS model as a tool for simulating turbulence on coarse grids. Finally, we demonstrate the coupling of GSIS and RANS to efficiently solve the kinetic equation in flow regimes spanning from turbulence-dominated to rarefied conditions.

%Although the Boltzmann equation encapsulates the gas dynamics across turbulent to rarefied regimes, the computational demands of DNS are overwhelming. In regions of high Re, the spatial grid must be finely resolved, while in regions of high Knudsen number Kn, the discrete velocity grid requires dense sampling. Given that the DNS of NS equations is already a time-intensive process for simulating turbulence, the prospect of performing the DNS of the Boltzmann equation in scenarios where turbulence and rarefaction coexist is beyond the reach of current computational capability. 
%To address this challenge, we introduce a multiscale modeling approach that offers a viable alternative.
%Our idea is to couple the Reynolds-averaged Navier–Stokes (RANS) turbulence model into the Boltzmann equation, to ease the requirement of fine spatial grids in turbulent regime.  The coupling should process the asymptotic-preserving property, i.e., it automatically recovers the RANS model when Re is high, and the Boltzmann equation when Kn is large. Moreover, from the numerical perspective, since the RANS produces the time-averaged steady state, the Boltzmann equation will also be solved by the general synthetic iteration scheme (GSIS) tailored for efficient steady-state simulations~\citep{Su2020Can,Zhang2024Efficient}.

%In the following, we first introduce the Boltzmann kinetic model which describe the gas dynamics from the continuum to rarefied flow regimes. Second, we introduce the two-temperature NS equations derive from the kinetic equation when the Knudsen number is small, and describe the RANS model for efficient simulation of turbulence on coarse spatial grid. 
%Third, we couple the GSIS and RANS to efficiently find the solution of the kinetic equation from the turbulent to rarefied  regimes. 


%With the prosperity of various multiscale methods for flow from all regimes, faster and more efficient methods on coarser grids are gradually substituting the role of DSMC in many applications. These deterministic methods solve a model equation with simplified collision term instead of the original Boltzmann equation, such methods include the unified gas-kinetic scheme \citep{Xu2010}. There is also , which differs from above methods by its inclusion of a macroscopic solver. These methods bring a more suitable description of flows in transition regime and usually have the asymptotic behavior of returning to the NS solution at extreme conditions. They have also relaxed the spatial and temporal discretization requirements for multiscale flow problems and achieved good results in many engineering applications.


% \begin{equation}
% \frac{{\partial f}_{l}}{{\partial t}} + \boldsymbol{\xi} \cdot \nabla {f}_{l} = \frac{{g}_{l,t}-{f}_{l}}{\tau} + \frac{{g}_{l,r}-{g}_{l,t}}{{Z}_{r}\tau},\quad l=0, 1,
% \end{equation}

\subsection{Polyatomic Gas Kinetic Model}

While the dynamics of monatomic gases is described by the Boltzmann equation, that of the polyatomic gas is described by the \cite{WangChang1951Transport} equation. 
To reduce the computational cost, simplified kinetic equations are usually adopted~\citep{Wu2015kinetic,li2021uncertainty}. Here, two reduced VDFs $f_0(t, \bm{x}, \bm{\xi})$ and $f_1(t, \bm{x}, \bm{\xi})$ are used to describe the translational and rotational states of molecular gas, where $t$ is the time, $\bm{x}=(x_1,x_2,x_3)$ is the spatial coordinate, $\bm{\xi}=(\xi_1,\xi_2,\xi_3)$ is the molecular velocity. The rotational degrees-of-freedom is a constant $d_r$, and it is assumed the vibrational and electronic energy levels are not excited, although the model can be easily extended to include these non-equilibrium and even multi-physics effects such as radiation~\citep{Li2023Kinetic}. The evolution of VDFs is governed by the following Boltzmann kinetic equations:
\begin{equation}\label{general_model}
    \begin{aligned}
        &\frac{\partial f_0}{\partial t}+\bm{\xi}\cdot \nabla f_0 = \frac{g_{0t}-f_0}{\tau}+\frac{g_{0r}-g_{0t}}{Z_r\tau}, \\
        & \frac{\partial f_1}{\partial t}+\bm{\xi}\cdot \nabla f_1 = \frac{g_{1t}-f_1}{\tau}+\frac{g_{1r}-g_{1t}}{Z_r\tau}, 
    \end{aligned}
\end{equation}
where $\tau$ and ${Z}_{r}\tau$ are the elastic and inelastic collision characteristic time, respectively, with ${Z}_{r}$ being the rotational collision number. The elastic collision conserves the kinetic energy, while the inelastic collision exchanges the translational and rotational energies. In order the make the kinetic model mimic the behaviors (such as to recover the shear viscosity, bulk viscosity, translational and internal heat conductivities) of the \cite{WangChang1951Transport} equation as closely as possible, the reference VDFs to which the gas system will relax are designed as follows:
\begin{equation}\label{reference_VDF}
    \begin{aligned}
        g_{0t}&= \rho\left(\frac{1}{2\pi RT_t}\right)^{3/2}\exp\left(-\frac{c^2}{2RT_t}\right)\left[1+\frac{2\bm{q}_{t}\cdot\bm{c}}{15RT_tp_t}\left(\frac{c^2}{2RT_t}-\frac{5}{2}\right)\right],\\
        g_{0r}&= \rho\left(\frac{1}{2\pi RT}\right)^{3/2}\exp\left(-\frac{c^2}{2RT}\right)\left[1+\frac{2\bm{q}_{0}\cdot\bm{c}}{15RTp}\left(\frac{c^2}{2RT}-\frac{5}{2}\right)\right],\\
        g_{1t}&=\frac{d_r}{2}RT_rg_{0t} + \left(\frac{1}{2\pi RT_t}\right)^{3/2}\frac{\bm{q}_{r}\cdot\bm{c}}{RT_t}\exp\left(-\frac{c^2}{2RT_t}\right), \\
        g_{1r}&=\frac{d_r}{2}RTg_{0r} + \left(\frac{1}{2\pi RT}\right)^{3/2}\frac{\bm{q}_{1}\cdot\bm{c}}{RT}\exp\left(-\frac{c^2}{2RT}\right),
    \end{aligned}
\end{equation}
with $\bm{q}_{0},~\bm{q}_{1}$ being linear combinations of translational and internal heat fluxes \citep{li2021uncertainty}. For nitrogen, the coefficient matrix $\bm{A}=[0.786,-0.201,-0.059,0.842]$ and $Z_r=3.5$.

Macroscopic quantities, such as the density $\rho$, flow velocity $\bm{u}$, deviatoric stress $\bm{\sigma}$, translational and rotational temperature $T_t$ and $T_r$, translational and rotational heat flux $\bm{q}_t$ and $\bm{q}_r$, are obtained by taking the moments of VDFs. The total temperature $T$ is defined as the equilibrium temperature between the translational and internal modes $T=(3T_t+d_rT_r)/(3+d_r)$. The pressure related to the translational motion is $p_t=\rho R T_t$, while the total pressure is $p=\rho RT$.

The gas kinetic model describes the gas-gas interaction, in order to fully determine the gas dynamics in wall-bounded problems, the gas-surface interaction should be specified. In this work, we adopt the Maxwell gas-surface boundary condition, where the gas molecules hitting the solid wall will be reflected diffusely. 


\subsection{Synthetic NS Equations}\label{sec:NSequations}

Exploiting the relation between macroscopic quantities and mesoscopic VDFs, the macroscopic moment equations can be derived from the kinetic equation \eqref{general_model}. The first three equations below describe the conservation of mass, momentum, and total energy, and the fourth equation accounts for the exchange between translational and rotational energies:
\begin{equation}\label{eq:macroscopic_equation_2}
\begin{aligned}
\frac{\partial \rho}{\partial t} + \nabla \cdot (\rho \boldsymbol{u}) = 0,\\
\frac{\partial \rho \boldsymbol{u}}{\partial t} + \nabla \cdot (\rho \boldsymbol{u} \boldsymbol{u}) = -\nabla \cdot (\rho R T_t \textbf{I} + \boldsymbol{\sigma}),\\    
\frac{\partial \rho e}{\partial t} + \nabla \cdot (\rho e \boldsymbol{u}) = -\nabla \cdot (\rho R T_t \boldsymbol{u} + \boldsymbol{\sigma} \cdot \boldsymbol{u} + {\boldsymbol{q}}_{t} + {\boldsymbol{q}}_{r}),\\
\frac{\partial \rho e_r}{\partial t} + \nabla \cdot (\rho e_r \boldsymbol{u}) = -\nabla \cdot {\boldsymbol{q}}_{r} + \frac{d_r \rho R}{2}\frac{T-T_r}{{Z}_{r}\tau},
\end{aligned}
\end{equation}

Equation \eqref{eq:macroscopic_equation_2} is not closed, since the stress and heat fluxes have not been expressed in terms of the density, velocity, temperature and their spatial gradients. The Chapman-Enskog expansion of the kinetic equation to the first-order of Kn yields the linear NS constitutive relations. The (laminar, or physical) shear viscosity could be then obtained as $\mu=p_t\tau$, while the transitional and rotational thermal conductivities $\kappa_t$ and $\kappa_r$ are acquired through the coefficient matrix $\bm{A}$, $\mu$ and $d_r$~\citep{li2021uncertainty}. With a constant $d_r$ of 2, the conductivities could be calculated as:
\begin{equation}\label{eq:kappaAnumber}
	\left[ 
      \begin{array}{ccc} 
        \kappa_t \\ \kappa_r 
      \end{array}
    \right]
	= \mu
        \left[
        \begin{array}{ccc} 
        3.546 \\ 1.435
        \end{array}
        \right].
\end{equation}


\subsection{GSIS-SST Scheme for All Flow Regimes}

To study rarefied gas dynamics, the numerical solution of the kinetic equation~\eqref{general_model} is required. Yet, due to the VDFs being defined in a six-dimensional phase space, the computational burden is significantly higher compared to solving the NS equations. Fortunately, for most engineering applications, rarefied gas flows are typically laminar, and the focus is primarily on steady-state solutions. As a result, implicit iteration methods are generally employed. In this section, we provide a brief overview of the recently developed General Synthetic Iterative Scheme (GSIS) for efficiently simulating rarefied laminar flows, and then introduce the GSIS-SST model, tailored for cases where turbulence and rarefaction coexist.

GSIS is a multi-scale method that alternatively solves the mesoscopic kinetic equation and macroscopic synthetic equation~\citep{Su2020Can,Zhang2024Efficient}. The synthetic equation is given by \eqref{eq:macroscopic_equation_2}, but now the stress and heat flux are constructed as
\begin{equation}\label{eq:full_constitutive}
    \begin{aligned}
        \bm{\sigma} &= -\mu \left(\nabla\bm{u}+\nabla\bm{u}^{\mathrm{T}}-\frac{2}{3}\nabla\cdot\bm{u}\mathrm{I}\right) + \text{HoT}_{\bm{\sigma}},\\
        \bm{q}_{t} &= -\kappa_t\nabla T_t + \text{HoT}_{\bm{q}_{t}},\\
        \bm{q}_{r} &= -\kappa_r\nabla T_r + \text{HoT}_{\bm{q}_{r}},
    \end{aligned}
\end{equation}
where the high-order terms (HoTs) describing the rarefaction effects are constructed as:
\begin{equation}\label{eq:getHoTs}
    \begin{aligned}
        \text{HoT}_{\bm{\sigma}} &= \int \left(\bm{c}\bm{c}-\frac{c^2}{3}\mathrm{I}\right)f_0 \mathrm{d}\bm{\xi} -\bm{\sigma}^{\text{NS}},\\
      \text{HoT}_{\bm{q}_{t}} &= \int \bm{c} \frac{c^2}{2}f_0 \mathrm{d}\bm{\xi} -\bm{q}_{t}^{\text{NS}},\\
        \text{HoT}_{\bm{q}_{r}} &= \int \bm{c}f_1 \mathrm{d}\bm{\xi}  -\bm{q}_{r}^{\text{NS}},
    \end{aligned}
\end{equation}
with $\bm{c}=\bm{\xi}-\bm{u}$ is the peculiar (thermal) velocity, and $\textbf{I}$ is the identity matrix. The $\bm{\sigma}^{\text{NS}}$, $\bm{q}_{t}^{\text{NS}}$ and $\bm{q}_{r}^{\text{NS}}$ calculated based on linear NS constitutive relations using the macroscopic properties from the moments of the VDFs as well. 

\begin{figure}
\centering
\includegraphics[width=1\linewidth]{Artworks/demo.png}
\caption{Schematic of the GSIS and GSIS-SST. The kinetic equation is solved by the discrete velocity method iteratively (here $k$ is the iteration step). Between each iteration, the HoTs extracted from the kinetic solver are fed into the macroscopic synthetic equation, which is solved to the steady state or for $m\approx400$ steps. Then, the updated macroscopic quantities are fed into the kinetic solver through the modification of VDFs. Detailed implementation of GSIS are given by~\cite{Liu2024Further}. Different to the pure GSIS, in GSIS-SST the turbulent viscosity and heat conductivities are added in the macroscopic synthetic equation.
}
\label{Demo}
\end{figure}

As sketched in figure~\ref{Demo}, the kinetic solver provides HoTs to the synthetic equation~\eqref{eq:macroscopic_equation_2}, while the solution of synthetic equation, when solved to the steady-state, steers the evolution of VDFs towards the steady state. It must be emphasized that, as shown in figure~\ref{Demo}, \eqref{eq:full_constitutive} and~\eqref{eq:getHoTs} are solved at different iteration steps, thus the NS constitutive relations cannot cancel out each other until the converged solution is found.

As has been demonstrated in various numerical simulations, this kind of treatment facilities the fast convergence in the whole range of gas rarefaction~\citep{Su2020Can,Liu2024Further,Zhang2024Efficient}. Furthermore, according to the Chapman-Enskog expansion, in the continuum limit, the HoTs are proportional to $(\text{Kn}^2)$~\citep{Su2020Fast}, such that the constitutive relation~\eqref{eq:full_constitutive} asymptotically preserves the NS limit when Kn is small.

To effectively simulate turbulence, even within the scope of the NS equations, it is essential to employ turbulence models. Given the significantly higher computational cost associated with the kinetic solvers, the incorporation of turbulence models is highly demanded.
Thanks to the explicit inclusion of the NS constitutive relations in~\eqref{eq:full_constitutive}, the RANS model can be seamlessly integrated into the GSIS framework. That is, once the turbulence viscosity $\mu_{turb}$ from the SST model is obtained, it is superimposed into the physical viscosity in the NS equations. Consequently, the stress and heat fluxes are formulated as follows:
\begin{equation}\label{eq:NSsigma}
\begin{aligned}
\boldsymbol{\sigma}&  = 
-(\mu_{lam} + \mu_{turb})\left(\nabla{\boldsymbol{u}}+\nabla{\boldsymbol{u^\text{T}}}-\frac{2}{3}\nabla\cdot\boldsymbol{u}\textbf{I}\right) + \text{HoT}_{\bm{\sigma}},\\
\boldsymbol{q}_{t}&  =  
-(\kappa_{t,lam}+\kappa_{t,turb})\nabla{T_t}
 + \text{HoT}_{\bm{q}_{t}},\\
\boldsymbol{q}_{r}&  = 
-(\kappa_{r,lam}+\kappa_{r,turb})\nabla{T_r}
 + \text{HoT}_{\bm{q}_{r}}.
\end{aligned}
\end{equation}

The general algorithm of the GSIS-SST is sketched in figure~\ref{Demo}. 

\subsection{Turbulence Model for Hypersonic Flows}

When installed laterally to the HFVs body axis, jet based method could help with HFVs' attitude control and maneuver \cite{Tian2022}, especially at the upper part of near-space, where the atmosphere there is too rarefied to provide valid dynamic pressure for conventional mechanical control surfaces. Its largest difference from the reaction control system (RCS) of satellites and spacecrafts is that the jet-flow interaction effect normally does not exist or not important in RCS applications, while such interaction for flapless flight control in upper space is indispensable and beneficial.
%However, previous studies on jet based active flow control method are conducted mostly in the continuum regime using conventional NS solvers, or micro-scale jets into quiescent space and vacuum plume with hybrid NS-DSMC (direct simulation Monte Carlo) solvers \cite{Henry2021Adaptive,Virgile2022Optimisation,Cai2022Review,Liu2024Study}. 

%Earlier ones among these researches employ DSMC methods and recent ones have tried various mesoscopic methods. The studied altitudes concentrate mainly around 70-80 km and the quantities examined falls to force amplification factor of the thrust from the jets. 

%They usually assume a fully turbulent environment by default and uses Reynolds-averaged Navier-Stokes (RANS) models or sometimes Large Eddy Simulation (LES). For The numerical methods are usually direct simulation Monte-Carlo (DSMC) and its combination with conventional Navier-Stokes (NS) solver.


%Numerically, researches on opposing jet are even more abundant thanks to the development of CFD methods and computer hardware. Geometry model from \cite{Hayashi2003} is popular for research on opposing jet flow mechanism \cite{BilalHussainShah2010,Rong2012,Huang2018,Huang2021}. Other researchers studied the opposing jet parametrically, in order to find optimized jet flow and geometry parameters \cite{Li2016,Ji2021}. There are also studies combining the opposing jet with other pass TPS, such as aerospike with opposing jet \cite{Moradi2018,Pish2019,Fan2019}, aerodisk or aerodome with opposing jet\cite{BarzegarGerdroodbary2014,Zhu2021a}. Some research groups even put opposing jet, lateral jet and aerospike or other active TPS, such as transpiration cooling, all together \cite{Shen2020,Zhang2022a,Meng2021}. During these numerical studies with simple or complex designs, turbulence model is always present. Most popular choice of turbulence model is the $k-\omega$ Shear Stress Transport (SST) model, it is found to be better than others regarding opposing jet simulation \cite{Ou2018}. Research from \cite{Tian2023} lies emphasis on the flow parameter design of opposing jets for stable flow control effect throughout a re-entry trajectory. They proposed to use total pressure ratio between the jet and the free flow behind the outer shock instead of static or total pressure ratio between the jet and directly the free flow. They also qualitatively proved the relationship between such pressure ratio and the position of jet Mach disk, enabling the assessment of flow control effect across different flight altitude and Mach number.



\subsection{Sonic Lateral Jet on Sharp Leading Edge}
\leib{Figure~\ref{fig:}} displays the pressure and Mach number contour at altitude 70 km with $PR=2.5$ a

\subsection{Kn}Change of Vortex before jet due to rarefaction and turbulence
The change of \leib{figure~\ref{fig:Geom}}
Mimicking flight altitude change




\subsection{Supersonic Lateral Jet on Sharp Leading Edge}
In this part, a supersonic lateral jet on sharp leading edge is considered. This scenario mimics the cold jet based attitude control system for HFVs. The gas is supplied from pressurized nitrogen tank with a total pressure of 200,000 Pa and total temperature 300 K. Supersonic jet is chosen here due to higher efficiency in generating thrust compared to sonic ones. The jet nozzle central axis stands 0.5 m from nose-tip. The jet nozzle is model from the throat plane, which is 0.02 m over the flat lower surface. The exit of the jet has a diameter of 0.0102 m and the nominal exit Mach number is 3.95 (calculated with \leib{\eqref{}}). The height of the first layer of grid is 0.001 mm. 
The flight altitudes are set to 70 km and 80 km with a fixed Mach number of 25. In these range, the free flow dynamic pressure is too low for mechanical control surfaces to produce enough control force and moments. The angles of attack varies between 0° and 30°. 

\subsection{Sonic Opposing Jet on Blunt Leading Edge}
The blunt leading edge has a nose diameter of 0.03 m and a 0.004 m wide slot (radius $R_j=0.002~\text{m}$) is placed at the nose-tip. Nitrogen gas is ejected from the slot parallel to the free flow. The jet total pressure is 4,620 Pa and the exit static temperature is 250 K. The Mach number at the jet exit is 1, and the dimensionless jet density is then 873. Free flow at altitude 75 km comes from the left and has a Mach number of 25. The reference length is the nose diameter and the corresponding Knudsen number is then 0.06. 


\subsubsection{Contour}

\subsubsection{Surface Quantities}
For the opposing jet, surface pressure and heat flux are of interest. These two quantities on the model surface is plotted in \leib{figure~\ref{fig}}. The pressure plots start from small values near the jet exit and rises to the peak at around $x_1=-0.1~\text{m}$. This is also the position of jet flow reattachment. Then, the surface pressure drops statically until $x_1=0~\text{m}$, where flat section of the model begins. With a slight increase, the pressure on the flat section of the model drops constantly. 

The shear stress $\sigma_{xy}$

Surface heat flux experiences a similar pattern as surface pressure. A peak heat flux could be observed at the reattachment point of $x_1=-0.1~\text{m}$. Then, the heat flux on the flat part changes only slightly. The curve from GSIS solution runs completely under that from the GSIS-SST, the peak heat flux is 15\% lower than the GSIS-SST prediction. And the GSIS curve on the flat part drops generally as $x_1$ increases, while GSIS-SST curve increases. Such difference makes up finally a 76\% heat flux difference at the end of the model. As \leib{shown in contour}, the jet from GSIS-SST is much more dispersed over the flat section of the model, the lower temperature jet layer diminishes faster and the protection effect degrades more severely than the GSIS prediction.

\subsection{Sonic Lateral Jet on Blunt Leading Edge}
The model of a lateral jet on a blunt leading edge is borrowed from literature \cite{Zhao2023Numerical}. All geometry setting are the same. In their paper, incoming flow conditions of Mach number of 8, positive angles of attack up to 25° and altitudes ranging from 60~90 km are investigated. They employed the Conserved Discrete Unified Gas Kinetic Scheme, which has by now no consideration on turbulence.  
Here in this study, free flow condition at altitude 70 km and Mach number 15 is considered. Both positive and negative angles of attack are investigated, assuming the jet is used for maneuver, rather than purely longitudinally trimming. The jet has a exit temperature of 250 K and Mach number 1. Jet pressure ratio of 6.5 is given, which produces a jet exit pressure of roughly 1,000 times to free flow pressure. Turbulence quantities are initialized exactly same as introduced earlier.

The flight altitudes are set to 70 km, 80 km, 90 km and 100 km with a fixed Mach number of 25. In this range of altitude, the free flow dynamic pressure is too low for mechanical control surfaces to produce enough control force and moments. 

\begin{table}
    \centering
    \begin{tabular}{cllcllcllll}\hline
         Altitude& AoA&PR&  SST& $Fx_1$&$Fx_2$&  $Mx_3$ &$Mjx_3$ &$K_{Fx2}$ & $K_{Mx3}$&$Cim$\\ \hline
         65 km & 15°&2.5&   0& 2.33&98.39&   32.33&22.29&4.64 & 10.68 &0.374\\
 & & & 1& 3.05& 111.08& 36.95 &25.62&5.93 & 15.26 &0.579\\
 & & &RelDiff & 31.1\%& 12.9\% &14.3\% &14.9\% &27.7\% & 42.9\%&54.6\%\\ \hline

 70 km& 15°& 1.5& 0& 4.02& 93.57 & 31.30 &21.75&5.42 & 12.79 &0.257\\
 & & & 1& 4.99& 97.09 & 32.46 &22.56 &6.01 & 14.71 &0.303\\
 & & &RelDiff & 24.2\%& 3.8\% &3.7\% &3.7\% &11.0\% & 15.1\%&18.1\%\\

 & & 2.5& 0& 3.49& 102.50 & 33.96 &23.50 &4.56 & 10.72 &0.358\\
 & & & 1& 4.23& 109.74 & 36.99 &25.79 &5.29 & 13.72 & 0.490\\
 & & &RelDiff & 21.2\%& 7.1\% &8.9\% &9.7\% &16.1\% & 28.1\%&36.9\%\\

 & & 3.5& 0 & 3.09& 111.12 & 36.27 &24.93 &4.16 & 9.58 &0.441\\
 & & & 1& 3.71& 118.86 & 40.04 &27.92 &4.72 &12.26 &0.613\\
 & & &RelDiff & 20.1\%& 7.0\% &10.4\% &12.0\% &13.5\% & 27.9\% &39.1\%\\ \hline

 75 km& 15°& 2.5& 0 & 5.34& 110.07 & 36.98 &25.75 &4.65 &11.42 &0.360\\ 
& & & 1& 5.93& 112.60 & 37.93 &26.44 &4.90 & 12.36 &0.396\\
 & & &RelDiff & 11.1\%& 2.3\% &2.6\% &2.7\% &5.5\% & 8.2\% &10.0\%\\ \hline

 80 km& 0°& 2.5& 0 & 2.86& 48.03 & 15.41 &10.51 &4.34 & 10.98 &1.744\\ 
& & & 1& 2.97& 48.08 &15.49 &10.59 &4.35 & 11.06 &1.764\\
 & & &RelDiff & 3.9\%& 0.1\% &0.5\% &0.8\% &0.1\% & 0.8\% &1.1\%\\

 & 15°& & 0 & 8.02 & 123.67 &42.26 &29.65 &5.20 & 13.64 &0.401\\
& & & 1 & 8.26 &124.11 &42.33 &29.67 &5.24 &13.70 &0.402\\
 & & &RelDiff & 3.0\% &0.4\% &0.2\% &0.1\% &0.8\% & 0.4\% &0.2\%\\

 & 30°& & 0 & 12.82 & 283.10 &100.78 &71.90 &5.24 &10.98 &0.087\\ 
& & & 1& 13.20& 282.78 &100.40 &71.55 &5.19 & 10.57 &0.082\\
 & & &RelDiff & 3.0\% &-0.1\% &-0.4\% &-0.5\% &-0.8\% &-3.7\% &-6.4\%\\ \hline


 

\section{The influence of jet pressure ratio}\label{sec:PR}

Three jet pressure ratios (i.e., PR=1.5, 2.5, and 3.5) are considered at a constant altitude of 70 km and \leir{AoA=15°}. As this ratio is directly related to the density of the jet flow, and consequently the turbulent viscosity, varying $\text{PR}$ enables a comprehensive analysis of turbulence's impact on the flow field across varying intensities. %This examination provides insights into the role of pressure ratio in modulating turbulence effects and overall jet behavior. 
The flow structures are observed first to present the macroscopic change, then the turbulent quantities are analyzed to explain such changes, following then by their impact to the surface quantities, and finally to the integrated force and moments.




\subsection{Flow structure}


% \leir{just two simple figures, write concisely}

Figure~\ref{fig:H70dRho} displays the density gradient contour from GSIS (upper half) and GSIS-SST (lower half) with streamlines colored in Q-criterion.
As the PR is varied from 1.5 to 3.5, the overall structure of flow field remains consistent with the analysis presented in figure~\ref{fig:H70TtComment}. 
However, there are also changes. The jet flow occupied area is naturally enlarged as $\text{PR}$ increases. All the flow structures are larger, such as the vortices, the jet expansion fan.

% The recirculation zones in front of the jet and behind the jet expand. The recompression shock is not obvious when $\text{PR}=1.5$, but easily observable when $\text{PR}=3.5$. The boundary layer in the upstream recirculation zone is also visualized, while the low pressure downstream recirculation zone is free of high density gradient until the jet flow reattaches on the surface.


\begin{figure}[h]
    \centering
    \subfloat[$\text{PR}=1.5$]{\includegraphics[width=0.49\linewidth,trim={20 40 30 90}, clip]{Artworks/H70PR1.5dRhoCP.png}}
    \subfloat[$\text{PR}=3.5$]{\includegraphics[width=0.49\linewidth, trim={20 40 30 90}, clip]{Artworks/H70PR3.5dRhoCP.png}}
    % {\includegraphics[width=0.49\linewidth,trim={20 20 30 90}, clip]{Artworks/H70tauxy.png}}
    % %{\includegraphics[width=0.49\linewidth,trim={50 70 50 90}, clip]{Artworks/H70PR2.5dRhoCP.png}}
    % {\includegraphics[width=0.49\linewidth,trim={20 20 30 90}, clip]{Artworks/H70Q.png}}
    %{\includegraphics[width=0.49\linewidth, trim={50 70 50 90}, clip]{Artworks/H70PR3.5dRhoCP.png}}
    %{\includegraphics[width=0.49\linewidth,trim={20 20 30 90}, clip]{Artworks/H70RelDiffQ.png}}
    \caption{Magnitude of density gradient and streamlines colored with Q-criterion. 
    GSIS and GSIS-SST solutions are shown in the upper and lower half of each figure, respectively. Flight altitude is 70~km, AoA=15°.%$H$ is the penetration height of the jet.
    }
    \label{fig:H70dRho}
\end{figure}

% \begin{figure}[h]
%     \centering
%     {\includegraphics[width=0.49\linewidth,trim={0 50 0 0}, clip]{Artworks/H70J1_5DissiQ.png}}
%     {\includegraphics[width=0.49\linewidth,trim={0 50 0 0}, clip]{Artworks/H70J3_5DissiQ.png}}
%     \caption{ Contours of viscous dissipation rate $\epsilon$ colored with Q-criterion and streamlines. \leib{The GSIS solution is shown in the upper half and GSIS-SST is in the lower half of figures on the second row. Will enlarge the core area later.} 
%     Flight altitude is 70~km, and $\text{PR}$ are 1.5 (left column) and 3.5 (right column).
%     }
%     \label{fig:H70DissQ}
% \end{figure}


% Difference observed with increasing $\text{PR}$ is the growth in penetration height. Given that the outer bow shock at high altitudes is somewhat indistinct, we define the penetration height $H$ as the point (with $x_1>0.1~\text{m}$) on the jet flow streamlines that is closest to the wall and the jet exit. According to the GSIS-SST solutions, $H$ is roughly $0.0159~\text{m}$ (at $x_1=0.119~\text{m}$) when $\text{PR}=1.5$, and $0.0306~\text{m}$ when $\text{PR}=3.5$. It is evident that the penetration height increases with rising pressure ratio, and the highest point moves further downstream. The GSIS-SST and GSIS solutions exhibit negligible difference in $H$.
As for the difference between GSIS and GSIS-SST, the first thing that one may notice is that the upstream separation area is almost identical for GSIS and GSIS-SST, both in terms of streamlines shape and values of Q-criterion~\citep{Jeong1995On}. This implies a similar vortex strength and stability, which is beyond expectation since this is strong interaction area with high density and pressure, and likely to be influenced by turbulence. A trivial sign of the inclusion of turbulence only exists around the small vortex left to the jet exit, as PR increases. In the GSIS-SST solution, this small vortex is more diffusive, as its streamlines are not as layered as the less viscous GSIS one.

Another notable difference presents itself in the downstream separation area.
% is that the three vortices from GSIS and GSIS-SST solutions exhibit greater difference when $\text{PR}$ rises. 
% At lower $\text{PR}$, the two upstream vortices has similar size and location. The larger ones are characterized by multiple overlapped circulating streamlines and the \leir{smaller ones are smaller??} and also diffusive, implying a similar vortex strength and stability. 
The downstream vortex in GSIS is less diffusive than the GSIS-SST one even at the lowest PR. %as it is prone to vortex deformation and breaks into smaller vortex more easily. 
In the vortex core, Q from GSIS-SST in the large downstream vortex is lower than that from the GSIS solution, signaling a less rotational nature. It is also prone to vortex deformation and breaks into smaller vortex more easily. 
% due to higher effective viscosity (the combination of $\mu_{lam}$ and $\mu_{turb}$), which should typically promote the stable rotation and coherent structure of vortex.
The derived secondary vortex exists between the large downstream vortex and the wall (centers around $x_1=0.11~\text{m}$, at PR = 1.5) in GSIS solution, but is absent in GSIS-SST result, until PR is increased to 3.5. %(built up due to higher vorticity caused separation)
These observations well demonstrate the low stability nature of the less viscous GSIS solution, compared with turbulence statistically modeled GSIS-SST.

%one single streamline captures the whole vortex, whereas the vortex in GSIS-SST consists of multiple distinct layer of circulating streamlines (only one is plotted in the figure). 
%What else needs to be noticed is that there is also  , capturing fine-scale rotational details (as shown in at $\text{PR}=3.5$)
%Meanwhile, the GSIS-SST, due to the averaged nature of RANS framework, properly retains a smooth and layered structure. This implies the reduction in flow stability as jet flow grows stronger, and the divergence between the two solvers enlarges. Similar observation applies also for the downstream vortices. 

% When the $\text{PR}$ increases, all vortices grow in size. The large upstream vortex from GSIS and GSIS-SST are still characterized with intricate, overlapping streamlines. The smaller upstream vortex from GSIS is more structures than the GSIS-SST one. The large downstream vortex in GSIS is larger and more stretched than that in GSIS-SST, the secondary vortex near wall grows and forms layered structure in GSIS. With the increase in $\text{PR}$, such secondary vortex also appears in GSIS-SST, but in a rather small scale and less layering manner.

% These observations indeed exhibit the fine scale resolved ability of GSIS, which is of course a strength of the laminar GSIS. Yet, it also tend to make the scheme less stable in turbulent flows. %since it can also be seen that as $\text{PR}$ increases, more fine structures, such as the small downstream vortex, emerge and grow. 
%

% \leir{moving this part to section 3.1, merge figure 4 and 6 }
% Next, the vorticity field is examined with the Q-criterion as shown in figure~\ref{fig:H70DissQ}, whose positive value indicates that the local flow structure is dominated by rotation (the vorticity or rotational motion exceeds the rate of strain), and negative value suggests that strain dominates over rotation in the flow (the flow is more likely to stretch or compress fluid elements rather than maintain rotational coherence). 
% \cite{Jeong1995On}
% It is obvious that positive Q dominates the vortex cores. But the lower corner of the downstream large vortex also has positive Q, indicating the flow rotates and turns back toward the surface in a less chaotic and stable manner. 
% Q from GSIS-SST in the large downstream vortex is lower than that from the GSIS solution, although GSIS-SST shows higher effective viscosity (the combination of $\mu_{lam}$ and $\mu_{turb}$), which should typically promote the stable rotation and coherent structure of vortex. %This is the result of the breaking of the large vortices, the unstable large vortex in GSIS is prone to breaking.  
% This difference can be attributed to the instability of the large vortex in GSIS, which is more prone to breaking apart, whereas the turbulence modeling in GSIS-SST leads to greater vortex stability, but reduced local Q due to the smoothing effects of the turbulent viscosity.
% Negative Q could be identified at the corners of the vortices close to the jet, since flow separation and strong shear between flow layers exist. 
% Also, the free flow past the leading shock, the separation shock experiences shearing motion, while the streamlines of free flow past the outer bow shock are colored in both blue (negative) and red (positive). The blue part locates far from the jet flow, therefore the typical shear strain dominates. The red part locates right next to the jet flow, thus rotates due to the large velocity gradient between the free flow and the jet flow. At further downstream, the streamlines (outer part of the jet flow and the free flow) become blue again after passing through the recompression shock. The recompression shock suppresses rotation over shearing for a short distance, and followed by rotation created by the shearing between jet and free flow layer. But, finally, as the mixing between layers progress, both motions diminish and reach a balance.

\subsection{Turbulent Quantities}

%In this part, it will be demonstrated that the free flow turbulence does not impact the near wall region. The injected turbulence from the jet and generated turbulence in the downstream separation region together build up the difference between GSIS-SST and GSIS.% The positive relation between TKE and $\mu_r$ production is identified. 
% Free flow turbulence poses no much influence on the flow field downstream the jet exit, since the $\mu_{r}$ is only significant in jet-controlled area.
% k and $\mu_{r}$ production increases as $\text{PR}$ goes up.
% Turbulence promotes energy dissipation in the downstream recirculation region, thus helps main a stable vortex, shaping the difference mentioned in previous section.

% This part examines the turbulent quantities to further explain the cause of difference observed between GSIS and GSIS-SST previously.
To understand how the difference between GSIS and GSIS-SST arises, we examine fields of turbulent quantities, turbulent kinetic energy (TKE) and turbulent-to-laminar viscosity ratio $\mu_r$, as shown in figure~\ref{fig:H70mu_r}.
% demonstrates that turbulence from the free flow has negligible influence on the near-wall region. Instead, the injected turbulence from the jet and the turbulence generated in the downstream separation region are the primary sources to the observed differences between the GSIS-SST and GSIS models. \leir{replace this paragraph by: To explain XXX, we show the TKE ....}

\begin{figure}[h]
    \centering
    {\includegraphics[width=0.49\linewidth,trim={0 50 0 0}, clip]{Artworks/H70J1_5TKEMuR.png}}
    {\includegraphics[width=0.49\linewidth,trim={0 50 0 0}, clip]{Artworks/H70J3_5TKEMuR.png}}
    \caption{Contours of turbulent kinetic energy (upper half) and turbulent-to-laminar viscosity ratio (lower half) from GSIS-SST, when the PR is 1.5 (left) and 3.5 (right). 
    }
    \label{fig:H70mu_r}
\end{figure}

From the figures, high TKE could be observed across the flow field.
% Figure~\ref{fig:H70mu_r} provides the distribution of turbulent kinetic energy (TKE) from GSIS-SST solutions for PR=1.5 and 3.5. 
Large amount of TKE is present in the post-shock region, due to the leading shock, separation shock and outer bow shock. Shear layer between the jet flow and the post-shock free flow also produces large amount of TKE. Then comes to the recompression shock, whose TKE production exists mainly in the post-shock free flow and merges with those from shear layer. Moving toward the jet area, apparent boundary of high TKE exists, disconnecting the two regions.
The expected turbulent jet flow does not predominantly carry TKE as one might anticipate prior to computation, if compared to the huge amount of TKE from post-shock free flow. Within the jet flow area, TKE is generated downstream of the Mach disk and within the separation regions with high strain-rate, i.e. the small upstream vortex to the left of the jet and the large vortex to the right of the jet, as in fig~\ref{fig:H70dRho}.
Such production scales positively with PR. 
The near-wall region exhibits a low magnitude of TKE due to the turbulent dissipation enforced by the boundary conditions. 
% Furthermore, two vortices in fig~\ref{fig:H70dRho} are associated with substantial TKE: the small upstream vortex to the left of the jet and the large vortex to the right of the jet. The former vortex is linked to TKE production from shear motion and the velocity gradient $\partial{u_{2}}/\partial{x_1}$, while the latter large vortex primarily generates TKE through vortex deformation, as it is significantly elongated along the main jet flow direction, also influenced by the velocity gradient $\partial{u_{1}}/\partial{x_1}$.
 
However, not all of the TKE contributes to changes in the macroscopic flow field, as the derived $\mu_{turb}$ accounts for only a portion of the stress and heat flux, it is the relative magnitude of $\mu_{turb}$ compared to the physical viscosity $\mu_{lam}$ that determines the actual significance of turbulence. As the viscosity ratio $\mu_r$ shown in fig~\ref{fig:H70mu_r}, although TKE significantly increases after the outer shock, it has minimal impact on the solution because the $\mu_{r}$ ratio is quite low in the post-shock free flow region. In all solutions, $\mu_r$ is negligible in the area between the jet flow and the outer shock, cutting any connections between jet turbulence and free flow turbulence.
  
Only the TKE in jet-controlled area possesses real significance and is independent from free flow turbulence, due to the low temperature of jet flow.
We could see that the presumed turbulent jet carries high $\mu_{r}$ into the flow field. The jet $\mu_r$ diminishes in the expansion fan, but gets enhanced through the barrel shock and Mach disk.
%is concentrated in the core region of the jet flow within the expansion fan, and after the Mach disk near the shear layer. 
Also in the large vortex with high TKE right to the jet, TKE is turned into effect in form of $\mu_{turb}$. In addition, high $\mu_{r}$ could be observed after the jet flow reattaches the model surface, more evident in fig~\ref{fig:H70mu_r} with PR=3.5. Strip-like structures of high $\mu_{r}$ form near the wall and extends far downstream, responsible for turbulence related difference between GSIS and GSIS-SST. They come from two sources of high effective TKE: the downstream large vortex (TKE produced from vortex elongation) and the jet (TKE from boundary condition, Mach disk and recompression shock).
The $\mu_{r}$ dictated area also grows with increasing $\text{PR}$.
% the Mach disk and the recompression shock. Such strip grows for some distance and then diminishes as the jet flows further downstream, as the mixing with hot post-shock free flow brings up the temperature and molecular viscosity regain dominance.

 % A strip of high $\mu_{r}$ left to the barrel shock emerges. This strip follows the stretching direction of the upstream small vortex. A similar strip could also be seen in the downstream large vortex near the jet exit.

% We then choose to probe the viscosity profile at 

%Together with the observation of $\mu_{r}$, deeper insight into the difference between the two large downstream vortices (since $\mu_{r}$ is negligible in the upstream recirculation region, those vortices are not deeply influence by turbulence) could be obtained. 
% We could now explain the observed difference in the downstream separation region between GSIS-SST and GSIS in the previous part, with $\mu_{r}$. In the GSIS solution, the large downstream vortex is mainly sustained by the rotational inertia plus molecular viscosity of the flow and thus more prone to vortex deformation and breakdown, which is obvious that the vortices in GSIS are always longer in $x_1$ direction, and a secondary small vortex between the large one and the wall always appears larger than in GSIS-SST solutions, which has the help from additional turbulent viscosity.
% By examining the differences in $\mu_{r}$ between the large downstream vortices, we can infer the mechanisms at play. 

%Such trend also applies to GSIS solution, but difference exist. In GSIS solution, the penetration height and its horizontal distance to jet exit are smaller than GSIS-SST when $\text{PR}=1.5$ and 2.5, i.e., jet flow influence is smaller in GSIS solution. When $\text{PR}$ increases to 3.5 the GSIS solution gives larger value of $H$, and the highest point is further to the jet exit. But this is comparison based on the streamlines from jet exit. If observing the streamlines from free flow, and considering the displacement of these streamlines from the wall as an index for the jet flow impact, then the GSIS-SST predicts always a higher impact of the jet flows than GSIS. The difference between these two ways of observation is resulted from the influence of the vortices in the upstream recirculation zone. When the $\text{PR}$ is high, the streamlines from recirculation zone ocupy more area between the jet flow and free flow streamlines.


\subsection{Profiles of field quantities}
In order to deeper understand how turbulence and pressure ratio effect surface quantities, we
then investigate the viscosity profiles at $x_1=0.35~\text{m}$, where the jet has reattached on the model surface and a proper boundary layer has been formed. Figure~\ref{fig:H70Vis} provides the full profile of velocity, Mach number, laminar and turbulent viscosity with PR=1.5, also their change with different PR in the near wall layer ($|x_2| < 0.005~\text{m}$). Figure~\ref{fig:H70Vis}(a) is also marked with flow layers.
% Turbulence impacts the near wall region through dominant turbulent viscosity brought by the jet flow, and such impact grows with $\text{PR}$.
% In the flat section of the model, linear relationship between the outer shock position and the pressure ratio is identified.
% Turbulence influence is seen concentrated in the near wall jet flow layer.
% The considered jet turbulence increases the surface shear stress and heat flux both 
\begin{figure*}
    \centering
    {\includegraphics[width=0.37\linewidth]{Artworks/H70PR1_5VelMa2.png}}
    % {\includegraphics[width=0.3\linewidth]{Artworks/H70PR2_5VelMa2.png}}
    % {\includegraphics[width=0.3\linewidth]{Artworks/H70PR3_5VelMa2.png}}\\
    % \vspace{0.5cm}
    % {\includegraphics[width=0.3\linewidth]{Artworks/H70PR1_5VelMaDetail.png}}
    % {\includegraphics[width=0.3\linewidth]{Artworks/H70PR2_5VelMaDetail.png}}
    % {\includegraphics[width=0.3\linewidth]{Artworks/H70PR3_5VelMaDetail.png}}\\
    % \vspace{0.5cm}
    \includegraphics[width=0.32\linewidth]{Artworks/H70PR1_5Vis2.png}\\
    \vspace{0.5cm}
    \includegraphics[width=0.32\linewidth]{Artworks/H70PRVis.png}
    \includegraphics[width=0.32\linewidth]{Artworks/H70PRVisTurb.png}
    %  \includegraphics[width=0.3\linewidth]{Artworks/H70PR1_5Vis.png}
    % \includegraphics[width=0.3\linewidth]{Artworks/H70PR2_5Vis.png}
    % \includegraphics[width=0.3\linewidth]{Artworks/H70PR3_5Vis.png}\\
    % \vspace{0.5cm}
    %  \includegraphics[width=0.3\linewidth]{Artworks/H70PR1_5VisDetail.png}
    % \includegraphics[width=0.3\linewidth]{Artworks/H70PR2_5VisDetail.png}
    % \includegraphics[width=0.3\linewidth]{Artworks/H70PR3_5VisDetail.png}
    \caption{Profiles of velocity and Mach number (overview in $1^\text{st}$ row and detailed view in $2^\text{nd}$ row) and viscosity (overview in $3^\text{rd}$ row and detailed view in $4^\text{th}$ row) at $x_1=0.35~\text{m}$, when the altitude is 70~km. From left to right, $\text{PR}=1.5$, 2.5 and 3.5.}
    \label{fig:H70Vis}
\end{figure*}

% Figure~\ref{fig:H70VelMa} presents the velocity and Mach number at $x_1=0.35~\text{m}$. At $\text{PR}=1.5$, key flow features are annotated: the GSIS-SST model accurately reproduces the far-field free-flow conditions. Moving towards the wall, the dispersed outer shock is captured, followed by a transition into the post-shock region, where both Mach number and velocity decrease moderately. The post-shock free-stream layer lacks uniformity in Mach number and velocity due to low density. A shear layer is formed between the free-stream and jet flow close to the wall, leading to a sharp velocity drop. Differences between the GSIS-SST and GSIS solutions are minimal above the shear layer.

%the flow structures are marked. The GSIS-SST model reproduce the free flow conditions in the far field. Moving down to the wall, the dispersed outer shock is captured. Past the shock, the free-stream flow transitions into the post-shock region, where a moderate decrease in both Mach number and velocity exist.The free flow layer post shock does not exhibit a uniform distribution of Mach number and velocity. Closer to the wall, a shear layer forms between the free-flow layer and the jet flow, marking a significant drop in velocity. The difference between the GSIS-SST and GSIS solution is quite insignificant by now.
%
%and little difference is observed between the GSIS-SST and GSIS solution. 
%, with the GSIS-SST model predicting slightly earlier appearance of the shock than GSIS. 
%In the far-field region ($|x_2|>0.15~\text{m}$), both the GSIS and GSIS-SST models reproduce the free flow conditions. Moving down to the wall, the outer shock is captured by both models, with the GSIS-SST model predicting slightly earlier appearance of the shock than GSIS. 
%The outer shock is clearly affected by the rarefaction effects as it is much more thicker than shock in low altitude, \leib{since the discontinuity spans across multiple cells.}
%\leir{evidence?? not explicitly shown, but could be inferred from the plot}. 
%Past the shock, the free-stream flow transitions into the post-shock region, where the GSIS-SST and GSIS models show a moderate decrease in Mach number and velocity. Yet, the free flow layer does not exhibit a uniform distribution of Mach number and velocity. Closer to the wall, a shear layer forms between the free-flow layer and the jet, marking a significant drop in velocity, and little difference is observed between the GSIS-SST and GSIS solution. 

%Near the wall ($|x_2|<0.005~\text{m}$), the boundary layer is present, where the velocity drops to zero. The second row of figure~\ref{fig:H70VelMa} shows that the GSIS-SST model predicts thicker boundary layer, steeper gradients $\partial{u_1}/\partial{x_2}$ and $\partial{Ma}/\partial{x_2}$ could be observed. The near wall jet flow layer in GSIS-SST is better preseved than in GSIS, due to the existence of concentrated dominating extra viscosity $\mu_{turb}$ (as shown in the third row).
From figure~\ref{fig:H70Vis}(b), it is again proven that the free flow turbulence does not impact the jet-controlled area, since turbulent viscosity from free flow ($|x_2| > 0.13~\text{m}$) and jet flow ($|x_2| < 0.035~\text{m}$) is wide separated by near zero $\mu_{turb}$. When PR increases, the velocity as well as viscosity profiles are simply stretched in $x_2$ direction, with all the wall normal gradients get smoothed. They are not shown here for due to such similarities.

Detailed observation close to the wall ($|x_2| < 0.05~\text{m}$) tells that, laminar viscosity experiences delayed rise as PR increases, shown in figure~\ref{fig:H70Vis}(c). In both the GSIS and GSIS-SST solutions, $\mu_{lam}$ decreases rapidly as it approaches the wall, with minor differences between the two solvers in the near-wall region. Notably, the GSIS-SST solution predicts a higher $\mu_{lam}$ in the near wall region where turbulent mixing dominates, reflecting intensified energy exchange from hot outer flow to cold wall, which smooths out the temperature gradients across the flow field.

% first figure in the second row of figure~\ref{fig:H70Vis}), the boundary layer is evident, with velocity reducing to zero at the surface. The figure indicates that the GSIS-SST model predicts a thicker boundary layer with steeper velocity and Mach number gradients ($\partial u_1/\partial x_2$ and $\partial Ma/\partial x_2$). Additionally, the near-wall jet flow from GSIS-SST forms also a thicker uniform main stream layer, primarily due to the concentrated influence of the dominant turbulent viscosity ($\mu_{turb}$, shown in the third row), which damps disturbances from adjacent layers.
%more viscous profile, characterized by more aggressive velocity gradients $\partial{u_1}/\partial{x_2}$ near wall and slower increase in $u_1$ away from wall. All differences between the GSIS-SST and GSIS solutions are rooted in the jet layer, since the viscosity profile suggests that high and dominating $\mu_{turb}$ exists here. The GSIS-SST model provides a more typical high viscosity boundary layer.

% At $\text{PR}=2.5$, the viscosity profiles exhibit a stretched appearance in the $x_2$ direction compared to those at $\text{PR}=1.5$. Similarly, for $\text{PR}=3.5$, a nearly linear relationship emerges between the normal distance of the outer shock (measured from the wall) and the pressure ratio, as shown in the first row of the figures. 
% Specifically, the intersection point $x_\text{Ma}$, defined as the point where the Mach number profile (within the range of $5 < \text{Ma} < 20$) intersects the vertical axis, varies with $\text{PR}$: $x_\text{Ma} \approx 0.1177~\text{m}$ at $\text{PR}=1.5$, 0.1500~{m} at $\text{PR}=2.5$, and 0.1816~{m} at $\text{PR}=3.5$.
% This relationship can be approximated as $x_\text{Ma} = 0.032 \text{PR} + 0.0698$, which can aid in predicting the shock's location based on the pressure ratio. 
% It is also notable that, as $\text{PR}$ increases, the difference between the GSIS-SST and GSIS solutions becomes more pronounced, particularly in the Mach number profiles.

%When $\text{PR}=2.5$, profiles of the velocity and the Mach number look like stretched from those at $\text{PR}=1.5$ in the $x_2$ direction. Together with the results of $\text{PR}=3.5$, a nearly linear relationship between the normal distance of the outer shock (measured from the wall) and the pressure ratio is observed in the first row of figure~\ref{fig:H70VelMa}. 
%That is, if taking the intersection point $x_\text{Ma}$ (cross point of the dash-dot line with the vertical axis) of the linear part of the Mach number profile (in range of $5<\text{Ma}<20$), then the intersection point is $x_\text{Ma}\approx0.108~\text{m}$ at $\text{PR}=1.5$, 0.137~{m} at $\text{PR}=2.5$, and 0.163~{m} at $\text{PR}=3.5$, which can be fitted as $x_\text{Ma}=0.0276\text{PR}+0.0669$. This relation could be helpful for shock prediction, whose inner bound could be estimated by $x_\text{Ma}$ if $\text{PR}$ is given. A last point worth mentioning is that when $\text{PR}$ increases, the difference between GSIS-SST and GSIS solution becomes more obvious, as the Mach number profiles display.
% The influence of turbulence is visualized by plotting the distribution of laminar viscosity ($\mu_{lam}$) and turbulent viscosity ($\mu_{turb}$) at $x_1 = 0.35~\text{m}$ in figure~\ref{fig:H70VelMa} (only $\text{PR}=1.5$ is plotted in the 3rd row, since pressure ratio only stretches the curves). The profiles of these quantities in the wall-normal direction are generally well-separated, allowing clear identification of their influence.
%The influence of turbulence is visualized by plotting the distribution of physical viscosity (laminar part) $\mu_{lam}$ and turbulent viscosity $\mu_{turb}$ at $x_1=0.35~\text{m}$ in the third and bottom rows of figure~\ref{fig:H70VelMa}. The dominant areas of both quantities in the wall normal direction are generally separated, making it easy to identify the source of influence. 
% The $\mu_{lam}$ from all solutions exhibit low values in the far field, which increase after the outer shock due to rising temperature, then decrease near the wall as a result of the cooler jet flow near the wall and the wall temperature itself. At $\text{PR}=1.5$ for both solutions, $\mu_{lam}$ increases at approximately $|x_2|=0.14~\text{m}$, with a slight change in slope visible around $|x_2|=0.12~\text{m}$. The peak in $\mu_{lam}$ occurs at $|x_2|=0.065~\text{m}$. In both the GSIS and GSIS-SST solutions, $\mu_{lam}$ decreases rapidly as it approaches the wall, with minor differences between the two solvers in the near-wall region. Notably, the GSIS-SST solution predicts a higher $\mu_{lam}$ in the near wall region where turbulent mixing dominates, reflecting intensified energy exchange from hot outer flow to cold wall, which smooths out the temperature gradients across the flow field.
%The $\mu_{lam}$ at far field is low, and increases after the outer shock as temperature increases, finally falls when approaching the wall due to the low temperature jet flow near wall and the lowest temperature of wall. When $\text{PR}=1.5$, $\mu_{lam}$ increases at around $|x_2|=0.125~\text{m}$ (difference between GSIS and GSIS-SST solution is trivial here), a slight change in slope could be observed at $|x_2|=0.11~\text{m}$. Peak of $\mu_{lam}$ locates around $|x_2|=0.06~\text{m}$. The curves from GSIS-SST and GSIS both return to a small value at wall. Difference between GSIS-SST and GSIS is minor, the GSIS-SST curve always lies over the GSIS one until $|x_2|<0.045~\text{m}$ (as shown in detailed view of viscosity). As $x_2$ approaches wall, $\mu_{lam}$ from GSIS crosses that from GSIS-SST at around 0.01~m, and then quickly falls to the low value defined by wall temperature. The higher $\mu_{lam}$ of GSIS-SST prediction in this part of the curve comes intensified energy exchange, which evens the temperature difference across the flow field.
As the pressure ratio increases to $\text{PR}=2.5$, the $\mu_{lam}$ curves become more stretched in the $x_2$ direction, with the near wall cross-over point between the GSIS and GSIS-SST solutions shifting further away from the wall. This change is attributed to the increased jet flow injection into the near-wall region, which blocks the influence from outer hot free flow layer and thus mitigates the differences in viscosity predictions between the two solvers. These trends are further amplified at $\text{PR}=3.5$, where the viscosity profiles extend even further, showing an increased influence of the jet on the near-wall flow.
%When $\text{PR}=2.5$, the $\mu_{lam}$ curves are stretched in $x_2$ direction, and the cross points of both curves move further from the wall. The discrepancy between GSIS-SST and GSIS solutions also shrinks within $|x_2|<0.015~\text{m}$, since more jet flow is injected into the flow field and occupies the near wall region. These changes are also reflected in solution with $\text{PR}=3.5$. 
The turbulent viscosity $\mu_{turb}$ is derived from the GSIS-SST solution, and high in the far-field due to the boundary conditions in the free stream. As the flow approaches the outer shock, $\mu_{turb}$ decreases due to the faster rise in turbulent dissipation frequency ($\omega$) compared to turbulent kinetic energy ($k$), effectively decoupling boundary conditions' influence. At $\text{PR}=1.5$, $\mu_{turb}$ peaks at $|x_2|=0.105~\text{m}$, then decreases toward the shear layer. The shear layer, which is characterized by large velocity gradients, fosters the production of turbulent kinetic energy and an increase in turbulent viscosity (peaking at $|x_2|=0.009~\text{m}$) before the decay of $\mu_{turb}$ near the wall.

At higher pressure ratios (i.e., $\text{PR}=2.5$ and $\text{PR}=3.5$), the peak of $\mu_{turb}$ shifts outward and increases in the jet flow region. The peak near the wall at $\text{PR}=3.5$ reaches $\mu_{\text{turb}}=0.0331$, indicating stronger turbulent dissipation associated with amount of the jet flow.

The dominance of turbulent viscosity in the jet flow region, particularly at higher pressure ratios, highlights the importance of turbulence consideration in the near-wall flow, which substantially affects shear stress and heat transfer predictions.


This analysis reveals that in hypersonic flows with turbulent jets, the effective turbulence is primarily localized within the jet flow region and independent of free flow turbulence. Such effective turbulence is generated by unique mechanisms within the jet flow region, i.e. the jet Mach disk, the recompression shock, and downstream vortices, which exert a dominant influence on the flow field. This mechanism of turbulence production is distinct from the influence of free flow turbulence, which is overshadowed in these high-temperature, high-Mach environments.

%The distribution of $\mu_{turb}$ is obtained only from GSIS-SST solution, it possesses a high value at far field due to the boundary condition assigned to the free flow. It decreases before the outer shock. It is because earlier and faster rise of turbulent dissipation frequency $\omega$ than $k$. This observation removes the influence of boundary conditions on the flow field after the outer shock. When $\text{PR}=1.5$, the turbulent viscosity forms a small peak at around $|x_2|=0.105~\text{m}$, respecting the fact of turbulence generation after the shock. Since this peak, $\mu_{turb}$ diminishes as $|x_2|$ decreases until around 0.06~m approaching the shear layer between the free flow and the jet flow. The shear layer with large velocity gradient leads to the production of turbulent kinetic energy and therefore the increase of $\mu_{turb}$. The turbulent viscosity $\mu_{turb}$ climbs to a peak at $|x_2|=0.009~\text{m}$ and then approaching zero as the $k$ is to be dissipated on the wall. 
%When $\text{PR}=2.5$, the peak of $\mu_{turb}$ in the free flow region is moved further to around $|x_2|\approx0.135~\text{m}$. Massive production of $\mu_{turb}$ is expected in the jet flow region and is reflected in the figure. The peak at around $|x_2|=0.0117~\text{m}$ has a much larger value than the $\mu_{lam}$ peak, demonstrating the dominance of jet turbulence in this region.
%When $\text{PR}=3.5$, the peak of $\mu_{turb}$ near the wall is at $|x_2|=0.0122~\text{m}$, with $\mu_{turb}=0.0331$ at this peak, the $\mu_{r}$ reaches around 30.

% \subsection{Non-equilibrium effects}

% Since the GSIS-SST is a two temperature non-equilibrium solver, the non-equilibrium effect of the lateral jet flow field at high altitude is also examined. Figure~\ref{fig:H70TtTr} provides the contour of temperature ratio between translational temperature $T_t$ and the rotational temperature $T_r$. The figure employs a divergent color-map, with red indicating higher $T_t$ than $T_r$, blue representing higher $T_r$ over $T_t$ and white indicating equilibrium state between the two temperature. It is rather clear that in most of the area behind around the jet flow field, the translational temperature is well over the rotational one (of course they are in equilibrium in the far field). In the shock area, non-equilibrium is characterized by the larger $T_t$ than $T_r$, the barrel shock, the Mach disk, the separation shock and the recompression shock could all be identified by high temperature ratio in red. Just downstream the shock, $T_r$ takes over the region. \leir{Temperature ratio in blue mostly occupies region with strong expansion and low pressure. ??}

% With the pressure ratio increases, the non-equilibrium effect gets biased towards high temperature ratio, the expansion region colored in blue with higher $T_r$ than $T_t$ enlarges but the difference between the two temperature gets milder, suggesting a change towards local equilibrium.

% \begin{figure*}
%     \centering
%     {\includegraphics[width=0.33\linewidth]{Artworks/H70PR1.5TtTr.png}}
%     {\includegraphics[width=0.33\linewidth]{Artworks/H70PR2.5TtTr.png}}
%     {\includegraphics[width=0.33\linewidth]{Artworks/H70PR3.5TtTr.png}}
%     \caption{Contour of ratio between translational and rotational temperature with various pressure ratios (left: $\text{PR}=1.5$; middle: $\text{PR}=2.5$; right: $\text{PR}=3.5$).}
%     \label{fig:H70TtTr}
% \end{figure*}


\begin{figure}[h]
    \centering
    % {\includegraphics[width=0.49\linewidth,trim={20 20 30 90}, clip]{Artworks/H70PR1.5dRhoCP.png}}
    % {\includegraphics[width=0.49\linewidth, trim={20 20 30 90}, clip]{Artworks/H70PR3.5dRhoCP.png}}
    {\includegraphics[width=0.49\linewidth,trim={20 20 30 90}, clip]{Artworks/H70tauxy.png}}
    %{\includegraphics[width=0.49\linewidth,trim={50 70 50 90}, clip]{Artworks/H70PR2.5dRhoCP.png}}
    {\includegraphics[width=0.49\linewidth,trim={20 20 30 90}, clip]{Artworks/H70Q.png}}
    %{\includegraphics[width=0.49\linewidth, trim={50 70 50 90}, clip]{Artworks/H70PR3.5dRhoCP.png}}
    %{\includegraphics[width=0.49\linewidth,trim={20 20 30 90}, clip]{Artworks/H70RelDiffQ.png}}
    \caption{(Left) Surface shear stress $\sigma_{12}$ and (right) heat flux $Q$ with the jet pressure ratio.
    }
    \label{fig:H70tauQ}
\end{figure}

\subsection{Turbulence influence on surface quantities}
The cold jet in this study serves to reduce surface shear stress and heat flux. However, the turbulence associated with the jet significantly diminishes this reduction, affecting both magnitude and spatial extent. Notably, only the spatial extent of this effect varies with the pressure ratio $\text{PR}$.
% Intensity of friction reduction is independent of pressure ratio, extensity is highly dependent of PR.
% Larger PR maintains larger reduction range.


%The shear stress $\sigma_{12}$ on the model surface downstream the jet exit are plotted in the right top of figure~\ref{fig:H70dRho}. For all $\text{PR}$ values: $\sigma_{12}$ drops from a high positive value to some small negative level, \leib{oscillates between around 0 to -2.4 in the range of $0.1~\text{m}< x_1 <0.12\text{m}$, then generally climbs to local peak of around 1.3~2.2 and falls or rises depending on PR values when approaching the end of the model.}

The shear stress $\sigma_{12}$ distribution on the model surface downstream of the jet exit is shown in figure~\ref{fig:H70tauQ}. For all $\text{PR}$ values : $\sigma_{12}$ drops from a high positive level to a low negative one, oscillates between approximately 0 and -2 over in the range of $0.1~\text{m}< x_1 <0.13\text{m}$, then climbs to a peak of around 1.3–2.0 (depending on $\text{PR}$ and solver) before decreasing as it nears the model's end.

%\leib{Changes in $\sigma_{12}$ always starts earlier at lower than higher $\text{PR}$ in $x_1$ direction. The GSIS solution has a local peak around 2 at $x_1=0.15~\text{m}$ ($\text{PR}=1.5$) and then falls continuously until $x_1\approx0.5~\text{m}$. It then climbs up, signaling the degradation of the shear stress reduction effect from the jet. The GSIS-SST solution changes in a similar way as the GSIS one, yet with a higher local peak of around 2.2. And the GSIS-SST curve does not fall as much as the GSIS one, and starts to rise again from $x_1=0.228~\text{m}$, i.e., the GSIS-SST solver predicts a much shorter jet influencing range than the GSIS one. The discrepancy between the two curves are therefore quite substantial.

For lower $\text{PR}$, changes in $\sigma_{12}$ occur earlier along $x_1$ direction. At $\text{PR}=1.5$, the GSIS solution has a local peak around 1.7 at $x_1=0.165~\text{m}$, then declines constantly. The GSIS-SST solution shows a similar profile, with a slightly higher peak (~2.05) and a gentler decline, beginning to rise significantly again at approximately $x_1=0.45~\text{m}$, suggesting a shorter jet influence range than GSIS.

%When $\text{PR}=2.5$, the GSIS-SST and GSIS curves appear stretched in the $x_1$ direction compared to the $\text{PR}=1.5$ ones. The positive local peak has moved from $x_1=0.15~\text{m}$ at $\text{PR}=1.5$ to around $x_1=0.18~\text{m}$, and this peak of GSIS curve at $\text{PR}=2.5$ reaches only 1.7, while the GSIS-SST curve still has a 2.15 peak. Unlike the running of GSIS curve at $\text{PR}=1.5$, the GSIS curve at $\text{PR}=2.5$ drops to 1.4 at $x_1=0.245~\text{m}$, then increases until $x_1=0.35~\text{m}$ and drops all the way to the end of the model, implying the whole model enjoys the surface shear stress reduction effect of the jet. Again, the GSIS-SST solution gives different perception that the $\sigma_{12}$ is not reduced as much as GSIS predicted since $x_1>0.18~\text{m}$. The GSIS-SST curve rises unchangeably but less aggressive than the $\text{PR}=1.5$ one after dropping to 1.7 at 0.234~m, though still producing a significant deviation from the GSIS curve.
% but each reaching to a lower value than the $\text{PR}=1.5$ one near the end of the model. The GSIS-SST solution lies above the GSIS counterpart over the whole range of $x_1$ in the plot. Their differences starts obviously from the local peak at around 0.15~m, and diminish at $x_1\approx0.15$~m. until $x_1\approx0.5~\text{m}$, it gradually rises afterwards, marking a reduction in jet-induced shear stress

When $\text{PR}=2.5$, both curves appear stretched along $x_1$ direction compared to the $\text{PR}=1.5$ ones, with the GSIS peak shifting to around $x_1=0.2~\text{m}$. The GSIS peak is now lower at 1.5, while GSIS-SST holds steady at 2.0. Unlike at $\text{PR}=1.5$, the GSIS curve for $\text{PR}=2.5$ initially drops to 1.4 at $x_1=0.27~\text{m}$, then rising gradually until to $x_1=0.4~\text{m}$, and finally declines again, showing extended surface shear stress reduction. The GSIS-SST solution, however, suggests a weaker reduction ability as the curve lies over the GSIS one for a constant delta, also the secondary peak shifts slightly upstream to $x_1\approx0.37~\text{m}$, implying the degradation of reduction range.

%When $\text{PR}=3.5$, the curves of $\sigma_{12}$ resemble those at $\text{PR}=2.5$. The GSIS curve has now a further delayed and suppressed local peak of 1.33 at $x_1=0.214~\text{m}$. It also has a drop-rise-drop pattern and converges with the GSIS curve at $\text{PR}=2.5$ from $x_1>0.4~\text{m}$. The GSIS-SST prediction now shows a more obvious drop in the local peak value of 1.93 at $x_1=0.204~\text{m}$, agreeing with the local peak changing pattern from GSIS predictions, i.e., delay and drop with increasing $\text{PR}$ values. The rest of the curve still has an increasing trend toward the end of the model, but falls below the other two GSIS-SST curves, confirming that higher $\text{PR}$ creates more intense and longer lasting shear stress reduction.
For $\text{PR}=3.5$, the $\sigma_{12}$ curves resemble those at $\text{PR}=2.5$ but with further delayed and suppressed peaks. The GSIS peak shifts to 1.27 at $x_1=0.23~\text{m}$ with a drop-rise-drop trend, and overlaps with the other GSIS curves beyond $x_1>0.48~\text{m}$, where slight difference also exists: high $\text{PR}$ curves lie higher. The GSIS-SST solution at $\text{PR}=3.5$ exhibits a lower peak of 1.95 at $x_1=0.23~\text{m}$, generally overlaps with the $\text{PR}=2.5$ GSIS curve after $x_1>0.3~\text{m}$. 
%but maintains a rising trend towards the model's end, though below prior GSIS-SST curves, indicating that higher $\text{PR}$ enhances and prolongs shear stress reduction.

%exhibits larger deviation from the other tow pressure ratios. Compared to the GSIS-SST, the GSIS solution has a much larger local peak at around $x_1=0.2~\text{m}$ and a second peak at around 0.55~m. The GSIS-SST solution also presents a higher local peak at 0.2~m, but exhibits similar pattern as the lower pressure ratio GSIS-SST solutions after this peak. The stress level is also lower than the $\text{PR}=2.5$ GSIS-SST curve. 


Among these plots, it is also noticed that the peak value at around 0.2~m in GSIS reduces near linearly with increasing $\text{PR}$. The GSIS-SST groups always have a higher local peak, and a higher level following this peak. The variation of this local peak value in GSIS-SST with $\text{PR}$ is not as apparent as those in GSIS, whereas the peak location from both solvers does move further downstream as $\text{PR}$ increases. The GSIS solutions always produce a more aggressive suggestion on the intensity and extensiveness of shear stress reduction effect, while the GSIS-SST is more conservative, with the $\text{PR}=1.5$ GSIS-SST curve even considers such low pressure ratio is not able to serve the whole model.

%\leib{The relative difference in the integrated horizontal force $\text{Fx}_1$ over the model lower surface between GSIS and GSIS-SST is 24.2\%, 21.2\% and 20.1\% when PR=1.5, 2.5 and 3.5, respectively. }
%In contrast, the less viscous GSIS solution shows a similar pattern for PR = 1.5 and 2.5. However, the pattern for PR = 3.5 deviates, suggesting that the jet flow appears to repeatedly impinge on the model surface, leading to two distinct shear stress peaks.
As for the more sensitive index of surface heat flux, the picture is different. In GSIS solutions, there is always two local peaks in the range of $x_1=0.14~\text{m}$ to 0.2~m, due to less viscous separation and recompression process. The GSIS solutions also
predict a far longer ranger of heat flux reduction, only the curve with te lowest pressure ratio exhibits a slight recovery of surface heat flux on the downstream half of the model.
%Similar trends are observed for heat flux distribution, see the middle subfigure in the right column of Fig.~\ref{fig:H70dRho}.

In contrast, GSIS-SST is always the conservative one on predicting heat flux reduction extent and range, as the GSIS-SST curves have higher reattachment peaks and much earlier rise after the local peaks. The GSIS-SST curves rise significantly, with only the $\text{PR}=3.5$ curve ables to keep a lower heat flux level (similar as reattachment heat flux), but still far above the GSIS one.

About the quantified difference in heat flux between the two solvers, the GSIS prediction on heat flux is around $82\%\sim92\%$ lower than the GSIS-SST prediction at the end of the model.

The turbulence-induced differences between GSIS-SST and GSIS in the distribution of surface quantities can be categorized into three distinct stages. The first stage locates around the large downstream separation vortex, with turbulence significantly influences the positive peaks of surface quantities and relates to jet pressure ratio positively. The second stage occurs after flow reattachment along the middle portion of the flat surface, within which the turbulence effect stabilize. Finally, in the third stage, where the reduction effect diminishes toward the end of the model, the turbulence effect increases significantly as the pressure ratio decreases. These findings highlight the complex role of turbulence in shaping surface quantity distribution across different flow stages.

% The jet induced surface shear stress and heat flux reduction effect could be divided into three stages
% Based on the difference between GSIS-SST and GSIS, the turbulence induced difference could be divided into three stages, with the first stage happens around the large downstream separation vortex (around the positive peaks of surface quantities), the second stage starts after flow reattachment (middle part of the flat surface), the last one starts from where the reduction effect deteriorates (towards the end of the model). Jet pressure ratio enhances the turbulence effect in the first stage positively, while the turbulence effect stagnates in the second stage. And the turbulence effect increases largely with decreasing pressure ratio in the last stage.
%There is a clear non-linearity between the turbulence effect and the jet PR, e.g., the shear stress is largest in the intermediate PR. Reasons behind this might be that the macro flow pattern and micro turbulent mixing effect has different sensitivity to jet parameters. Further investigation into the influence of free flow Mach number, turbulent initial conditions and pressure ratios is worth-worthy. Since the largest deviations in the surface stress and heat flux between the GSIS-SST and GSIS simulations occur around $x_1=0.35$~m, in the following we focus on the analysis on this specific location.

\subsection{Integrated Forces and Moment}
Axial force is most influence by turbulence and such influence grows with increasing $\text{PR}$, while normal force and pitch moment from GSIS-SST and GSIS keeps a constant discrepancy.
\begin{figure}
    \centering
    {\includegraphics[width=0.32\linewidth]{Artworks/JetFx170.png}}
    {\includegraphics[width=0.32\linewidth]{Artworks/JetFx270.png}}
    {\includegraphics[width=0.32\linewidth]{Artworks/JetMx370.png}}
    \caption{Figures above give the integrated axial force $\text{Fx}_{1}$ (left), normal force $\text{Fx}_{2}$ (middle) and pitch moment $\text{Mx}_{3}$ (right) at 70~km with variation in pressure ratio $\text{PR}$. }
    \label{fig:FM70}
\end{figure}

The relationship between forces, moments, and the pressure ratio $\text{PR}$ is illustrated in Figure~\ref{fig:FM70} for the 70~km case. With increasing $\text{PR}$, the normal force $\text{Fx}_{2}$ and pitching moment $\text{Mx}_{3}$ both exhibit monotonic increases, while the axial force $\text{Fx}_{1}$ decreases slightly. The axial force with the jet on is notably lower than in the no-jet condition, confirming the effectiveness of the lateral jet in reducing frictional stress. The forces and moments relative to the nose tip scale nearly linearly with $\text{PR}$ across the range investigated. However, GSIS-SST consistently predicts higher values than GSIS, with discrepancies growing as $\text{PR}$ increases.

Quantitatively, the relative difference in $\text{Fx}_{1}$ between GSIS-SST and GSIS grows from less than 0.1\% at $\text{PR}=0$ to 13\% at $\text{PR}=1.5$, reaching around 19\% for $\text{PR}=3.5$. For the normal force $\text{Fx}_{2}$, GSIS-SST and GSIS results converge at $\text{PR}=0$, but the discrepancy for the jet cases stagnates around 10\% for all pressure ratios. Observation for $\text{Mx}_{3}$ shows similar pattern as $\text{Fx}_{2}$, where the relative difference lingers around $13\%\sim15\%$, with the maximum appears at $\text{PR}=2.5$, just as the case for $\text{Fx}_{2}$. The increasing relative difference of $\text{Mx}_{3}$ than $\text{Fx}_{2}$ also implies a constant shift of the aerodynamic center by turbulence influence.

The findings above suggest that the modeled turbulence influence scales with pressure ratio for the axial force, whereas its effect on the normal force, pitch moment, and the aerodynamic center remains unaffected by changes in pressure ratio. The reasons behind are that the axial force of current model is sourced only from surface friction, which is directly related to viscosity; while the normal force is surface pressure related, which is less sensitive to viscous influence, but determined by macroscopic flow structures.

% % \subsection{Force and Moment Augmentation Factors}
% Another key aspect which the aerospace engineers interest of is the force and moment augmentation factor $K$. It is defined as follows:
% \begin{equation}
% K=\frac{FM_{Wall,jet on}+FM_{jet}-FM_{Wall, jet off}}{FM_{jet}},
% \end{equation}
% here, quantity $FM$ could either be force or moment. %In this study, the force and moment here are only about the vertical force $\text{Fx}_2$, since the jet is placed also vertically and the lower surface is horizontal. The moments analyzed are in $x_3$ direction with two distinct centers of moment. The first one is a pitch moment (relative to nose-tip) serving for attitude adjustment (installment of the jet not aligning with vehicle center of mass), the second one is calculated to display the jet induced disturbance on attitude stabilization during orbital maneuver (jet exhausting axis crossing the center of mass). An interaction moment coefficient $Cim$ is defined as below to quantify the deviation of pitch moment from trimming condition caused by the jet. The results are plotted in the second column of figure~\ref{fig:FM}.
% In this study, we focus on the forces and moments generated by the lateral jet, primarily the vertical force $\text{Fx}_2$ and the moment $\text{Mx}_3$, which are critical for attitude control and stabilization. The pitch moment is evaluated relative to two reference points: the nose-tip, representing attitude adjustment, and the center of mass, reflecting disturbances during orbital maneuvers. To quantify deviations from trimming conditions caused by the jet, we define the interaction moment coefficient $Cim$ as follows:
% \begin{equation}
% Cim=\frac{M_{Wall,jet on}-M_{Wall, jet off}}{M_{Wall, jet off}},
% \end{equation}
% The results for $K_{Fx2}$, $K_{Mx3}$, and $Cim$ are summarized in Table~\ref{tab:ForceMoment} and plotted in Figure~\ref{fig:FM}.

% Both $K_{Fx2}$ and $K_{Mx3}$ decrease with increasing pressure ratio $\text{PR}$, reflecting a weakening influence of the lateral jet as $\text{PR}$ rises. For $K_{Fx2}$, the relative difference between GSIS-SST and GSIS reaches a peak of 16.1\% at $\text{PR}=2.5$, while for $K_{Mx3}$, the maximum overshoot is 28.1\% at the same pressure ratio. Notably, discrepancies in $K_{Mx3}$ remain significant at higher pressure ratios, reaching 27.9\% at $\text{PR}=3.5$. This saturation in augmentation factor differences may be attributed to insufficient model length to fully capture jet-induced effects at high $\text{PR}$.

% The interaction moment coefficient $Cim$ increases almost linearly with $\text{PR}$, with the relative difference between GSIS-SST and GSIS decelerating as $\text{PR}$ grows. This behavior is linked to a shift in the aerodynamic center: GSIS places it closer to the jet exit at higher $\text{PR}$, while GSIS-SST predicts a shift away from the jet exit, amplifying the lever arm and consequently the moment.

\section{The influence of AoA}\label{sec:AoA}

The AoA is varied among 0°, 15° and 30°, mimicking the maneuver of the hypersonic vehicles. The flight altitude is increased to 80~km, corresponding to Kn=0.0375 for the model in figure~\ref{fig:H70TtComment}, since attitude adjustment of hypersonic flight vehicles is more likely to happen at higher altitudes. The jet pressure ratio is kept at 2.5. 


\subsection{Flow structure}
At different angle of attack, the flow structures vary notably. The left column of figure~\ref{fig:H80dRho} illustrates the density gradient magnitudes, highlighting the progressive compression of the jet-controlled region as the AoA increases. This compression is accompanied by the shrink of the jet-controlled region, surrounded by streamlines emanating from the jet exit.

%As AoA increases, the interaction between the jet and the free stream intensifies due to the growing angle between their velocities. This transforms the interaction from a predominantly deflective mechanism to a collision-like interaction, resulting in stronger upstream disturbances, as evidenced by higher upstream pressure levels and a reduction in the size of the downstream separation vortex.

\begin{figure}
    \centering
    {\includegraphics[width=0.49\linewidth, trim={0 20 0 80}, clip]{Artworks/H80A0DissiQ.png}}
    {\includegraphics[width=0.49\linewidth, trim={0 20 0 80}, clip]{Artworks/H80A0TKEMuR.png}}\\
    % {\includegraphics[width=0.49\linewidth, trim={0 20 0 80}, clip]{Artworks/H80A15DissiQ.png}}
    {\includegraphics[width=0.49\linewidth, trim={0 20 0 80}, clip]{Artworks/H80AoA15dRhoCP3.png}}
    {\includegraphics[width=0.49\linewidth, trim={0 20 0 80}, clip]{Artworks/H80A15TKEMuR.png}}\\
    {\includegraphics[width=0.49\linewidth, trim={0 20 0 80}, clip]{Artworks/H80A30DissiQ.png}}
    {\includegraphics[width=0.49\linewidth, trim={0 20 0 80}, clip]{Artworks/H80A30TKEMuR.png}}
    \caption{(Left column) Contours of density gradient magnitude and streamlines at the altitude of 80~km, and AoA are 0° (top), 15° (middle) and 30° (bottom), with upper half from GSIS and lower half from GSIS-SST. (Right column) Contours of turbulent kinetic energy (upper half) and turbulent-to-laminar viscosity ratio (lower half) from GSIS-SST at 80~km and AoA=0° (top) and 30° (middle), with upper half from GSIS and lower half from GSIS-SST. (Right column, bottom) Contour of viscous dissipation rate and streamlines colored in Q criterion at 80~km and AoA=30°, with upper half from GSIS and lower half from GSIS-SST. 
    }
    \label{fig:H80dRho}
\end{figure}

At AoA = 0°, the upstream vortex is weak, but the recirculation region is extensive. A secondary upstream vortex also develops, reaching its largest size at this AoA. Downstream of the jet exit, the expansive jet flow prevents free-stream reattachment to the surface, resulting in dominant jet behavior in the near-wall region and making it difficult to define the penetration height. A large downstream vortex is also observed in this configuration.

At AoA = 15°, the upstream vortices reach their maximum size due to enhanced shear between the jet and free stream, which generates increased vorticity and promotes vortex growth. However, as AoA increases further, the intensified interaction compresses the vortices, limiting their rotational freedom. This compression represents a balance between shear-driven vortex growth and the constraining effects of excessive strain, which suppresses further development of vortices.

Comparing GSIS-SST and GSIS models reveals that turbulence plays a critical role in regions of strong shear and vortex dynamics. Turbulence helps stabilize and organize vortices, even under conditions of intensified stretching and high shear at larger AoAs.% These effects contribute to the observed variations in downstream separation pressure, as depicted in the last sub-figure of figure~\ref{fig:H80dRho}.


\subsection{Turbulent Quantities}
More and more concentrated and intense turbulent kinetic energy and turbulent-to-laminar viscosity ratio are observed as AoA increases.

At AoA = 0°, a high TKE region forms around the Mach disk, where the small angle between the free stream and jet flow allows the jet to expand with minimal compression, leading to low TKE production outside this region. A strip of large TKE appears along the stretching direction of the downstream vortex, driven by sharp velocity gradients in the developing near-wall boundary layer, most notably at AoA = 30°.

The turbulent viscosity ratio ($\mu_r$) follows the TKE distribution, peaking in jet-dominated regions and vanishing where the free stream dominates, due to the higher post-shock temperature. This indicates that turbulence is localized near high-gradient flow features and is independent of far-field conditions, highlighting the turbulence model’s sensitivity to localized effects.

Turbulence also affects vortex dynamics. At AoA = 0°, the downstream vortex shrinks and its high-Q region contracts slightly compared to the laminar GSIS solution, which stretches further. This suggests that the absence of turbulent dissipation in GSIS leads to a less stable vortex. In the downstream vortex, stretching converts rotational energy into TKE, enhancing viscous dissipation and explaining the differences between GSIS and GSIS-SST results.

As AoA increases, TKE production intensifies near shock structures, except around the Mach disk, where it drops. This drop is due to the reduced jet expansion at higher AoA, which decreases the shock front Mach number and weakens the Mach disk. Additionally, a intensified strip of TKE and $\mu_{r}$ extends from the stretched vortex to the downstream boundary layer, implying growing turbulence influence with higher AoAs.


%\subsection{\leib{Turbulent Quantities and Vortex}}
%\leib{The distribution of turbulent quantities, such as turbulent kinetic energy (TKE) and turbulent viscosity ratio ($\mu_{r}$), reveals distinct patterns across different angles of attack (AoA), as shown in figure~\ref{fig:H80DissQ}. 


% \begin{figure}
%     \centering
%     % {\includegraphics[width=0.49\linewidth]{Artworks/H80A0TKEMuR.png}}
%     % {\includegraphics[width=0.49\linewidth]{Artworks/H80A0DissiQ.png}}\\
%     % {\includegraphics[width=0.49\linewidth]{Artworks/H80A15TKEMuR.png}}
%     % {\includegraphics[width=0.49\linewidth]{Artworks/H80A15DissiQ.png}}\\
%     {\includegraphics[width=0.49\linewidth]{Artworks/H80A0TKEMuR.png}}
%     {\includegraphics[width=0.49\linewidth]{Artworks/H80A30TKEMuR.png}}
%     {\includegraphics[width=0.49\linewidth]{Artworks/H80A30DissiQ.png}}
%     \caption{(Left) Contours of turbulent kinetic energy (upper half) and turbulent-to-laminar viscosity ratio (lower half). 
%     (Right) Contours of viscous dissipation rate $\epsilon$ and streamlines colored with Q-criterion, GSIS solution is shown in the upper half and GSIS-SST is in the lower half of these figures.  Flight altitude is 80~km, and AoA are 0° and 30° (from top to bottom for each row).
%     }
%     \label{fig:H80DissQ}
% \end{figure}
% At AoA = 15°, the TKE distribution changes significantly. While the TKE around the Mach disk weakens, higher TKE emerges near other shock structures, such as the separation shock, outer shock, and recompression shock, which intensify at higher AoAs. Additionally, a strip of large TKE appears along the stretching direction of the large downstream vortex, driven by the sharp velocity gradients in the developing near-wall boundary layer.

% The turbulent viscosity ratio ($\mu_{r}$) closely mirrors the TKE distribution in regions dominated by jet flow but vanishes in areas governed by the free stream, again due to the larger increase in post shock temperature. This highlights the localized influence of turbulence near high-gradient flow features and colder area, also the independence of far-field initial conditions for turbulence model.

% The effects of turbulence on vorticity are also notable. At AoA = 0°, the downstream vortex shrinks, with its high-Q region contracting slightly compared to the laminar GSIS solution, where the vortex stretches further. This reflects the less stable nature of GSIS solution in the absence of turbulent dissipation. Also in the downstream vortex, vortex stretching dominates energy transfer, converting rotational energy into TKE, which in turn enhances viscous dissipation and drives the observed differences between GSIS and GSIS-SST solutions.

% At AoA = 15°, the upstream vortex from GSIS-SST has higher Q but is reduced in size due to stronger compression, while the downstream vortex shrinks further and shifts upstream closer to the jet exit. The downstream vortex also deforms along the main flow direction, a trend that persists at AoA = 30°. 

% Combining the observations above, consistent patterns emerge as AoA increases: TKE production intensifies near shock structures, except around the Mach disk, where TKE drops. This drop can be attributed to the reduced expansion of the jet flow at higher AoA, since the shock front Mach number is largely decreased, thus the intensity of the Mach disk. Additionally, a TKE production strip extends from the center of the stretched downstream vortex to the adjoining boundary layer, reflecting the combined effects of vortex stretching and boundary layer development.
% }



\subsection{Profiles of field quantities}

To compare GSIS-SST and GSIS, we examine the shear stress components: laminar ($\sigma_{12,lam}$), turbulent ($\sigma_{12,turb}$), and rarefaction-induced ($\sigma_{12,HoT}$) at $x_1=0.35~\text{m}$, as shown in figure~\ref{fig:H80Proftxy}. The contribution of turbulence to shear stress is seen located in the near wall jet flow layer, and rises as AoA goes up. 
\begin{figure}
    \centering
    \vspace{0.3cm}
    \subfloat[AoA= 0°]{\includegraphics[width=0.32\linewidth]{Artworks/H80AoA0Proftxy.png}}
    \subfloat[AoA= 15°]{\includegraphics[width=0.32\linewidth]{Artworks/H80AoA15Proftxy.png}}
    \subfloat[AoA= 30°]{\includegraphics[width=0.32\linewidth]{Artworks/H80AoA30Proftxy.png}}
    \caption{The GSIS-SST results of the NS laminar, turbulent and rarefied parts of shear stress at $x_1=0.35~\text{m}$ at the altitude of 80~km.
    }
    \label{fig:H80Proftxy}
\end{figure}
At AoA = 0°, $\sigma_{12,lam}$ has three peaks: at $|x_2|=0.2~\text{m}$ (outer shock), $|x_2|=0.08~\text{m}$ (shear layer), and near the wall. $\sigma_{12,turb}$ is negligible except within the jet boundary layer, where it matches $\sigma_{12,lam}$ at $|x_2|=0.013~\text{m}$. The rarefaction-related stress $\sigma_{12,HoT}$ affects both the far-field and the shock, but negatively impacts the region between the shock and $|x_2|<0.05~\text{m}$, with a negative influence near the wall causing velocity slip.

At higher AoAs, stress components shift closer to the wall, with $\sigma_{12,lam}$ and $\sigma_{12,turb}$ extending rightward due to increased compression and shear. $\sigma_{12,HoT}$ also increases, extending further into the outer shock region, but its negative portion diminishes as the rarefaction effects reduce.

Near the wall, both $\mu_{lam}$ and $\mu_{turb}$ increase at high AoAs, as shown in figure~\ref{fig:H80Viscosity}. The rise of $\mu_{lam}$ could be attributed by higher temperature gradient, and $\mu_{turb}$ of GSIS-SST further intensifies the rise of $\mu_{lam}$, shaping the displayed difference between GSIS-SST and GSIS. The $\mu_{turb}$ increases obviously in maximum magnitude, yet the influential range shrinks abruptly as AoA grows over 0°, and stays similarly for AoA=15° and 30°.

This suggests that turbulence enhances momentum and energy exchange at specific locations as AoA increases, but its overall significance may be difficult to estimate as AoA increases, especially within AoA=0° to 15°. The surface shear stress and heat flux distribution in the next part provide then more information.



\begin{figure}
    \centering
     %\subfloat[AoA=0°]{\includegraphics[width=0.32\linewidth]{Artworks/H80AoA0ProfVis.png}}
     %\subfloat[AoA=15°]{\includegraphics[width=0.32\linewidth]{Artworks/H80AoA15ProfVis.png}}\\
    \subfloat[Laminar viscosity]{\includegraphics[width=0.37\linewidth]{Artworks/H80ProfVisDetail2.png}}
    \subfloat[Turbulent viscosity (GSIS-SST)]{\includegraphics[width=0.37\linewidth]{Artworks/H80ProfVisDetailTurb.png}}
    \caption{Profile of viscosity at $x_1=0.35~\text{m}$ at altitude 80~km. 
    } 
    \label{fig:H80Viscosity}
\end{figure}

%This is reflected in the $\mu_{lam}$ profile, where significant discrepancies between GSIS-SST and GSIS arise near wall. As AoA increases and compression intensifies, turbulence amplifies the differences of $\mu_{lam}$ near the wall but in a shorter range. Therefore, the difference 

%At higher angles of attack (AoA), turbulent viscosity ($\mu_{turb}$) remains constant, but its influence diminishes as the jet becomes more confined near the wall. Laminar viscosity ($\mu_{lam}$), on the other hand, increases more rapidly with AoA due to compression and enhanced temperature gradients, reducing the relative contribution of turbulence.




\subsection{Turbulence influence on surface quantities}
Sensible discrepancies on surface shear stress and heat flux are also noticed across different angles of attack even at 80~km. 

Figure \ref{fig:H80tauxy} illustrates the surface shear stress $\sigma_{12}$ on the lower surface downstream of the jet exit, a negative peak at around 0.15~m could be seen and scales with increasing AoA. At AoA = 0°, $\sigma_{12}$ exhibits a comparable pattern to the results at 70~km altitude shown in figure \ref{fig:H70dRho}, with a distinct local positive peak around $x_1 = 0.23~\text{m}$ followed by a steady decrease. At AoA = 15°, the peak shifts closer to the jet exit, around $x_1 = 0.19~\text{m}$, and the stress gradually declines downstream. For AoA = 30°, such positive peak shifts again downstream, but the local peak at $x_1 = 0.2~\text{m}$ is less pronounced in GSIS solution. Across all cases, the GSIS-SST solution consistently predicts higher values of $\sigma_{12}$ compared to GSIS. The difference induced by turbulence around the positive peak correlate positively with AoA, while on the aft section of the model, relationship between the turbulence influence and AoA gets hard to decide. 

The second figure of figure~\ref{fig:H80tauxy} shows surface heat flux distributions. A local peak is present near $x_1 = 0.16\sim0.20~\text{m}$ across all AoAs, but its prominence diminishes as the AoA increases. At AoA = 0°, this peak (located around $x_1 = 0.20~\text{m}$) is the global maximum within the plotted range. Heat flux drops significantly downstream in GSIS but rises slightly in GSIS-SST, indicating enhanced mixing and degraded cooling effect in the latter. At AoA = 15°, the heat flux climbs again after the local peak, which becomes smaller relative to the heat flux near the end of the model (even falls below that in GSIS-SST). This trend intensifies at AoA = 30°, with the local peak flattening further, and the curve rises considerably. The GSIS-SST curve also deviates substantially from the GSIS one. The relative difference of heat flux between the solvers rest around $30\%\sim40\%$, generally increase together with AoA. 

As described above, the difference between GSIS-SST and GSIS solutions is evident in both shear stress and heat flux. GSIS-SST consistently predicts higher values due to the influence of turbulence, which enhances mixing and increases effective viscosity near the wall. %For heat flux, GSIS prediction on heat flux is at most 40\% smaller than the GSIS-SST ones, with the location of the maximum difference shifting from $x_1 = 0.72~\text{m}$ to 0.25~m as AoA increases.% At AoA = 0°, the difference peaks at $x_1 = 0.72~\text{m}$, moving to $x_1 = 0.40~\text{m}$ at AoA = 15° and $x_1 = 0.25~\text{m}$ at AoA = 30°. This upstream shift reflects the increasing dominance of convective effects at higher AoAs, which enhance heat transfer near the jet exit.

For integrated forces and moment under varying AoA, the largest discrepancy between GSIS-SST and GSIS occurs at AoA=30°, where a 5\% difference in the axial force $Fx_{1}$ is observed, a faint positive relation between AoA and such difference could be noticed, this observation proved the inference based on the $\mu_{turb}$ profile in the previous part. And for the normal force and pitch moment, no sensible difference between GSIS-SST and GSIS is identified at 80~km.

The observed changes in surface quantities again confirm the positive relation between turbulence influence and angle of attack. As AoA increases, the the jet flow bends sharply and impinges on the wall heavily, compressing the jet-controlled area, promoting development of thinner boundary layer and higher gradients, producing thus more turbulence kinetic energy and influence.
%reflect the complex interplay between turbulence and convection process. At low AoA, turbulence dominates a wider range with space for diffusion to progress, yet with a reduced intensity. While at high AoA, its intensity increases as convection brings higher gradients, but the convection process also constraints the turbulent diffusion, limiting its range of significance. Such effects combining together, resulting into hardly identifiable relation between turbulence and angle of attack.
%enhancing mixing and promoting higher shear stress and heat flux, as evident in the GSIS-SST results. The relatively parallel alignment of the jet flow, free stream, and surface downstream allows turbulence to develop efficiently, sustaining energy and momentum transfer. As AoA increases, the jet flow bends sharply and impinges on the wall, amplifying strain rates and convective transport while constraining turbulence-dominated mixing regions. This shifts dominance toward laminar effects, as $\mu_{lam}$ scales with temperature and increases significantly due to higher compression and temperature gradients, while $\mu_{turb}$ remains nearly constant. Although turbulence influence remains locally significant in regions such as shock-induced vortices and boundary layers, the overall role of turbulence in these flows weakens at large AoAs.

%As pressure ratio stays the same, mu turb does not changes much in the near wall layers as shown previously, while the mu lam scales with temperature which gets significantly higher under compression at high AoA and also the enhanced energy exchange attribute to mu turb. In summary, low AoA mu turb dominates, high AoA velocity gradient increases, mu turb increases, increase of mu turb enhances also temperature gradient, thus boosting mu lam, weakening influence from turbulence. 

%Turbulence remains influential in localized regions, particularly around shock-induced vortices and boundary layers. However, the increased dominance of convection at higher AoAs reshapes the distribution of shear stress and heat flux, leading to upstream shifts of key features and a flatter heat flux profile near the jet exit. These trends underscore the dynamic balance between turbulent mixing, strain-driven effects, and convective transport as AoA varies.


\begin{figure}
    \centering
    \includegraphics[width=0.49\linewidth,trim={20 20 30 90},clip]{Artworks/H80txy.png}
    \includegraphics[width=0.49\linewidth,trim={20 20 30 90},clip]{Artworks/H80Q.png}
    % \includegraphics[width=0.32\linewidth]{Artworks/H80AoA0txy.png}
    % \includegraphics[width=0.32\linewidth]{Artworks/H80AoA15txy.png}
    % \includegraphics[width=0.32\linewidth]{Artworks/H80AoA30txy.png}\\
    %    \vspace{0.5cm}
    % \includegraphics[width=0.32\linewidth]{Artworks/H80AoA0Q.png}
    % \includegraphics[width=0.32\linewidth]{Artworks/H80AoA15Q.png}
    % \includegraphics[width=0.32\linewidth]{Artworks/H80AoA30Q.png}
    \caption{Variation of surface shear stress and heat flux at altitude 80~km with AoA.
    }
    \label{fig:H80tauxy}
\end{figure}
% (from left to right)
% For varying AoA, the largest discrepancy between GSIS-SST and GSIS occurs at AoA=0°, where a 4\% difference in $Fx_{1}$ is observed. This highlights the sensitivity of axial force predictions to turbulence effects at small angles of attack.
% \begin{table}
%     \centering
%     \begin{tabular}{cllcllcllll}\hline
%          Altitude& AoA&PR&  SST& $Fx_1$&$Fx_2$&  $Mx_3$ &$Mjx_3$ &$K_{Fx2}$ & $K_{Mx3}$&$Cim$\\ \hline

%  80 km& 0°& 2.5& 0 & 2.86& 48.03 & 15.41 &10.51 &4.34 & 10.98 &1.744\\ 
% & & & 1& 2.97& 48.08 &15.49 &10.59 &4.35 & 11.06 &1.764\\
%  & & &RelDiff & 3.9\%& 0.1\% &0.5\% &0.8\% &0.1\% & 0.8\% &1.1\%\\

%  & 15°& & 0 & 8.02 & 123.67 &42.26 &29.65 &5.20 & 13.64 &0.401\\
% & & & 1 & 8.26 &124.11 &42.33 &29.67 &5.24 &13.70 &0.402\\
%  & & &RelDiff & 3.0\% &0.4\% &0.2\% &0.1\% &0.8\% & 0.4\% &0.2\%\\

%  & 30°& & 0 & 12.82 & 283.10 &100.78 &71.90 &5.24 &10.98 &0.087\\ 
% & & & 1& 13.20& 282.78 &100.40 &71.55 &5.19 & 10.57 &0.082\\
%  & & &RelDiff & 3.0\% &-0.1\% &-0.4\% &-0.5\% &-0.8\% &-3.7\% &-6.4\%\\ \hline
%     \end{tabular}
%     \caption{Axial force $Fx_1$, normal force $Fx_2$, pitch moment $Mx_3$ (relative to nose-tip), $Mjx_3$ (relative to jet center) and corresponding augmentation factors $K$ at 80~km. Condition flags same as previous that in previous rows are omitted. Rows with SST flag equals 0 list GSIS results, while with flag 1 list GSIS-SST results. The rows start with RelDiff provides the relative difference of quantity of interest (QoI) from GSIS-SST (1 row above) relative to GSIS (2 rows above), i.e., $QoI_{GSIS-SST}/QoI_{GSIS}-1$.}
%     \label{tab:ForceMoment}
% \end{table}

%\subsection{Integrated Force and Moments}
%For integrated forces and moment under varying AoA, the largest discrepancy between GSIS-SST and GSIS occurs at AoA=30°, where a 5\% difference in $Fx_{1}$ is observed, a faint positive relation between AoA and such difference could be noticed. %This highlights the sensitivity of axial force predictions to turbulence effects at small angles of attack.

%The influence of angle of attack (AoA) is interwoven with $\text{PR}$ effects. For example, at 80~km, augmentation factors display non-linear behavior with AoA, but the percentage differences between GSIS-SST and GSIS remain minor, typically under 4\%. This suggests an indirect relationship between turbulence and AoA in shaping the augmentation factors, primarily mediated by changes in flow alignment and jet penetration. Given the limited impact, these results are included here for completeness.

==> bk2.tex <==
% The flow structures are shown first to present the macroscopic change, then the turbulent quantities are analyzed to explain such changes, followed by their impact to the surface quantities and the integrated force and moments.


% \subsection{Flow structure}

% \begin{figure}[h]
%     \centering
%     \subfloat[$\text{PR}=1.5$]{\includegraphics[width=0.49\linewidth,trim={20 40 30 90}, clip]{Artworks/H70PR1.5dRhoCPQ.png}}
%     \subfloat[$\text{PR}=3.5$]{\includegraphics[width=0.49\linewidth, trim={20 40 30 90}, clip]{Artworks/H70PR3.5dRhoCPQ.png}}
%     \caption{Magnitude of density gradient and streamlines colored with Q-criterion. 
%     GSIS and GSIS-SST solutions are shown in the upper and lower half of each figure, respectively. %Flight altitude is 70~km, AoA=15°.
%     }
%     \label{fig:H70dRho}
% \end{figure}

% Figure~\ref{fig:H70dRho} displays the density gradient contour from GSIS and GSIS-SST.
% As the PR is varied from 1.5 to 3.5, the overall structure of flow field remains consistent with the analysis presented in figure~\ref{fig:H70TtComment}, except that 
% the jet flow occupied area is  enlarged. 


% The streamlines, which are colored in Q-criterion~\citep{Jeong1995On}, are also compared. 
% The Q-criterion is defined to be $0.5(\|\bm{\Omega}\|^2-\|\ \textbf{S}\|^2)$, with $\bm{\Omega}$ and $\textbf{S}$ each being the anti-symmetric and symmetric part of the velocity gradient tensor.
% A positive value of Q indicates that the local flow structure is dominated by rotation, and a negative value suggests that strain dominates over rotation. Figure~\ref{fig:H70dRho} shows that, the upstream separation area is almost identical between GSIS and GSIS-SST. 
% In the downstream separation area, however,
% the downstream vortex in GSIS is less diffusive than the GSIS-SST even at the lowest PR, as it has a more concentrated core with higher Q. By probing at around the vortex core, it is found that the Q-criterion from GSIS-SST in the large downstream vortex is lower or more evenly distributed, since the additional turbulent viscosity helps with vorticity diffusion. 
% The vortex in GSIS is also prone to vortex deformation and breaks into smaller vortex more easily. The derived secondary vortex exists between the large downstream vortex and the wall in GSIS solution (rests around $x_1=0.11~\text{m}$, at PR = 1.5), but is absent in GSIS-SST result, until PR is increased to 3.5.
% These observations well demonstrate the low stability nature of the less viscous GSIS solution, compared with turbulence statistically modeled GSIS-SST.


\section{The influence of jet PR}\label{sec:PR}

Three jet PRs (i.e., PR=1.5, 2.5, and 3.5) are considered at AoA=15° and an altitude of 70 km, at which both rarefaction and turbulence effects are significant. As the jet ratio is directly related to the density of the jet flow, and consequently the turbulent viscosity, varying $\text{PR}$ enables a comprehensive analysis of turbulence's impact on the flow field across varying intensities. 

\subsection{Turbulence influence on surface quantities}


In the GSIS solutions, the shear stress curves oscillate in the range of $0.1~\text{m}< x_1 <0.15~\text{m}$, then climbs to a positive peak before decreasing as it nears the model's end. As the jet controlled area increases with the PR, the shear stress curve stretches horizontally.
The GSIS-SST curves share the same pattern as the GSIS, but the largest discrepancy between GSIS-SST and GSIS occurs at the rear of the model, where the relative difference reaches 127\%. The distribution of normal force is similar to that of the shear stress, with maximum relative difference between GSIS-SST and GSIS reaching 20\%. 

\begin{figure}
    \centering
    {\includegraphics[width=0.32\linewidth]{Artworks/H70tauxy2.png}}
    {\includegraphics[width=0.32\linewidth]{Artworks/H70tauyy2.png}}
    {\includegraphics[width=0.32\linewidth]{Artworks/H70Q2.png}}
    {\includegraphics[width=0.32\linewidth]{Artworks/JetCFx170.png}}
    {\includegraphics[width=0.32\linewidth]{Artworks/JetCFx270.png}}
    {\includegraphics[width=0.32\linewidth]{Artworks/JetCMx370.png}}
    \caption{(First row) Surface quantities at different jet PR. 
    The shear stress $\sigma_{12}$ and normal force are normalized by free flow pressure $p$, while the heat flux $q$ is normalized by $p\sqrt{RT}$. (Second row) Variations of the  integrated axial force, normal force and pitch moment with respect to PR. The force coefficients are forces normalized by $0.5\gamma p\text{Ma}^2\ell$.
    }
    \label{fig:H70tauQFM}
\end{figure}

The integrated forces and pitch moment are compared in the second row of figure~\ref{fig:H70tauQFM}, as a function of the PR. 
Predictions from GSIS-SST on the axial force coefficient are almost constantly $0.0013$ higher than the GSIS ones, and thus building up an increasing relative difference due to the general decreasing trend when PR rises, i.e. nearly zero at $\text{PR}=0$ to 13\% at $\text{PR}=1.5$, reaching around 19\% for $\text{PR}=3.5$.
% The normal forces and pitch moment scale also nearly linearly with $\text{PR}>1.5$. However, 
Meanwhile, GSIS-SST consistently predicts higher values than GSIS on coefficients of normal force and pitch moment, with discrepancies growing as $\text{PR}$ increases. 
% Different from the axial force, the absolute discrepancy of normal force between GSIS-SST and GSIS grows with PR, while 
The relative difference for normal force coefficient stagnates around 10\% for all PRs, due to increase also in normal force. Similar pattern applies for the pitch moment coefficient, whose relative difference lingers around $13\%\sim15\%$ (peaks at $\text{PR}=2.5$).
%with the maximum appears at $\text{PR}=2.5$. 
% the increased relative difference than normal force implies a shift of the aerodynamic center by turbulence influence.


% The surface heat flux experiences significant influence from turbulence modeling. 
On surface heat flux, the GSIS  predicts a far longer range of heat flux reduction after initial positive peaks, only the curve with the lowest PR exhibits a slight recovery of surface heat flux on the downstream half of the model.
On the contrary, GSIS-SST predicts higher positive peaks and much earlier rise after the local peaks, i.e., at the end of the model, the heat flux in GSIS-SST is around 5 to 12 times higher than the GSIS. This indicates the turbulence effects weaken the jet's capability in thermal protection.

% The findings above suggest that the modeled turbulence influence scales with PR for the axial force, whereas its effect on the normal force, pitch moment, and the aerodynamic center remains unaffected by changes in PR, for current model. The difference originates from the imparity between the turbulence influence versus PR and the overall effect of lateral jet versus PR. The former has been explained with the three stages analysis for its complex relation with PR, while the latter is straightforward as the jet serves to reduce shear stress, and builds normal force and pitch moment, thus shaping distinct relative influence of turbulence on them.

%It is seen from above that the turbulence effect changes in a slow pace with PR, while the forces and moment change fast and divergently, thus shaping different trends of relative turbulence influence.

% of turbulence thus increases with PR, while stagnates for normal force and moment.
% The reasons behind are that the axial force of current model is sourced only from surface friction, which is directly related to viscosity; while the normal force is surface pressure related, which grows in a faster pace than the observed turbulence augmentation. 
%is less sensitive to viscous influence, but determined by macroscopic flow structures.

\subsection{Turbulent Quantities}
%negative part of sig12, turbulence reduce rotation, vel gradient, thus positively shift shear stress. positive part, turb vis build up, increasing shear stress, reaching max after reattachment, while Q max out at reattachment point. afterwards, mut production, velgrad reduction, shaping somehow stable effect, until jet gets too dispersed and loses reduction effect totally.
%near wall velgrad increases as boundary layer develop (greater than GSIS) velgrad in field smooth, mur decreases mulam smooth out
%PR1.5 goes up, jet flow layer gets hot much faster than 2.5 3.5





% \leir{shorten this paragraph, apparently the next paragraph is more important} 
%High TKE production scales positively with PR and could be observed across the lateral jet flow field, particularly around shocks and shear layers.
% Shear layer between the jet flow and the post-shock free flow also produces large amount of TKE, so is the reattachment shock.% Coming then to the reattachment shock, TKE is significantly produced in the post-shock free flow side, and then merges with those from shear layer. 
% Moving toward the jet area, apparent boundary of high TKE exists, disconnecting the two regions.
%Apparent boundary of high TKE around the shear layer disconnects the jet and free flow regions.
% The expected turbulent jet flow does not predominantly carry TKE as one might anticipate prior to computation, if compared to the huge amount of TKE from post-shock free flow. 
%Within the jet flow area, TKE is massively generated downstream the Mach disk and within the separation regions due to high strain-rate, i.e. the small upstream vortex left to the jet and the large downstream vortex.%, as in figure~\ref{fig:H70dRho}.
% Such production scales positively with PR.
% The near-wall region exhibits a low magnitude of TKE due to the turbulent dissipation enforced by the boundary conditions. 
 

  
To understand how the difference between GSIS and GSIS-SST arises, we examine the turbulent-to-laminar viscosity ratio $\mu_r$, which determines the actual significance of turbulence. It is seen from figure~\ref{fig:H70mu_r} that, 
the presumed turbulent jet carries high $\mu_{r}$ into the flow field. $\mu_r$ decreases slightly in the jet expansion fan, but is enhanced through the barrel shock and Mach disk.
In addition, high $\mu_{r}$ could be observed after the jet flow passes through the reattachment shock and reattaches the model surface. Strip-like structures of high $\mu_{r}$ form near the wall and extend far downstream, responsible for turbulence related difference between GSIS and GSIS-SST. 
% The strips come from two sources of high effective TKE: the downstream large vortex (at around $x_1\approx0.12~\text{m}$, TKE produced from vortex elongation) and the jet (TKE from boundary condition, Mach disk and reattachment shock).
The $\mu_{r}$ dictated area grows with increasing $\text{PR}$.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth,trim={0 10 10 440}, clip]{Artworks/H70J2_5MuR.png}
    \caption{Contours of the turbulent-to-laminar viscosity ratio rom GSIS-SST, when the PR is 2.5. 
    }
    \label{fig:H70mu_r}
\end{figure}

\leib{explain the pattern before positive peaks}
When PR increases, the downstream separation counter-clockwise vortex grows bigger, near wall velocity gradient and $\mu_{lam}$ both reduce, shaping the right and upward shift of local negative peak in shear stress. With turbulence considered, the velocity gradients near wall are further smoothed through turbulence mixing by $\mu_{turb}$, providing further upward but reduced shifts by turbulence in shear stress around negative peaks, as PR goes up. Meanwhile, the turbulence influence on positive peak scales with PR due to stronger reattachment shock. Similar reasons apply for normal force and heat flux too.%However, the large vortex at high PR does produce more TKE in larger area. These turbulence leads to the positive relation between turbulence and PR before the local positive peaks.

% makes the shift of positive peak from GSIS to GSIS-SST in shear stress, normal force and heat flux grow as PR increases.

% and heat flux. However, larger vortex promotes turbulence production, the additional $\mu_{turb}$ smooths the temperature field, increases $\mu_{lam}$, making the a positive 
% and promotes turbulence production. The produced turbulence in turn pulls up shear stress through $\mu_{turb}$.


\leib{middle part of the curves, coexistence of turb and rare}
To deeper understand the physics of how turbulence and PR affect the flow field after flow reattachment, we investigate in figure~\ref{fig:H70Vis} the profiles of velocity, shear stress and viscosity at $x_1=0.35~\text{m}$ with PR=1.5, where the jet has reattached on the model surface and a proper boundary layer has been formed.  
% At the sampling location shown in figure~\ref{fig:H70Vis}(a), 
Distinct flow layers are established and marked in figure~\ref{fig:H70Vis}(a), difference between GSIS-SST and GSIS starts to emerge around the indistinct shear layer, since $\mu_r$ is only significant near wall (figure~\ref{fig:H70mu_r}). %corresponding to the $\mu_r$ distribution in figure~\ref{fig:H70mu_r}. 
% It is clearly seen that, the outer shock is largely blurred due to gas rarefaction. Below the also indistinct shear layer, the difference between GSIS-SST and GSIS starts to emerge, due to the turbulence influence as shown in figure~\ref{fig:H70Vis}(b-c). 

% The contributions to shear stress from different physical processes are shown in figure~\ref{fig:H70Vis}(b). The laminar part peaks at the outer shock, the shear layer and the near-wall layer. Together with figure~\ref{fig:H70Vis}(c), the appearance of these peaks are clear: increase in post-shock temperature pulls up $\mu_{lam}$, high velocity gradient across shock and shear layer make up high $\sigma_{12,lam}$, and the near-wall velocity gradient excites production of $\sigma_{12,lam}$ despite drop in $\mu_{lam}$. 


\begin{figure}[h]
    \centering
    {\includegraphics[width=0.32\linewidth]{Artworks/H70PR1_5VelMa2.png}}
    \includegraphics[width=0.32\linewidth]{Artworks/H70PR1_5txy.png}
    \includegraphics[width=0.32\linewidth]{Artworks/H70PR1_5Vis2.png}
    \caption{Macroscopic flow quantities sampled at $x_1=0.35~\text{m}$, when PR=1.5. The velocity, shear stress and viscosity are normalized by $\sqrt{RT}$, $p$ and $pL/\sqrt{RT}$, respectively.
    }
    \label{fig:H70Vis}
\end{figure}

The contributions to shear stress from different physical processes are shown in figure~\ref{fig:H70Vis}(b). The laminar part peaks at the outer shock and the shear layer, due to the increase in post-shock temperature (pulls up $\mu_{lam}$, as shown in figure~\ref{fig:H70Vis}(c)) and high velocity gradient across shock and shear layer. Meanwhile, the near-wall high velocity gradient also excites production of $\sigma_{12,lam}$ despite drop in $\mu_{lam}$. 
At the first peak (outer shock), gas rarefaction effect dominates over turbulence, since the turbulent peak is ignorable and the HoT peak is almost as large as the laminar one. 
Around the shear layer, turbulent part contributes greatly as the laminar part, while the HoT makes a small negative effect to shear stress. At the last peak of $\sigma_{12,lam}$ near wall, turbulent part drops to 0 due to the disappearance of $\mu_{turb}$ enforced by wall boundary condition, while HoT part again exhibits negative value for slip effect.
With this example at PR=1.5, it is clear that turbulence enhances momentum (figure~\ref{fig:H70VisDetail}(a)) and wall normal energy exchange (figure~\ref{fig:H70VisDetail}(b)), i.e. in the form of smmoth changes of GSIS-SST curves. Turbulence also impacts primarily the shear layer and the jet flow layer, and scales with PR, as shown in figure~\ref{fig:H70VisDetail}(c)

With enhanced momentum exchange by turbulence, the velocity distribution exhibits reduced slopes especially at high $\mu_{turb}$ region, as per comparison between GSIS-SST and GSIS. The enhanced energy exchange by turbulence could be observed through $\mu_{lam}$ (figure~\ref{fig:H70VisDetail}(b)), with the GSIS-SST solution predicts an earlier and smoother drop of $\mu_{lam}$.
Since turbulence smooths the momentum and energy change only inside the flow field, gradients adjacent to the wall go up. Meanwhile, increase in PR thickens jet flow layer, yet reducing further the gradients of velocity near wall. Due to the opposite effect of turbulence and PR, the turbulence shifts of shear stress and normal force thus suffer little from increased PR in the middle part of the model. 

%turbulence influences gradients
% turbulence mixing intensifies temperature gradient at the wall, leading to , leading to reduced turbulence influence on the model surface.
% incease in PR increases tempearture gradient at wall, increase in PR reduces slip effect, turbulence mixing is the near wall area does not further increase the energy exchange due to the already smooth temperature field, 

% With increase in PR, the thicker jet flow layer further leads a more smooth change of velocity below $x_2<0.02~\text{m}$, also a drop of $\mu_{lam}$ at further location from the wall. 
% Meanwhile, the dominant $\mu_{turb}$ from GSIS-SST in the near-wall jet flow layer could be seen scales positively with PR in figure~\ref{fig:H70VisDetail}(b). Thus, with decrease in velocity gradient, the shear stress in the middle part of the model does not suffer largely increased turbulence shift, despite the growth in $\mu_{turb}$. 

% low 1.5 slip, ulam high, turb increases velgrad near wall (reduce with PR), thus neg post together, change stablize
% the laminar viscosity drops at further location from the wall when PR increases
% free flow turbulence generally poses no influence to the flow field. 
% Meanwhile, gas rarefaction effect slightly counteracts to the turbulence effect around the shear layer, and greatly corrects the stress at the rarefied outer shock. %, and the wall shear stress
% emerges and significantly contributes to the blurred outer shock at 70~km as marked in figure~\ref{fig:H70Vis}(a), also effects the shear layer and the wall shear stress.

% With change in PR, the enhanced energy exchange could 
% Figure~\ref{fig:H70Vis}(c) shows again that the free flow turbulence does not impact the jet-controlled area, since turbulent viscosity from free flow ($|x_2| > 0.13~\text{m}$) and jet flow ($|x_2| < 0.035~\text{m}$) is wide separated by near zero values of $\mu_{turb}$. 
% When PR increases, these profiles are stretched in $x_2$ direction, with all the wall normal gradients get smoothed; they are not shown here due to such similarities. %Difference of $\mu_{lam}$ profile between GSIS-SST and GSIS exists at where $\mu_{turb}$ grows significantly.

% Figure~\ref{fig:H70VisDetail}(a) shows that with enhanced energy exchange by turbulence, , close to the wall ($|x_2| < 0.05~\text{m}$), the laminar viscosity drops at further location from the wall when PR increases, while the GSIS-SST solution predicts an earlier and smoother drop of $\mu_{lam}$. This indicates that the wall normal temperature gradient is smoothed with increasing PR and further smoothed by modeled turbulence.
% than GSIS when $|x_2|$ decreases, reflecting intensified energy exchange from hot outer flow to cold wall due to the additional $\mu_{turb}$, which smooths out the temperature gradients.

% Figure~\ref{fig:H70VisDetail}(b) shows that the dominant $\mu_{turb}$ from GSIS-SST scales positively with PR, while figure~\ref{fig:H70VisDetail}(c) proves that the velocity gradient $\partial{u_{1}}/\partial{x_2}$ is smoothed with increased PR, as the jet flow layer is thicker. Thus, despite the growth in $\mu_{turb}$, the shear stress in the middle part of the model does not suffer largely increased turbulence shift.
% It comes from upstream transport as mentioned previously (\leir{the strip in figure~\ref{fig:H70mu_r}}) and from local high velocity gradients. We believe the former contributes more, since as the PR increases, the velocity gradient $\partial{u_{1}}/\partial{x_2}$ is smoothed in figure~\ref{fig:H70VisDetail}(c).
\begin{figure*}
    \centering
    \subfloat[Velocity]{\includegraphics[width=0.32\linewidth]{Artworks/H70PRVelDetail.png}}
    \subfloat[Laminar Viscosity]{\includegraphics[width=0.32\linewidth]{Artworks/H70PRVis.png}}
    \subfloat[Turbulent Viscosity]{\includegraphics[width=0.32\linewidth]{Artworks/H70PRVisTurb.png}}
    \caption{Detailed profiles of viscosity and velocity in the near wall region at $x_1=0.35~\text{m}$ with different PR ratios.}
    \label{fig:H70VisDetail}
\end{figure*}

\leib{rise of the curve near the end}
As the jet flow layer proceeds to the end of the model, accompanied turbulence keeps enhancing momentum and energy exchange in the wall-normal direction, and also diminishes as $x_1$ grows. The cool near wall jet flow gets hotter due to turbulence diffusion, the molecular viscosity $\mu_{lam}$ in GSIS-SST increases thus faster than GSIS, resulting in an earlier loss of stress reduction effect, i.e. rise of GSIS-SST curves near the end of the model. Such rise of GSIS-SST gets earlier as PR decreases, since the the jet flow layer is thinner and more prone to free flow influence.

% While the heat flux or the temperature gradient change more vigorously with PR and turbulence effect, as shown in figure~\ref{fig:H70VisDetail}(a), thus a decreased turbulence influence with increasing PR is observed.
% high PR creates more thicker and smoother jet flow layer with reduced temperature gradient, leading to reduced heat flux. 
% The thicker jet flow layer also pushes the hot free flow further away, thus turbulence mixing is less influenced by the hot free flow, finally shaping a decreased turbulence influence with PR. 
% The dominance of turbulent viscosity in the jet flow region, particularly at higher PRs, highlights the importance of turbulence consideration in the near-wall flow, which substantially affects shear stress and heat transfer predictions. However, the above observations also indicates the difficulty of predicting the relation between turbulence influence and PR on surface quantities at this location:
% although turbulent viscosity increases as PR grows, laminar viscosity and velocity gradients drop. 








% \subsection{Flow structure}

% At different AoA, the flow structures vary notably, thus their density gradient magnitudes are all given in the left column of figure~\ref{fig:H80dRho}, their streamlines are also colored in Q as figure~\ref{fig:H70dRho}.

% % The left column of figure~\ref{fig:H80dRho} illustrates the density gradient magnitudes, highlighting the progressive compression of the jet-controlled region as the AoA increases. This compression is accompanied by the shrink of the jet-controlled region, surrounded by streamlines emanating from the jet exit. The streamlines 



% \begin{figure}
%     \centering
%     {\includegraphics[width=0.49\linewidth, trim={0 20 0 80}, clip]{Artworks/H80AoA0dRhoCPQ.png}}
%     {\includegraphics[width=0.49\linewidth, trim={0 20 0 80}, clip]{Artworks/H80A0TKEMuR.png}}\\
%     % {\includegraphics[width=0.49\linewidth, trim={0 20 0 80}, clip]{Artworks/H80A15DissiQ.png}}
%     {\includegraphics[width=0.49\linewidth, trim={0 20 0 80}, clip]{Artworks/H80AoA15dRhoCPQ.png}}
%     {\includegraphics[width=0.49\linewidth, trim={0 20 0 80}, clip]{Artworks/H80A15TKEMuR.png}}\\
%     {\includegraphics[width=0.49\linewidth, trim={0 20 0 80}, clip]{Artworks/H80AoA30dRhoCPQ.png}}
%     {\includegraphics[width=0.49\linewidth, trim={0 20 0 80}, clip]{Artworks/H80A30TKEMuR.png}}
%     \caption{(Left column) Contours of density gradient magnitude and streamlines colored in Q-criterion, with upper half from GSIS and lower half from GSIS-SST. (Right column) Contours of turbulent kinetic energy (upper half) and turbulent-to-laminar viscosity ratio (lower half) from GSIS-SST. The altitude is 80~km, and AoA are 0° (top), 15° (middle) and 30° (bottom).
%     % with upper half from GSIS and lower half from GSIS-SST. (Right column) Contours of turbulent kinetic energy (upper half) and turbulent-to-laminar viscosity ratio (lower half) from GSIS-SST at 80~km and AoA=0° (top) and 30° (middle), with upper half from GSIS and lower half from GSIS-SST. (Right column, bottom) Contour of viscous dissipation rate and streamlines colored in Q criterion at 80~km and AoA=30°, with upper half from GSIS and lower half from GSIS-SST. 
%     }
%     \label{fig:H80dRho}
% \end{figure}
% Upstream separation region experiences non-linear pattern of change with AoA. Large upstream separation but weak rotation is observed at AoA = 0°. A secondary upstream vortex also develops, reaching its largest size at this AoA. Reduced separation and strong vortex is present at AoA = 15°, the upstream vortices reach their maximum size due to enhanced shear between the jet and free stream, which generates increased vorticity and promotes vortex growth. However, as AoA increases further, the intensified interaction further compresses the vortices, limiting their rotational freedom, left only a tiny vortex. Similar as the results at 70~km, turbulence poses minimum influence on the upstream region.

% The downstream region follows in contrast a monotonic pattern of change and presents most of the influence from turbulence. The height of the downstream separation region reduces as AoA increases, and the length increases. The Q-criterion highlights the difference between GSIS-SST and GSIS, which gets obvious around the downstream vortex since AoA=15°. The recompression shock in GSIS-SST also comes earlier than GSIS with increasing AoA, as indicated by the transition of Q from red to blue in figure~\ref{fig:H80dRho}.

% % Downstream of the jet exit, the expansive jet flow prevents free-stream reattachment to the surface, resulting in dominant jet behavior in the near-wall region and making it difficult to define the penetration height. A large downstream vortex is also observed in this configuration.

% % Reduced separation and strong vortex is present at AoA = 15°, the upstream vortices reach their maximum size due to enhanced shear between the jet and free stream, which generates increased vorticity and promotes vortex growth. 
% % However, as AoA increases further, the intensified interaction compresses the vortices, limiting their rotational freedom. 
% % This compression represents a balance between shear-driven vortex growth and the constraining effects of excessive strain, which suppresses further development of vortices.

% % Comparing GSIS-SST and GSIS models reveals that turbulence plays a critical role in regions of strong shear and vortex dynamics. Turbulence helps stabilize and organize vortices, even under conditions of intensified stretching and high shear at larger AoAs.
% Turbulence also affects vortex dynamics. At AoA = 0°, the downstream vortex shrinks and its high-Q region contracts slightly compared to the laminar GSIS solution, which stretches further. This suggests that the absence of turbulent dissipation in GSIS leads to a less stable vortex. In the downstream vortex, stretching converts rotational energy into TKE, enhancing viscous dissipation and explaining the differences between GSIS and GSIS-SST results.
\section{The influence of AoA}\label{sec:AoA}

The AoA is varied among 0°, 15° and 30°, mimicking the maneuver of the hypersonic vehicles. The flight altitude is increased to 80~km, corresponding to Kn=0.0375 for the model in figure~\ref{fig:H70TtComment}, since attitude adjustment of hypersonic flight vehicles is more likely to happen at higher altitudes. The jet PR is kept at 2.5. 

\subsection{Turbulence influence on surface quantities}
Increasing discrepancies on surface shear stress and heat flux are noticed with the rise of AoA at 80~km, as shown in figure~\ref{fig:H80tauxy}.

% Figure \ref{fig:H80tauxy} illustrates the surface shear stress $\sigma_{12}$ on the lower surface downstream of the jet exit, th a local positive peak around $x_1 = 0.23~\text{m}$ followed by a steady decrease. T
A negative peak at around 0.15~m could be seen for all AoAs and scales with increasing AoA. The $\sigma_{12}$ exhibits a comparable pattern to the results at 70~km altitude shown in figure \ref{fig:H70tauQFM}. 
Yet the location of the local positive peak (around $x_1 \approx 0.2~\text{m}$) does not show a consistent pattern of change with AoA, as it rests most closely to the jet exit at AoA = 15° ($x_1 = 0.19~\text{m}$). The peak is also less pronounced in GSIS solution at high AoA. % possibly due to the most elongated downstream vortex as in figure~\ref{fig:H80dRho}. 
After the positive peak, shear stress drops continuously for all AoA. 

%23.7 30, 14.9 15, 8.9 0.
Regarding the difference between GSIS-SST and GSIS, a positive relation between turbulence effect and AoA could be seen before the positive peaks. Afterwards, a stable turbulence shift at each PR is observed, though the relative difference differs among AoAs greatly.
Despite obvious discrepancies among shear stress, the turbulence effect on the integrated forces and moment is within 5\%, as the turbulence independent upstream interaction contributes more at this altitude.
% As for the difference between GSIS-SST and GSIS, only two stages could be observed since PR=2.5, just as the case at 70~km. The first stage also shows a positive relation between turbulence effect and AoA, while the second stage still shows stable turbulence shift at each PR, though the relative difference differs among PRs greatly.
% At AoA = 15°, the peak shifts closer to the jet exit, around $x_1 = 0.19~\text{m}$, and the stress gradually declines downstream. For AoA = 30°, such positive peak shifts again downstream, but the local peak at $x_1 = 0.2~\text{m}$ is less pronounced in GSIS solution. Across all cases, the GSIS-SST solution consistently predicts higher values of $\sigma_{12}$ compared to GSIS. 
% The difference induced by turbulence around the positive peak correlate positively with AoA, while on the aft section of the model, relationship between the turbulence influence and AoA gets hard to decide. 

% The second figure of figure~\ref{fig:H80tauxy} shows surface heat flux distributions. receives great influence from angle of attack. The heat flux stays 
As for the surface heat flux in figure~\ref{fig:H80tauxy}, it stays at low values throughout the model surface at low AoA, and increases significantly as AoA gets larger.
A local peak is present near $x_1 = 0.16\sim0.20~\text{m}$ across all AoAs. %but its prominence rises as the AoA increases.
Heat flux after the local peak drops constantly at AoA=0° both in GSIS and GSIS-SST, with the latter being slightly higher than the former, indicating enhanced mixing and degraded cooling effect in GSIS-SST under turbulence influence. As AoA goes up, this dropping trend is replaced by an increasing trend, and an expanded discrepancy between GSIS-SST and GSIS.
%The relative difference of heat flux between the solvers rest around $30\%\sim40\%$, generally increase together with AoA. 
The maximum relative difference of heat flux between the solvers rest around $47\%\sim70\%$, generally increase together with AoA.

% The turbulence effect on the integrated forces and moment is within 5\%, since the observed local difference is not enough (as at 70~km) to alter the total forces and moment, which depend more on the turbulence independent upstream interaction.
% As for integrated forces and moment, a faint positive relation between AoA and the turbulence effect for the axial force could be noticed, since the largest relative difference of GSIS-SST relative to GSIS occurs at AoA=30°, where a 5\% difference is observed. %this observation proved the inference based on the $\mu_{turb}$ profile in the previous part. they vary with AoA positively. A
% And for the normal force and pitch moment, no sensible difference between GSIS-SST and GSIS is identified, as they depend more on less sensitive surface pressure distribution, which does not vary much due to turbulence at 80~km.

% The observed changes in surface quantities again confirm the positive relation between turbulence influence and angle of attack. As AoA increases, the the jet flow bends sharply and impinges on the wall heavily, compressing the jet-controlled area, promoting development of thinner boundary layer and higher gradients, producing thus more turbulence kinetic energy and influence.


\begin{figure}
    \centering
    \includegraphics[width=0.32\linewidth,trim={0 0 0 0},clip]{Artworks/H80txy2.png}
    \includegraphics[width=0.32\linewidth,trim={0 0 0 0},clip]{Artworks/H80Q2.png}
    \caption{Variation of surface shear stress and heat flux at altitude 80~km with AoA.
    }
    \label{fig:H80tauxy}
\end{figure}



\subsection{Turbulent Quantities}

% The right column of figure~\ref{fig:H80dRho} presents the distributions of turbulent kinetic energy and turbulent-to-laminar viscosity ratio, which shows increasingly concentrated and intense TKE and $\mu_r$ as AoA increases.
% The distribution of TKE and $\mu_r$ follows similar pattern as those at 70~km (figure~\ref{fig:H70mu_r}).

% The production of TKE after jet Mach disk reduces as AoA increases, while the TKE production from near wall layer intensifies. At AoA = 0°, a high TKE region forms around the Mach disk, where the small angle between the free stream and jet flow allows the jet to expand with minimal compression, and thus a stronger Mach disk which higher AoA does not enjoy.
% leading to low TKE production outside this region.
% A strip of large TKE appears along the elongation direction of the downstream vortex, driven by sharp velocity gradients in the developing near-wall boundary layer, most notably at AoA = 30° as in figure~\ref{fig:H80dRho}(f).

% The turbulent viscosity ratio $\mu_r$ follows the TKE distribution, peaking in jet-dominated regions and vanishing where the free stream dominates, due to the higher post-shock temperature, similar as the situation at 70~km (figure~\ref{fig:H70mu_r}). Besides, the source of high $\mu_r$ is more biased toward the near wall layer rather than jet and Mach disk. Although the intensity of $\mu_r$ increases as AoA goes up, the thickness diminishes. 

% These distinct behaviors of TKE and $\mu_r$ with AoA make it difficult to predict the overall influence of turbulence with variation in AoA.

% This indicates that turbulence is localized near high-gradient flow features and is independent of far-field conditions, highlighting the turbulence model’s sensitivity to localized effects.


% As AoA increases, TKE production intensifies near shock structures, except around the Mach disk, where it drops. This drop is due to the reduced jet expansion at higher AoA, which decreases the shock front Mach number and weakens the Mach disk. Additionally, a intensified strip of TKE and $\mu_{r}$ extends from the stretched vortex to the downstream boundary layer, implying growing turbulence influence with higher AoAs.

%compression induce higher post shock temperature, temp diffuse as x1 grows, near wall Tgradient increases, (GSIS-SST larger than GSIS), thus higher q 
%High AoA compression, high temperature and t diffusion, mu_r increases fast and early, but also decreases faster; therefore, overall effect seems stagnate, or balanced out.

%\subsection{Profiles of field quantities}
The distribution of $\mu_r$ follows similar pattern as those at 70~km (figure~\ref{fig:H70mu_r}). High AoA further compresses the downstream vortex, elongates the vortex in $x_1$ direction and builds up steeper wall normal gradients. Rise of AoA also promotes turbulence generation through vortex deformation, and the produced turbulence viscosity smooths out the vorticity in the vortex core, but increases velocity gradient near wall, therefore shaping positive relative between turbulence influence and AoA before the positive peaks in figure~\ref{fig:H80tauxy}.

Shear stress components at the middle of the model are examined: laminar ($\sigma_{12,lam}$), turbulent ($\sigma_{12,turb}$), and rarefaction-induced ($\sigma_{12,HoT}$) at $x_1=0.35~\text{m}$, as shown in figure~\ref{fig:H80Proftxy}, to compare GSIS-SST and GSIS from a more elemental aspect.
\begin{figure}%[h]
    \centering
    \vspace{0.3cm}
    \subfloat[AoA= 0°]{\includegraphics[width=0.32\linewidth]{Artworks/H80AoA0Proftxy.png}}
    \subfloat[AoA= 15°]{\includegraphics[width=0.32\linewidth]{Artworks/H80AoA15Proftxy.png}}
    \subfloat[AoA= 30°]{\includegraphics[width=0.32\linewidth]{Artworks/H80AoA30Proftxy.png}}
    \caption{The GSIS-SST results of the NS laminar, turbulent and rarefied parts of shear stress at $x_1=0.35~\text{m}$ at the altitude of 80~km.
    }
    \label{fig:H80Proftxy}
\end{figure}

% The contribution of turbulence to shear stress is seen limited in the near wall jet flow layer, and rises as AoA goes up. 
The shear stresses display a positive stretch and compression toward the wall as AoA increases.
Separated regions of dominance by turbulent contribution and rarefaction-induced HoT are observed again. 
% At AoA = 0°, $\sigma_{12,lam}$ has three peaks: at $|x_2|=0.2~\text{m}$ (outer shock), $|x_2|=0.08~\text{m}$ (shear layer), and near the wall. 
Turbulent part $\sigma_{12,turb}$ is negligible except within the jet boundary layer, where it matches the magnitude of $\sigma_{12,lam}$ and scales with AoA. The rarefaction-related stress $\sigma_{12,HoT}$ exhibits a similar but extended influence range compared with the 70~km case, with the exception of the negative impact within the free flow post-shock area. This negative contribution diminishes as the rarefaction effect is reduced when AoA increases.% The $\sigma_{12,HoT}$ also presents a negative influence near the wall to induce velocity slip.


% At higher AoAs, stress components also shift closer to the wall, with $\sigma_{12,lam}$ and $\sigma_{12,turb}$ extending rightward due to increased compression and shear. $\sigma_{12,HoT}$ also increases, extending further into the outer shock region, but its negative portion diminishes as the rarefaction effects reduce.
%, most apparently reducing the negative influence of rarefaction behind the outer shock

\begin{figure}[h]
    \centering
    \subfloat[Laminar viscosity]{\includegraphics[width=0.32\linewidth]{Artworks/H80ProfVisDetail2.png}}
    \subfloat[Turbulent viscosity (GSIS-SST)]{\includegraphics[width=0.32\linewidth]{Artworks/H80ProfVisDetailTurb.png}}
    \caption{Profile of viscosity at $x_1=0.35~\text{m}$ at altitude 80~km. 
    } 
    \label{fig:H80Viscosity}
\end{figure}

As shown in figure~\ref{fig:H80Viscosity}, both $\mu_{lam}$ and $\mu_{turb}$ increase near the wall at high AoAs. The rise of $\mu_{lam}$ could be attributed to compression induced higher temperature gradient, and $\mu_{turb}$ of GSIS-SST further intensifies the near-wall rise of $\mu_{lam}$, a typical difference between turbulent and laminar boundary layer profile. The $\mu_{turb}$ increases due to enhanced compression and the associated higher shearing. Obvious increase in maximum magnitude of $\mu_{turb}$ is accompanied with the rise of AoA as shown in figure~\ref{fig:H80Viscosity}(b), yet the influential range shrinks abruptly as AoA grows from 0° to 15°, and stays similarly thereafter, implying a non-linear relationship. 

% In contrast to diminished near-wall velocity gradient and thus the decreasing shear stress curve toward the end of the model, the higher $\mu_{lam}$, $\mu_{turb}$ and temperature gradient at higher AoA together lead to the faster rise and turbulence shift of heat flux curve along $x_1$ direction. 

For surface heat flux, rise in AoA has similar effect of decrease in PR, as higher AoA results in thinner jet flow layer, thus higher temperature gradient at wall (could be read from $\mu_{lam}$ in figure~\ref{fig:H80Viscosity}(a)) and degradation of heat flux reduction effect. With the increased turbulence viscosity in the jet layer further rise up wall temperature gradient, the heat flux rises further from GSIS-SST.

% This suggests that turbulence enhances momentum and energy exchange at specific locations as AoA increases, but its overall significance may be difficult to estimate as AoA increases, especially within AoA=0° to 15°. %The surface shear stress and heat flux distribution in the next part provide then more information., shaping the displayed difference between GSIS-SST and GSIS.




